Cryptography with Certified Deletion

We propose a new, unifying framework that yields an array of cryptographic primitives with certified deletion. These primitives enable a party in possession of a quantum ciphertext to generate a classical certificate that the encrypted plaintext has been information-theoretically deleted, and cannot be recovered even given unbounded computational resources. - For X \in {public-key, attribute-based, fully-homomorphic, witness, timed-release}, our compiler converts any (post-quantum) X encryption to X encryption with certified deletion. In addition, we compile statistically-binding commitments to statistically-binding commitments with certified everlasting hiding. As a corollary, we also obtain statistically-sound zero-knowledge proofs for QMA with certified everlasting zero-knowledge assuming statistically-binding commitments. - We also obtain a strong form of everlasting security for two-party and multi-party computation in the dishonest majority setting. While simultaneously achieving everlasting security against all parties in this setting is known to be impossible, we introduce everlasting security transfer (EST). This enables any one party (or a subset of parties) to dynamically and certifiably information-theoretically delete other participants' data after protocol execution. We construct general-purpose secure computation with EST assuming statistically-binding commitments, which can be based on one-way functions or pseudorandom quantum states. We obtain our results by developing a novel proof technique to argue that a bit b has been information-theoretically deleted from an adversary's view once they output a valid deletion certificate, despite having been previously information-theoretically determined by the ciphertext they held in their view. This technique may be of independent interest.

==> EST-3-deprecated.tex <==
\section{Cryptography with Everlasting Security Transfer}
\label{sec:2pc-est}

In this section, we construct bit commitment and secure computation schemes that satisfy our notion of Everlasting Security Transfer (EST). In \cref{subsec:2PC-defs}, we formalize the notion of deletion and EST in the context of simulation security. We also derive a quantum sequential composition theorem for \emph{reactive functionalities}, extending the framework of \cite{C:HalSmiSon11}. Extending to reactive functionalities is crucial for us, since the bit commitment functionality we compose has multiple phases. Finally, we formalize composition of protocols with EST, defining the notion of a ``deletion-composable'' protocol. Next, we show how to construct ideal commitments with EST in \cref{subsec:one-sided} and \cref{subsec:ideal}, via a two-step process outlined in \cref{subsec:tech-overview}. Finally, in \cref{subsec:secure-computation}, we make use of our ideal commitment with EST, our composition theorems, and known compilers, to obtain the notions of two-party and multi-party computation with EST.


\subsection{Definitions}\label{subsec:2PC-defs}

\paragraph{Ideal functionalities.}

An ideal functionality $\cF$ is a classical interactive machine specifying some (potentially reactive) distributed classical computation. Reactive means that the distributed computation is broken into multiple ``phases'' with distinct inputs and outputs, and the outputs of previous phases may be used as inputs in later phases. For now, we will specifically consider \emph{two-party} functionalities. Each invocation of an ideal functionality is associated with some session id $\mathsf{sid}$. We will be interested in designing protocols that \emph{securely realize} ideal functionalities (defined later), but first we specify the main ideal functionality that we consider in this work: bit commitment $\cF_\com$. %and oblivious transfer $\cF_\OT$.

\protocol{Ideal functionality $\cF_\com$}{Specification of the bit commitment ideal functionality.}{fig:comIF}{
Parties: committer $C$ and receiver $R$
\begin{itemize}
    \item Commit phase: $\cF_\com$ receives a query $(\text{Commit},\mathsf{sid},b)$ from $C$, records this query, and sends $(\text{Commit},\mathsf{sid})$ to $R$.
    \item Reveal phase: $\cF_\com$ receives a query $(\text{Reveal},\mathsf{sid})$ from $C$, and if a message $(\text{Commit},\mathsf{sid},b)$ has been recorded, sends $(\text{Reveal},\mathsf{sid},b)$ to $R$.
\end{itemize}
\noindent}

%\protocol{Ideal functionality $\cF_\OT$}{A specification of the string oblivious transfer ideal functionality.}{fig:OTIF}{
%Parameters: message length $n = n(\secp)$\\
%Parties: sender $S$ and receiver $R$
%\begin{itemize}
    %\item $\cF_\OT$ receives a query $(\text{Sender},\mathsf{sid},m_0,m_1)$ from $S$, where $m_0,m_1 \in \{0,1\}^n$, and records $(\text{Sender},\mathsf{sid},m_0,m_1)$. 
    %\item $\cF_\OT$ receives a query $(\text{Receiver},\mathsf{sid},b)$ from $R$. If a message $(\text{Sender},\mathsf{sid},m_0,m_1)$ has been recorded, send $(\text{Output},\mathsf{sid},m_b)$ to $R$, and otherwise ignore the message.
%\end{itemize}
%}

In this work, we will consider augmenting ideal functionalities with a ``deletion phase'', which can be used by parties to transfer everlasting security. When parties are labeled $A$ and $B$, we maintain the precedent that deletion is from $B$ to $A$, that is, $A$ can request that $B$ deletes $A$'s information.

\protocol{Deletion phase}{Specification of a generic deletion phase that can be added to any ideal functionality $\cF$.}{fig:delPhase}{
Parties: $A$ and $B$
\begin{itemize}
    \item Receive a query $(\mathsf{DelRequest},\mathsf{sid})$ from $A$, and send $(\mathsf{DelRequest},\mathsf{sid})$ to $B$.
    \item Receive a query $(\mathsf{DelResponse},\mathsf{sid})$ from $B$. If a message $(\mathsf{DelRequest},\mathsf{sid})$ has been recorded, send $(\mathsf{DelResponse},\mathsf{sid})$ to $A$, and otherwise ignore the message. %\textcolor{red}{removing the $d$, since if the receiver does not delete that can just be denoted by no DeleteResponse message from $B$.}
\end{itemize}
}

Importantly, if a deletion phase is added to a \emph{reactive} functionality $\cF$, we allow party $A$ to request the Deletion phase (send $\mathsf{DelRequest}$) \emph{between any two phases of $\cF$}, or \emph{at the end of $\cF$}. But, once the Deletion phase has been executed, this marks the end of the reactive functionality, so no other phases will be executed.

\paragraph{Security with abort.} In what follows, we will by default consider the notion of \emph{security with abort}, where the ideal functionality $\cF$ is always modified to (1) know the identities of corrupted parties and (2) be slightly reactive: after all parties have provided input, the functionality computes outputs and sends these outputs to the corrupt parties only. Then the functionality awaits either a ``deliver'' or ``abort'' command from the corrupted parties. Upon receiving ``deliver'', the functionality delivers any honest party outputs. Upon receiving ``abort'', the functionality instead delivers $\abort$ to all the honest parties.

\paragraph{The real-ideal paradigm.} A two-party protocol $\Pi_\cF$ for computing the (potentially reactive) functionality $\cF$ consists of two families of quantum interactive machines $A$ and $B$. An adversary intending to attack the protocol by corrupting a party $M \in \{A,B\}$ can be described by a family of sequences of quantum interactive machines $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$, where $\ell$ is the number of phases of $\cF$. This adversarial interaction happens in the presence of an \emph{environment}, which is a family of sequences of quantum operations $\{\cZ_\secp \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$, and a family of initial advice states $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$. It proceeds as follows.

\begin{itemize}
    \item $\cZ_{\secp,1}$ receives as input $\ket{\psi_\secp}$. It outputs what (if any) inputs the honest party $H \in \{A,B\}$ is initialized with for the first phase of $\Pi_\cF$. It also outputs a quantum state on registers $(\sA,\sZ)$, where $\sA$ holds the state of the adversary and $\sZ$ holds the state of the environment,
    \item $\cA_{\secp,1}$ receives as input a state on register $\sA$, and interacts with the honest party in the first phase of $\Pi_\cF$. It outputs a state on register $\sA$.
    \item $\cZ_{\secp,2}$ receives as input registers $(\sA,\sZ)$ along with the honest party outputs from the first phase. It computes honest party inputs for the second phase, and updates registers $(\sA,\sZ)$.
    \item $\cA_{\secp,2},\cZ_{\secp,3},\dots,\cA_{\secp,\ell}$ are defined analogously.
\end{itemize}

Given an adversary, environment, and advice, we define the random variable $\Pi_\cF[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ as the output of the above procedure, which includes registers $(\sA,\sZ)$ and the final honest party outputs.

An \emph{ideal-world} protocol $\widetilde{\Pi}_\cF$ for functionality $\cF$ consists of ``dummy'' parties $\widetilde{A}$ and $\widetilde{B}$ that have access to an additional ``trusted'' party that implements $\cF$. That is, $\widetilde{A}$ and $\widetilde{B}$ only interact directly with $\cF$, providing inputs and receiving outputs, and do not interact with each other. We consider the execution of ideal-world protocols in the presence of a simulator, described by a family of sequences of quantum interactive machines $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$, analogous to the definition of an adversary above. This interaction also happens in the presence of an environment $\{\cZ_\secp \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$, and a family of initial advice states $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, as described above, and we define the analogous random variable $\widetilde{\Pi}_\cF[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.

%\paragraph{Local simulation.} In what follows, we will say that protocol $\Pi_\cF$ \emph{securely realizes} the functionality $\cF$ if, roughly, for every QPT adversary $\{\cA_\secp\}_{\secp \in \bbN}$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$ such that the outputs of $\Pi_\cF[\ket{\psi_\secp},\cA_\secp]$ and $\widetilde{\Pi}_\cF[\ket{\psi_\secp},\cS_\secp]$ are computationally indistinguishable. However, in order to obtain good (sequential) composability guarantees for reactive functionalities, we will restrict the type of valid simulators that we consider. 

%We define \emph{local simulation} as follows. Consider any quantum interactive machine $\cA = \cA_\secp$ attacking a protocol $\Pi_\cF$ for a reactive functionality $\cF$ with $\ell$ phases. Without loss of generality, we can write $\cA \coloneqq (\cA_1,\cB_1,\cA_2,\dots,\cB_{\ell-1},\cA_\ell)$ with the following properties.
%\begin{itemize}
    %\item Each $\cA_i$ is a quantum interactive machine and each $\cB_i$ is a quantum operation.
    %\item All $\cA_i$ and $\cB_i$ have the same input and output register $\sA$.
    %\item $\cA_1$ is initialized with the $\sA$ register of some advice state $\ket{\psi}$ and interacts with the honest party in the first phase of $\cF$. The output of $\cA_1$ is the state on $\sA$ right after the last message of the first phase of $\Pi_\cF$ is sent (whether it is from the adversary or the honest party).
    %\item $\cB_1$ is initialized with $\sA$, and outputs the state right before the first message of the second phase of $\Pi_\cF$ is sent. 
    %\item $\cA_2$ is initialized with $\sA$, and interacts with the honest party in the second phase of $\cF$, from right before the first message is sent, to right after the last message is sent. 
    %\item $\cB_2,\dots,\cA_\ell$ are defined similarly. 
%\end{itemize}

%Then, $\cS$ is a \emph{local simulator} defined based on $\cA$ if the following properties hold.
%\begin{itemize}
    %\item The description of $\cS$ includes interactive machines $\cS_1,\dots,\cS_\ell$, where each $\cS_i$ is defined based only on $\cA_i$, and each $\cS_i$ operates on two registers: the adversary's state register $\sA$, and a simulator's state register $\sS$. Moreover, each $\cS_i$ just interacts with the $i$'th phase of the ideal functionality $\cF$.
    %\item The simulator $\cS$ operates as follows. It initializes $\cS_1$ with the $\sA$ register of the advice state $\ket{\psi}$ and the register $\sS$ initialized with 0 qubits. After $\cS_1$ outputs registers $(\sA,\sS)$, it runs $\cB_1$ on $\sA$. Then, it runs $\cS_2$ on $(\sA,\sS)$, $\cB_2$ on $\sA$, and so on until $\cS_\ell$ outputs $(\sA,\sS)$. Finally, $\sS$ is discarded, and $\sA$ is passed on to the distinguisher.
%\end{itemize}





%Then, a local simulator is a simulator $\cS_\secp$ defined based on $\cA_\secp$, where each chunk of $\cS_\secp$ that interacts in a phase of $\cF$ is defined solely (but arbitrarily) based on the corresponding chunk of $\cA_\secp$, and each chunk of $\cS_\secp$ that operates between phases is defined to be exactly equal to the corresponding chunk of $\cA_\secp$. 

\paragraph{Secure realization and composition.} Now, we formally define what it means for a protocol $\Pi_\cF$ to securely realize a (potentially reactive) functionality $\cF$. We give definitions for both computational and statistical security.

\begin{definition}[Computational secure realization]\label{def:securerealization}
A protocol $\Pi_\cF$ \emph{computationally securely realizes} the $\ell$-phase functionality $\cF$ if for every QPT adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting either party $A$ or $B$, there exists a QPT simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ such that for any QPT environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$, polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, and QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, it holds that \[\bigg|\Pr\left[\cD_\secp\left(\Pi_\cF[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = 1\right] - \Pr\left[\cD_\secp\left(\widetilde{\Pi}_\cF[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = 1\right]\bigg| = \negl(\secp).\]
\end{definition}

For the notion of statistical secure realization, we allow the adversary and environment to be unbounded, but we require that the simulator is at most polynomially larger than the adversary. 

\begin{definition}[Statistical secure realization]\label{def:statsecurerealization}
A protocol $\Pi_\cF$ \emph{statistically securely realizes} the $\ell$-phase functionality $\cF$ if there exists a polynomial $p(\cdot)$ such that for every (potentially unbounded) adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting either party $A$ or $B$, there exists a simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ with size at most $p(\secp)$ times the size of $\{\cA_\secp\}_{\secp \in \bbN}$, such that for any (potentially unbounded) environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$ and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, it holds that \[\TD\left(\Pi_\cF[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}],\widetilde{\Pi}_\cF[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp).\]
\end{definition}

\begin{remark}
Recall that trace distance between two distributions is an upper bound on the advantage that any unbounded machine has in distinguishing the distributions, so the above definition is equivalent to saying that no unbounded distinguisher has better than negligible advantage in distinguishing the real and ideal world outputs.
\end{remark}


Next, we consider the \emph{hybrid} model, where parties can make calls to an ideal-world protocol implementing some ideal functionality $\cG$. We call such a protocol a $\cG$-hybrid protocol, and denote it $\Pi^{\cG}$. Supposing that we also have a real-world protocol $\Gamma$ implementing $\cG$, we can consider the \emph{composed} protocol $\Pi^{\cG/\Gamma}$, where each invocation of $\cG$ is replaced with an invocation of the protocol $\Gamma$ for computing $\cG$. In this work, while we allow $\Pi$ to utilize many invocations of $\Gamma$, \textbf{we require that each phase of each invocation of $\Gamma$ is \emph{atomic}, meaning that no other protocol messages are interleaved during each phase of $\Gamma$}. That is, if $\cG$ is a reactive functionality, we allow different phases of different invocations to be interleaved, but we require that at any point in time, only a single phase is being executed, and no other protocol messages are interleaved during the computation of this phase. In this case, we can show the following sequential composition theorem, which is a straightforward extension of the composition theorem given in \cite{C:HalSmiSon11} to handle reactive functionalities.

\begin{theorem}[Extension of \cite{C:HalSmiSon11}]\label{thm:composition}
Let $\cF$ and $\cG$ be (potentially reactive) functionalities, let $\Pi^\cG$ be a $\cG$-hybrid protocol that computationally (resp. statistically) securely realizes $\cF$, and let $\Gamma$ be a protocol that computationally (resp. statistically) securely realizes $\cG$. Then, $\Pi^{\cG/\Gamma}$ computationally (resp. statistically) securely realizes $\cF$.
\end{theorem}

\begin{proof}
Let $\cG$ be a reactive $\ell$-phase functionality. Throughout this proof, we drop the dependence on $\secp$ for convenience. Let $(\cA,\cZ)$ be any adversary and environment attacking the protocol $\Pi^{\cG/\Gamma}$. Consider the first time in $\Pi^{\cG/\Gamma}$ that $\Gamma$ is invoked, which means the first time that the first phase of some subroutine $\Gamma$ is invoked (we note that other $\Gamma$ subroutines could occur between the phases of this first invocation). Write $(\cZ_1,\cA_1,\dots,\cZ_\ell,\cA_\ell)$ as an adversary and environment attacking the protocol $\Gamma$, according to the following. 

\begin{itemize}
    \item $\cZ_1$ runs $\cZ$ and then runs the interaction between $\cA$ and the honest party until right before the first time $\Gamma$ is invoked in $\Pi^{\cG/\Gamma}$. It outputs the adversary's state on register $\sA$, the honest party's input to $\Gamma$, and any other state kept by $\cZ$ along with the honest party's state on register $\sZ$.
    \item $\cA_1$ consists of the part of $\cA$ that interacts in the first phase of $\Gamma$. It takes as input a state on $\sA$ and outputs a state on $\sA$.
    \item $\cZ_2$ takes as input registers $(\sA,\sZ)$ and the honest party's output from $\Gamma$. It runs the interaction between $\cA$ and the honest party in $\Pi^{\cG/\Gamma}$ until right before the second phase of $\Gamma$ is invoked.
    \item $\cA_2,\cZ_3,\dots,\cA_\ell$ are defined analogously.
\end{itemize}

Now, since $\Gamma$ computationally (resp. statistically) securely realizes $\cG$, there exists a simulator $(\cS_1,\dots,\cS_\ell)$ defined based on $(\cA_1,\dots,\cA_\ell)$ such that, if we replace each $\cA_i$ interacting with the honest party with $\cS_i$ interacting with the ideal functionality $\cG$, then the output remains computationally (resp. statistically) indistinguishable. Note that the resulting interaction, defined by $(\cZ_1,\cS_1,\dots,\cZ_\ell,\cS_\ell)$, can be described by an adversary and environment $(\cA',\cZ)$ attacking the protocol $\Pi^{\cG/\Gamma}$ where the first invocation of $\Gamma$ is replaced with the parties querying the ideal functionality $\cG$. This follows because only the parts of $\cA$ that interacted in the first invocation of $\Gamma$ were changed, since each phase of $\Gamma$ was atomic. Now, continuing this argument for each invocation of $\Gamma$, we eventually arrive at an adversary and environment $(\cA'',\cZ)$ attacking the $\cG$-hybrid protocol $\Pi^\cG$. Note that $\cA''$ was defined based on $\cA$, and $\cZ$ remained unchanged. Thus, the fact that $\Pi^\cG$ computationally (resp. statistically) securely realizes $\cF$ completes the proof of the theorem, since we can define a simulator $\cS''$ based on $\cA''$, where indistinguishability will hold for any environment $\cZ$. 
%
%Note that there may be a part of the adversary that interacts in $\Pi^{\cG/\Gamma}$ before the first phase of $\Gamma$ is invoked, and we will include this part in the computation of the initial advice state $\ket{\psi}$ which is given to $\cA_1$. Then, since $\Gamma$ computationally (resp. statistically) securely realizes $\cG$ with local simulation, we can define a simulator $(\cS_1,\cB_1,\dots,\cS_\ell)$ as described above, which interacts with the $\ell$ phases of ideal functionality $\cG$. This simulator now defines an adversary $\cA'$ attacking the protocol $\Pi^{\cG/\Gamma}$, where the first time that $\Gamma$ is invoked, the parties actually query the ideal functionality $\cG$ instead. Note that we can still define a valid adversary $\cA'$ because only the parts of $\cA$ that interacted in the first invocation of $\Gamma$ were changed, by the local simulation guarantee and the fact that each phase of $\Gamma$ was atomic. Now, continuing this argument for each invocation of $\Gamma$, we eventually arrive at an adversary $\cA''$ attacking the $\cG$-hybrid protocol $\Pi^\cG$. Thus, the fact that $\Pi^\cG$ computationally (resp. statistically) securely realizes $\cF$ with local simulation completes the proof of the theorem. 
\end{proof}

\paragraph{Secure realization with everlasting security transfer.}

Next, we define the notion of secure realization with everlasting security transfer (EST). Here, parties are interested in securely computing an ideal functionality $\cF$ with a \emph{deletion phase} added to the end, which we denote by $\cF^{\Del}$. 

The deletion phase adds one bits to each honest party output, which we denote by $\mathsf{DelReq}$ (which is party $B$'s output, and is set to 1 if party $A$ initiates the Delete phase by issuing a request, and 0 otherwise) and $\mathsf{DelRes}$ (which is party $A$'s output, and is set to 1 if party $B$ sends a Delete response and 0 otherwise). Then, we have the following definition.

\begin{definition}[Secure realization with Everlasting Security Transfer]\label{def:security-with-EST}
A protocol $\Pi_\cF$ securely realizes the $\ell$-phase functionality $\cF$ between parties $A$ and $B$ with EST if $\Pi_\cF$ computationally securely realizes $\cF^\Del$ (\cref{def:securerealization}) and the following additional properties hold.
\begin{itemize}
\item
{\bf Statistical security against $A$ when no security transfer occurs.} There exists a polynomial $p(\cdot)$ such that for every (potentially unbounded) adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting party $A$, there exists a simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ with size at most $p(\secp)$ times the of size of $\{\cA_\secp\}_{\secp \in \bbN}$, such that for any (potentially unbounded) environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$ and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF^\Del}^{\mathsf{DelReq} = 0}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelReq} = 0}_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to be equal to $\Pi_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if party $B$'s output $\mathsf{DelReq}$ is set to 0, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.

\item {\bf Certified everlasting security against $B$.} For every QPT adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting party $B$, there exists a QPT simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ such that for any QPT environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$, and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF^\Del}^{\mathsf{DelRes} = 1}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF^\Del}^{\mathsf{DelRes} = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelRes} = 1}_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to be equal to $\Pi_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if party $A$'s output $\mathsf{DelRes}$ is set to 1, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF^\Del}^{\mathsf{DelRes} = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.
\end{itemize}
\end{definition}

\paragraph{Deletion-composable protocols.} Finally, we consider the composition of protocols that securely realize functionalities with EST. Suppose we have a $\cG^\Del$-hybrid protocol $\Pi^{\cG^\Del}$ for implementing a functionality $\cF^\Del$. We say that $\Pi^{\cG^\Del}$ is \emph{deletion-composable} if the following two properties hold. 
\begin{enumerate}
    \item If the deletion phase of $\cF^\Del$ is never requested, then none of the deletion phases of $\cG^\Del$ are requested.
    \item If the deletion phase of $\cF^\Del$ is accepted by party $A$, meaning that $\mathsf{DelRes} = 1$, then it must be the case that the deletion phases of all the $\cG^\Del$ sub-routines are requested and accepted by $A$.
\end{enumerate}

Then, we can show the following composition theorem, which essentially follows from \cref{thm:composition}.

\begin{theorem}
\label{thm:compose-EST}
Let $\Pi^{\cG^\Del}$ be a deletion-composable protocol that statistically securely realizes\footnote{One could strengthen this theorem to only requiring that $\Pi^{\cG^\Del}$ securely realizes $\cF^\Del$ with EST, but we state the theorem with statistical security for simplicity.} a functionality $\cF^\Del$, and let $\Gamma$ be a protocol that securely implements $\cG^\Del$ with EST. Then $\Pi^{\cG^\Del / \Gamma}$ securely implements $\cF^\Del$ with EST.
\end{theorem}

\begin{proof}
First, the fact that $\Pi^{\cG^\Del/\Gamma}$ computationally securely realizes $\cF^\Del$ follows from directly from \cref{thm:composition} and the fact that both statistical secure realization and secure realization with EST imply computational secure realization. 

Next, statistical security against $A$ in $\Pi^{\cG^\Del/\Gamma}$ when $\mathsf{DelReq} = 0$ also follows directly from \cref{thm:composition} (applied to statistical secure realization), since by the first property of deletion-composability, all of the underlying $\Gamma$ protocols are statistically secure against $A$.

Finally, we argue certified everlasting security against $B$ in $\Pi^{\cG^\Del/\Gamma}$ when $\mathsf{DelRes} = 1$. This does not follow generically from the statement of \cref{thm:composition}. However, it can be shown via essentially the same proof as the proof of \cref{thm:composition}. Starting with $\Pi^{\cG^\Del/\Gamma}$, we replace each invocation of $\Gamma$ with an invocation of $\cG^\Del$ one by one. Conditioned on the deletion phase of $\cG^\Del$ passing, we know that this switch is statistically indistinguishable by the environment, due to the fact that $\Gamma$ securely implements $\cG^\Del$ with EST. Thus, conditioned on the deletion phase of each $\cG^\Del$ being accepted, we know that protocols $\Pi^{\cG^\Del/\Gamma}$ and $\Pi^{\cG^\Del}$ are statistically indistinguishable by the environment. We also know that $\Pi^{\cG^\Del}$ and $\cF^\Del$ are statistically indistinguishable by the environment, by assumption. Thus, by the second property of deletion composability, it follows that $\Pi^{\cG^\Del / \Gamma}$ and $\cF^\Del$ are statistically indistinguishable by the environment conditioned on $\mathsf{DelRes} = 1$, completing the proof.
\end{proof}


%Given such an adversary, and an honest party input $\{x_\secp\}_{\secp \in}$ define the random variable $\Pi_\cF[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ as follows. $\cA_\secp(\sA)$ interacts with $\{P_i(x_{i,\secp})\}_{i \in H}$ during the execution of $\Pi_\cF$. $\cA_\secp$ outputs a quantum state on register $\sA'$, and $\{P_i(x_{i,\secp})\}_{i \in H}$ output classical strings $\{y_i\}_{i \in H}$. The output of the random variable then consists of the quantum state on registers $\sD$ and $\sA'$, along with $\{y_i\}_{i \in H}$. We will also define the random variable $\Pi_\cF^{\mathsf{Hon}}[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ to just consist of $\{y_i\}_{i \in H}$.

%An \emph{ideal-world} protocol $\widetilde{\Pi}_\cF$ for functionality $\cF$ consists of ``dummy'' parties $\widetilde{P}_1,\dots,\widetilde{P}_n$ that have access to an additional ``trusted'' party that implements $\cF$. That is, $\widetilde{P}_1,\dots,\widetilde{P}_n$ each interact directly with $\cF$, which eventually returns outputs to them. We consider the execution of ideal-world protocols in the presence of a simulator, described by a family $\{\cS_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$. 

%Given such a simulator, and a set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, define the random variable $\widetilde{\Pi}_\cF[\cS_\secp,\allowbreak\cD_\secp,\allowbreak\ket{\psi}^{\sA,\sD},\allowbreak\{x_{i,\secp}\}_{i \in H}]$ as follows. $\cS_\secp(\sA)$ interacts with $\{\widetilde{P}_i(x_{i,\secp})\}_{i \in H}$ during the execution of $\widetilde{\Pi}_\cF$. $\cS_\secp$ outputs a quantum state on register $\sA'$, and $\{\widetilde{P}_i(x_{i,\secp})\}_{i \in H}$ output classical strings $\{y_i\}_{i \in H}$. The output of the random variable then consists of the quantum state on registers $\sD$ and $\sA'$, along with $\{y_i\}_{i \in H}$. We will also define the random variable $\widetilde{\Pi}_\cF^{\mathsf{Hon}}[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ to just consist of $\{y_i\}_{i \in H}$.


\subsection{One-sided ideal commitments}\label{subsec:one-sided}

In this section, we construct what we call a \emph{one-sided ideal commitment with EST}. In the following subsection, we define this primitive as well as some underlying building blocks.

\subsubsection{Definitions and building blocks}
A one-sided ideal commitment with EST satisfies full-fledged security with EST against a malicious committer, but not against a malicious receiver. This commitment satisfies the weaker property of certified everlasting hiding against a malicious receiver. These properties are formalized below, where we denote by $\cF_{\mathsf{Com}}^{\mathsf{Del}}$ the commitment ideal functionality from \proref{fig:comIF} augmented with the delete phase from \proref{fig:delPhase}.

\begin{definition}[One-sided ideal commitment with EST]
\label{def:one-sided}

A three-phase (Commit, Reveal, Delete) commitment scheme is a \emph{one-sided ideal commitment with EST} if
\begin{enumerate}
    \item It computationally securely realizes $\cF_{\mathsf{Com}}^{\mathsf{Del}}$ (\cref{def:securerealization}) against a corrupt committer $C$.
    \item It satisfies statistical security against a corrupt committer $C$ that does not initiate deletion (first part of \cref{def:security-with-EST}). 
    
    %That is, there exists a polynomial $p(\cdot)$ such that for every (potentially unbounded) adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting $C$, there exists a simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ with size at most $p(\secp)$ times the of size of $\{\cA_\secp\}_{\secp \in \bbN}$, such that for any (potentially unbounded) environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$ and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF_{\mathsf{Com}}}^{\mathsf{DelReq} = 0}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF_{\mathsf{Com}}}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelReq} = 0}_{\cF_{\mathsf{Com}}}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to equal $\Pi_{\cF_{\mathsf{Com}}}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if the honest party output $\mathsf{DelReq}$ is set to 0, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF_{\mathsf{Com}}}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.
    %security with EST (\cref{def:security-with-EST}) against adversaries that corrupt the committer $C$,
    \item It satisfies correctness of deletion (\cref{def:correctness-deletion}) and it satisfies certified everlasting hiding (\cref{def:CEH}) against adversaries that corrupt the receiver $R$.
\end{enumerate}
\end{definition}

To construct this object, our building block will be a \emph{computationally-hiding statistically-efficiently-extractable} (CHSEE) commitment, which is a two-phase (Commit, Reveal) commitment that satisfies correctness (\cref{def:correctness-decommitment}), standard computational hiding (\cref{def:comp-hiding}), and the following notion of binding. Note that this is similar to \cref{def:SB}, except that the extractor must be \emph{efficient}.

\begin{definition}[Statistical efficient extractability]\label{def:SEE}
A commitment scheme satisfies \emph{statistical efficient extractability} if for any QPT adversary $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase, there exists a QPT extractor $\cE = \{\cE_\secp\}_{\secp \in \bbN}$, such that for any initial advice $\{\ket{\psi_\secp}^{\sAux,\sC^*}\}_{\secp \in \bbN}$ and any QPT adversary $\{\cC^*_{\Rev,\secp}\}_{\secp \in \bbN}$ in the Reveal phase,
\[\TD\left(\Real^{\cC^*}_\secp,\Ideal^{\cC^*,\cE}_\secp\right) = \negl(\secp),\] where $\Real^{\cC^*}_\secp$ and $\Ideal^{\cC^*,\cE}_\secp$ are defined as follows.

\begin{itemize}
    \item $\Real_\secp^{\cC^*}$: Execute the Commit phase $(\sC^*,\sR) \gets \Com\langle \cC^*_{\Com,\secp}(\sC^*),\cR_{\Com,\secp}\rangle$, where $\cC^*_{\Com,\secp}$ has as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$. Execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the committer's final state on register $\sC^*$. Output $(\mu,\sC^*,\sAux)$, which includes the $\sAux$ register of the original advice state.
    \item $\Ideal_\secp^{\cC^*,\cE}$: Run the extractor $(b^*,\sC^*,\sR) \gets \cE_\secp(\sC^*)$, where the extractor takes as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$, and outputs a bit $b^*$ and a state on registers $\sC^*,\sR$. Next, execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the committer's final state on register $\sC^*$. If $\mu \in \{\bot,b^*\}$ output $(\mu,\sC^*,\sAux)$, and otherwise output a special symbol $\Fail$.
\end{itemize}

\end{definition}

\begin{importedtheorem}[\cite{BCKM2021}]\label{thm:CHSEE}
There exists a construction of CHSEE commitments that makes black-box use of any computationally-hiding statistically-binding commitment (\cref{def:comp-hiding} and \cref{def:SB}).\footnote{In \cite{BCKM2021}, a different notion of statistical binding for the underlying commitment was used, but it was noted by \cite{cryptoeprint:2021:1663} that the extractor-based definition of statistical binding suffices.}
\end{importedtheorem}
These are implied by OT with statistical security against one party, which was constructed in~\cite{BCKM2021}, based on the black-box use of computationally-hiding statistically-binding commitments.
Alternatively, CHSEE commitments can be obtained more directly by plugging in the statistically-equivocal computationally-extractable commitments from \cite{BCKM2021} into the extractability compiler \cite[Section 5]{BCKM2021}. Furthermore, this implies that CHSEE commitments can be based on the black-box use of one-way functions~\cite{BCKM2021} or pseudo-random quantum states~\cite{cryptoeprint:2021:1691,cryptoeprint:2021:1663}. 
%\end{remark}

\subsubsection{Construction}
We construct one-sided ideal commitments with EST from CHSEE commitments in \proref{fig:one-sided}. We note that constructing one-sided ideal commitments with EST does not just follow immediately from applying our certified deletion compiler, as in our construction of commitments with certified everlasting hiding from statistically-binding commitments in \cref{subsec:com-ZK}. The reason is that we need indistinguishability between the real and ideal worlds to hold against a malicious committer \emph{even if the delete phase is run}. To satisfy this property, we actually use additional invocations of the CHSEE commitment going in the ``opposite'' direction during the Delete phase of \proref{fig:one-sided}.


Next, we prove the following theorem.
\begin{theorem}\label{thm:one-sided}
\proref{fig:one-sided} is a one-sided ideal commitment with EST (according to \cref{def:one-sided}).
\end{theorem}
The theorem follows by combining Lemmas \ref{lem:os-id-one}, \ref{lem:os-id-two}, \ref{lem:os-idthree} and \ref{lem:os-idfour} proved below.

\protocol{\proref{fig:one-sided}: One-sided ideal commitment with EST}{Construction of one-sided ideal commitment with EST, from a CHSEE commitment.}{fig:one-sided}{
Ingredients: a CHSEE commitment $(\Com,\Rev)$ \\
Parties: committer $C$ with input $b \in \{0,1\}$ and receiver $R$.\\

\underline{\textbf{Commit phase}} 
\begin{itemize}
    \item $C$ samples $x,\theta \gets \{0,1\}^\secp$.
    \item $C$ and $R$ execute $\sC_\theta,\sR_\theta \gets \Com\langle C(\theta),R\rangle$.
    \item $C$ and $\cR$ execute $\sC_b,\sR_b \gets \Com\langle C(b \oplus \bigoplus_{i:\theta_i = 0} x_i),R\rangle$.
    \item $C$ sends $\ket{x}_\theta$ to $R$ on register $\sX$.
\end{itemize}

\underline{\textbf{Reveal phase}} 
\begin{itemize}
    \item $C$ and $R$ execute $\theta \gets \Rev\langle C(\sC_\theta),R(\sR_\theta)\rangle$.
    \item $C$ and $R$ execute $b' \gets \Rev\langle C(\sC_b),R(\sR_b)\rangle$.
    \item  $R$ measures the qubits $i$ of register $\sX$ such that $\theta_i = 0$ to obtain $x_i$, and then outputs $b' \oplus \bigoplus_{i:\theta_i = 0} x_i$.
\end{itemize}

\underline{\textbf{Delete phase}\footnote{Note that both the Reveal phase and the Delete phase require $C$ and $R$ to run $\Rev\langle C(\sC_\theta),R(\sR_\theta)\rangle$.
So if the Reveal phase has already been run, we can instruct $R$ to abort if a deletion is requested, since we don't require any correctness of deletion or everlasting security after Reveal.}} 
\begin{itemize}
    \item $R$ measures all qubits of register $\sX$ in the Hadamard basis to obtain a string $x' \in \{0,1\}^\secp$.
    \item $R$ and $C$ execute $\secp$ Commit phases of $\Com$, with $R$ as the committer, committing bit-by-bit to $x'$: $\sR_{x',i},\sC_{x',i} \gets \Com \langle R(x'_i),C\rangle$.
    \item $C$ and $R$ execute $\theta \gets \Rev\langle C(\sC_\theta),R(\sR_\theta)\rangle$.
    \item $R$ and $C$ execute the Reveal phase of $\Com$ for each $i$ such that $\theta_i = 1$: $x'_i \gets \Rev \langle R(\sR_{x',i}),C(\sC_{x',i})\rangle$.
    \item $C$ accepts (outputs 1) if $x'_i = x_i$ for all $i$ such that $\theta_i = 1$.
\end{itemize}

}

%Next, we define the notion of CHSEE commitments with \emph{everlasting security transfer} (EST). These are three-phase (Commit, Delete, Open) commitments (syntax is defined in \cref{subsec:com-ZK}) that are similar to commitments with certified everlasting hiding. That is, they satisfy correctness (\cref{def:correctness-decommitment} and \cref{def:correctness-deletion}) and certified everlasting hiding (\cref{def:CEH}). They also satisfy a \emph{strengthening} of statistical efficient extractability (\cref{def:SEE}) that remains meaningful \emph{even if the deletion phase is run}. In particular, if the Delete phase is run, the view produced by the extractor remains \emph{computationally} (instead of statistically) indistinguishable from the real view. Note that by itself, \cref{def:SEE} says nothing about the view when the Delete phase is run, so we must specify a new definition, which we call statistical efficient extractability with EST.

%\begin{definition}[Statistical efficient extractability with EST]
%A commitment scheme satisfies \emph{statistical efficient extractability with EST} if the following hold, where $\{\ket{\psi_\secp}^{\sAux,\sC^*}\}_{\secp \in \bbN}$ is any non-uniform advice.


%exists a polynomial $p(\secp)$ such that for any (potentially unbounded) adversary $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase and initial advice $\{\ket{\psi_\secp}^{\sAux,\sC^*}\}_{\secp \in \bbN}$, there exists an extractor $\cE = \{\cE_\secp\}_{\secp \in \bbN}$ with running time at most $p(\secp)$ times the running time of $\cC^*_{\Com,\secp}$, such that the following hold.

%First, for any unbounded adversary  $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase, there exists an unbounded extractor $\{\cE_\secp\}_{\secp \in \bbN}$ such that for every unbounded adversary $\{\cC^*_{\Rev,\secp}\}_{\secp \in \bbN}$ in the Reveal phase,
%\[\TD\left(\EVREAL^{\cC^*}_\secp,\EVIDEAL^{\cC^*,\cE}_\secp\right) = \negl(\secp),\] where $\EVREAL^{\cC^*}_\secp$ and $\EVIDEAL^{\cC^*,\cE}_\secp$ are defined as follows.

%\begin{itemize}
    %\item $\EVREAL_\secp^{\cC^*}$: Execute the Commit phase $(\sC^*,\sR) \gets \Com\langle \cC^*_{\Com,\secp}(\sC^*),\cR_{\Com,\secp}\rangle$, where $\cC^*_{\Com,\secp}$ has as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$. Execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the committer's final state on register $\sC^*$. Output $(\mu,\sC^*,\sAux)$, which includes the $\sAux$ register of the original advice state.
    %\item $\EVIDEAL_\secp^{\cC^*,\cE}$: Run the extractor $(b^*,\sC^*,\sR) \gets \cE_\secp(\sC^*)$, where the extractor takes as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$, and outputs a bit $b^*$ and a state on registers $\sC^*,\sR$. Next, execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the committer's final state on register $\sC^*$. If $\mu \in \{\bot,b^*\}$ output $(\mu,\sC^*,\sAux)$, and otherwise output a special symbol $\Fail$.
%\end{itemize}

%Second, for any QPT adversary $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase, there exists a QPT extractor $\{\cE_\secp\}_{\secp \in \bbN}$, such that for any QPT adversary $\{\cC^*_{\Del,\secp}\}_{\secp \in \bbN}$ in the Delete phase, there is a QPT simulator $\cS = \{\cS_\secp\}_{\secp \in \bbN}$ such that for any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, it holds that \[\bigg|\Pr\left[\cD_\secp\left(\CREAL_\secp^{\cC^*}\right) = 1\right] - \Pr\left[\cD_\secp\left(\CIDEAL_\secp^{\cC^*,\cE,\cS}\right) = 1\right]\bigg| = \negl(\secp),\] where $\CREAL_\secp^{\cC^*}$ and $\CIDEAL_\secp^{\cC^*,\cE,\cS}$ are defined as follows.
%\begin{itemize}
    %\item $\CREAL_\secp^{\cC^*}$: Execute the Commit phase $(\sC^*,\sR) \gets \Com\langle \cC^*_{\Com,\secp}(\sC^*),\cR_{\Com,\secp}\rangle$, where $\cC^*_{\Com,\secp}$ has as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$. Execute $d \gets \Del\langle \cC^*_{\Del,\secp}(\sC^*),\cR_{\Del,\secp}(\sR)\rangle$ to obtain $d$ along with a final committer's state on register $\sC^*$. Output $(d,\sC^*,\sAux)$.
    %\item $\CIDEAL_\secp^{\cC^*,\cE,\cS}$: Run the extractor $(b^*,\sC^*,\sR) \gets \cE_\secp(\sC^*)$, where the extractor takes as input the $\sC^*$ register of $\ket{\psi_\secp}^{\sAux,\sC^*}$, and outputs a bit $b^*$ and a state on registers $\sC^*,\sR$. Run $(d,\sC^*) \gets \cS_\secp(\sC^*,\sR)$, and output $(d,\sC^*,\sAux)$.
%\end{itemize}



%\end{definition}


\subsubsection{Security against a corrupt committer}
\begin{lemma}
\label{lem:os-id-one}
\proref{fig:one-sided} computationally securely realizes $\cF_{\mathsf{Com}}^{\mathsf{Del}}$ (\cref{def:securerealization}) against a corrupt committer $C$. That is, for every QPT committer $\{\cC^*_\secp \coloneqq (\cC^*_{\secp,\Com},\cC^*_{\secp,\Rev},\cC^*_{\secp,\Del})\}_{\secp \in \bbN}$, there exists a QPT simulator $\{\cS_\secp \coloneqq (\cS_{\secp,\Com},\cS_{\secp,\Rev},\cS_{\secp,\Del})\}_{\secp \in \bbN}$, such that for any QPT environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\cZ_{\secp,2},\cZ_{\secp,3})\}_{\secp \in \bbN}$, polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, and QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, it holds that \[\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Com^\Del}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = 1\right] - \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Com^\Del}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = 1\right]\bigg| = \negl(\secp).\] 
\end{lemma}



\begin{lemma}
\label{lem:os-id-two}
\proref{fig:one-sided} satisfies statistical security against a corrupt committer $C$ that does not initiate deletion. That is, there exists a polynomial $p(\cdot)$ such that for every (potentially unbounded) committer $\{\cC^*_\secp \coloneqq (\cC^*_{\Com,\secp},\cC^*_{\Rev,\secp},\cC^*_{\Del,\secp})\}_{\secp \in \bbN}$, there exists a simulator $\{\cS_\secp \coloneqq (\cS_{\secp,\Com},\cS_{\secp,\Rev},\cS_{\secp,\Del})\}_{\secp \in \bbN}$ with size at most $p(\secp)$ times the of size of $\cC^*$, such that for any (potentially unbounded) environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\cZ_{\secp,2},\cZ_{\secp,3})\}_{\secp \in \bbN}$ and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelReq} = 0}_{\cF_{\mathsf{Com}}^\Del}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to equal $\Pi_{\cF_{\mathsf{Com}}^\Del}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if the receiver's output $\mathsf{DelReq}$ is set to 0, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.
\end{lemma}


\begin{proof} (of Lemmas \ref{lem:os-id-one} and \ref{lem:os-id-two})
We define a simulator $\cS = (\cS_\Com,\cS_\Rev,\cS_\Del)$ based on any adversary $\cC^* = (\cC^*_{\Com}, \cC^*_{\Rev}, \cC^*_{\Del})$ that will suffice to prove both lemmas. We have dropped the dependence on $\secp$ for notational convenience.
\begin{enumerate}
    \item {\bf Commit Phase.} $\cS_\Com$ does the following.
    \begin{itemize}
        \item Run the CHSEE extractor $(\theta^*,\sC^*,\sR_\theta) \gets \cE_\secp[\cC^*_{\Com,\theta}](\sC^*)$, where the extractor is defined based on the part of $\cC^*_\Com$ that interacts in the commitment to $\theta$. It takes as input $\cC^*_\Com$'s private state register $\sC^*$, and outputs a sequence of committed bits $\theta^*$ and a state on $\sC^*,\sR_\theta$.
        \item Next, run the CHSEE extractor $(d^*,\sC^*,\sR_b) \gets \cE_\secp[\cC^*_{\Com,b}](\sC^*)$, where the extractor is defined based on the part of $\cC^*_\Com$ that interacts in the commitment to $b \oplus \bigoplus_{i: \theta_i = 0} x_i$. It takes as input $\cC^*$'s private state register $\sC^*$, and outputs a committed bit $d^*$ and a state on registers $\sC^*,\sR_b$.
        \item Keep running $\cC^*_\Com$ until it outputs a state on register $\sX$.
        \item Measure the qubits $i$ of register $\mathsf{X}$ such that $\theta^*_i = 0$ to obtain $x^*_i$, and then send 
        $(\text{Commit}, \mathsf{sid}, b^*)$ where
        $b^* = d^* \oplus \bigoplus_{i:\theta^*_i = 0} x^*_i$ to the ideal functionality.
    \end{itemize}
    \item {\bf Reveal Phase.}
    $\cS_\Rev$ does the following.
    \begin{itemize}
        \item Execute the Reveal phase of CHSEE to obtain $\theta' \leftarrow \Rev\langle \cC^*_{\Rev,\theta}(\sC^*),R(\sR_\theta)\rangle$(and update the register $\sC^*$).
        \item Execute the Reveal phase of CHSEE to obtain $d' \leftarrow \Rev\langle \cC^*_{\Rev,b}(\sC^*),R(\sR_b)\rangle$ (and update the register $\sC^*$).
        \item If $\theta^* = \theta'$ and $d^* = d'$ then send $(\text{Reveal}, \mathsf{sid})$ to the ideal functionality.
    \end{itemize}
    \item {\bf Delete Phase.}
    If $\cC^*_\Del$ initializes the Delete phase, $\cS_\Del$ sends $(\mathsf{DelRequest},\mathsf{sid})$ to the ideal functionality, and upon obtaining $(\mathsf{DelResponse},\mathsf{sid})$, it does the following.
    %$\cS_3$ does the following if $\sC^*$ makes a delete request.
    \begin{itemize}
        \item For every $i$ such that $\theta^*_i = 1$, measure the $i^{th}$ qubit of register $\sX$ in the Hadamard basis to obtain $x'_i$.
        For all $i$ such that $\theta^*_i \in \{0,\bot\}$, set $x'_i = 0$.
        \item Execute $\lambda$ commit phases of $\Com$, with the simulator as the committer, committing bit-by-bit to $x'$.
        \item Execute the Reveal phase of $\cC^*$'s commitments to $\theta$ to obtain $\theta' \leftarrow \Rev\langle \cC^*_{\Del,\theta}(\sC^*),R(\sR_\theta)\rangle$ (and update the register $\sC^*$), where $\cC^*_{\Del,\theta}$ is the part of $\cC^*_\Del$ that interacts in the reveal phase of the commitment to $\theta$.
        \item If $\theta' \neq \theta^*$, abort. Otherwise, execute with $\cC^*$ the Reveal phase of commitments to $x'$ restricted to indices $i \in [\secp]$ such that $\theta'_i = 
        1$.
    \end{itemize}
\end{enumerate}
It is straightforward to see that the simulator runs in quantum polynomial time as long as $\cC^*$ runs in quantum polynomial time.

Statistical indistinguishability between the real and ideal distributions at the end of the Commit Phase or the Reveal Phase follows directly from \cref{def:SEE}, thereby proving Lemma \ref{lem:os-id-two}.

Furthermore, in the Delete phase, simulator and receiver strategies are identical on indices where $\theta^*_i = 1$. The only difference between these strategies is that the simulator commits to $0$ when $\theta^*_i = 0$ whereas the receiver commits to outcomes of measurements of the $i^{th}$ qubit of register $\sX$ in the Hadamard basis. Now, the Reveal phase for these commitments are only run when $\theta' = \theta^*$, and only restricted to indices $i \in [\lambda]$ such that $\theta_i' = 1$. Thus, computational indistinguishability during the Delete phase follows from a reduction to the computational hiding of $\Com$. This proves \cref{lem:os-id-one}.
\end{proof}

\subsubsection{Security against a corrupt receiver}
\begin{lemma}
\label{lem:os-idthree}
\proref{fig:one-sided} satisfies correctness of deletion (\cref{def:correctness-deletion}). 
\end{lemma}
\begin{proof}
This follows immediately from the description of the scheme.
\end{proof}

\begin{lemma}
\label{lem:os-idfour}
\proref{fig:one-sided} satisfies certified everlasting hiding (\cref{def:CEH}) against adversaries that corrupt the receiver $R$.
\end{lemma}
\begin{proof}
The first property of certified everlasting hiding follows immediately from the computational hiding of CHSEE and the fact that the delete phase is completely independent of the committed bit $b$.


The second property follows from the computational hiding of CHSEE and \cref{thm:main} by setting $\cZ_\secp(\theta)$ and $\cA_\secp$ as follows, based on any non-uniform corrupt receiver $\cR^* = \{\cR^*_{\secp,\Com},\cR^*_{\secp,\Del},\ket{\psi_\secp}\}_{\secp \in \bbN}$.

\begin{itemize}
    \item $\cZ_\secp(\theta)$ initializes registers $(\sR^*,\sD^*)$ with $\ket{\psi_\secp}$, runs $(\sC_\theta,\sR^*) \gets \Com\langle C(\theta),\cR^*_{\secp,\Com}(\sR^*)\rangle$ with the first part of $\cR^*_{\Com,\secp}$, and outputs the resulting state on register $\sR^*$.
    \item $\cA_\secp$ receives $\ket{x}_\theta, b \oplus \bigoplus_{i: \theta_i = 0} x_i,$ and the state on register $\sR^*$. It first runs $(\sC_b,\sR^*) \gets \Com\langle C(b \oplus \bigoplus_{i: \theta_i = 0} x_i),\cR^*_{\secp,\Com}(\sR^*)\rangle$ with the remaining part of $\cR^*_{\secp,\Com}$. Then, it sends $\ket{x}_\theta$ to $\cR^*_{\secp,\Com}$. Next, it runs $\cR^*_{\secp,\Del}$ until the beginning of the part where $\cR^*_{\secp,\Del}$ is supposed to commit to $x'$. At this point, it runs the extractor $\cE_\secp(\sR^*)$ for $\Com$, which outputs a certificate $x'$ and a left-over quantum state on register $\sR^*$.
\end{itemize}

%To show the second property, consider any non-uniform corrupt receiver $\cR^* = \{\cR^*_{\Com,\secp},\cR^*_{\Del,\secp},\ket{\psi}\}_{\secp \in \bbN}$. We appeal to \cref{thm:main}, and set $\cZ(m)$ for $m \in \{0,1\}^*$ to be the distribution that first initializes $\cR^*_{\Com,\secp}$ with the $\sR^*$ register of $\ket{\psi}$, runs 

%outputs a commitment according to $\Com$ to bit $b$, and the adversary $\cA$ for \cref{thm:main} as follows.

%$\cA$ on input $\ket{x}_\theta, b', \cZ(\theta)$ executes committer strategy for \proref{fig:one-sided} with state $\ket{x}_\theta, \cZ(\theta)$ and $\Com(b')$ in the commit phase, and runs the extractor $\cE_\secp(\sR^*)$ for $\Com$ on the $\secp$ commitments generated by $R$ in the delete phase to obtain and output certificate $x'$. 

Note that the delete phase succeeds in the experiment $\EVEXP_\secp^{\cR^*}(b)$ iff for every $i$ where $\theta_i = 1$, $x'_i = x_i$, where the $x'_i$ are opened by $\cR^*_{\secp,\Del}$. Also, by statistical efficient extractability of Com, the $\{x'_i\}_{i: \theta_i = 1}$ output by $\cE_\secp$ are equal to the $\{x'_i\}_{i: \theta_i = 1}$ opened by $\cR^*_{\secp,\Del}$, except with negligible probability. Thus, \cref{thm:main} implies that



\[\TD\left(\EVEXP_\secp^{\cR^*}(0),\EVEXP_\secp^{\cR^*}(1)\right) = \negl(\secp).\]
This completes the proof of the lemma.
\end{proof}

\subsection{Ideal commitments}\label{subsec:ideal}

In this section, we show how to generically upgrade a one-sided ideal commitment with EST to a full-fledged ideal commitment with EST. Our construction, which is given in \proref{fig:ideal}, is essentially the ``equivocality compiler'' from \cite{BCKM2021} with an added Delete phase.

\begin{theorem}\label{thm:ideal}
\proref{fig:ideal} securely realizes the commitment ideal functionality with EST (according to \cref{def:security-with-EST}).
\end{theorem}
The theorem follows by combining Lemmas \ref{lem:ts-id-one}, \ref{lem:ts-id-two}, \ref{lem:ts-idthree} and \ref{lem:ts-idfour} proved below.

\protocol
{\proref{fig:ideal}: Ideal commitment with EST}
{Ideal commitment with EST, from a one-sided ideal commitment with EST.}
{fig:ideal}
{
Ingredients: a one-sided ideal commitment with EST $(\Com,\Rev,\Del)$.\\
Parties: committer $C$ with input $b \in \{0,1\}$ and receiver $R$.\\

\vspace{-4mm}
\underline{\textbf{Commit phase}}
\begin{enumerate}
\item $C$ samples uniformly random bits $a_{i,j}$ for $i \in [\lambda]$ and $j \in \{0,1\}$.
\item For every $i \in [\lambda]$, $C$ and $R$ sequentially perform the following steps.
\begin{enumerate}
\item $C$ and $R$ execute four Commit phases sequentially, namely:
\begin{itemize}
    \item $\sC_{i,0,0}, \sR_{i,0,0} \leftarrow \Com \langle C(a_{i,0}), R \rangle$,
    \item $\sC_{i,0,1}, \sR_{i,0,1} \leftarrow \Com \langle C(a_{i,0}), R \rangle$, 
    \item $\sC_{i,1,0}, \sR_{i,1,0} \leftarrow \Com \langle C(a_{i,1}), R \rangle$,
    \item $\sC_{i,1,1}, \sR_{i,1,1} \leftarrow \Com \langle C(a_{i,1}), R \rangle$.
\end{itemize}
\item $R$ sends a choice bit $c_i \leftarrow \{0,1\}$.
\item $C$ and $R$ execute two Reveal phases, obtaining the opened bits:
\begin{itemize}
\item $u \leftarrow \Rev \langle C(\sC_{i,c_i,0}), R(\sR_{i,c_i,0}) \rangle$,
\item $v \leftarrow \Rev \langle C(\sC_{i,c_i,1}), R(\sR_{i,c_i,1}) \rangle$. 
\end{itemize}
If $u \neq v$, $R$ aborts. Otherwise, $C$ and $R$ continue.
\end{enumerate}
\vspace{-4mm}
\item For $i \in [\lambda]$, 
$C$ sets $b_i = b \oplus a_{i, 1-c_i}$ and
sends $\{b_i\}_{i \in [\lambda]}$ to $R$.
\end{enumerate}

\vspace{-2mm}
\underline{\textbf{Reveal phase}}
\vspace{-2mm}
\begin{enumerate}
    \item $C$ sends $b$ to $R$. In addition,
    \vspace{-2mm}
    \begin{enumerate}
    \item For $i \in [\lambda]$, 
    $C$ picks $\alpha_i \gets \{0,1\}$ and sends it to $\cR$. 
    \item $C$ and $R$ execute  $a_i' \leftarrow \Rev \langle C(\sC_{i,1-c_i,\alpha_i}), R(\sR_{i,1-c_i,\alpha_i}) \rangle$.
    \end{enumerate}
    \vspace{-4mm}
    \item $R$ accepts and outputs $b$ if for every $i \in [\lambda]$, $a_i' = b \oplus b_i$.
\end{enumerate}

\vspace{-2mm}
\underline{\textbf{Delete phase}}
\vspace{-2mm}
\begin{enumerate}
    \item For every $i \in [\secp]$, $C$ and $R$ sequentially perform the following steps.
    \vspace{-2mm}
    \begin{enumerate}
        \iffalse{
        \item If Reveal has not been performed, set $\beta_i = 0$, and otherwise set $\beta_i = 1-\alpha_i$.
        \item $C$ and $R$ execute $d_i \gets \Del\langle C(\sC_{i,1-c_i,\beta_i},R(\sR_{i,1-c_i,\beta_i}))$.
        }\fi
        \item If Reveal was performed, execute $D_i \gets \Del\langle C(\sC_{i,1-c_i,1-\alpha_i},R(\sR_{i,1-c_i,1-\alpha_i})\rangle$.
        \item Otherwise, set $D_i = D_{i,0} \wedge D_{i,1}$ where
        $D_{i,0} \gets \Del\langle C(\sC_{i,1-c_i,0},R(\sR_{i,1-c_i,0})\rangle$ and $D_{i,1} \gets \Del\langle C(\sC_{i,1-c_i,1},R(\sR_{i,1-c_i,1})\rangle$.
    \end{enumerate}
    \item If $D_i = 1$ for all $i \in [\secp]$, then $C$ outputs 1.
\end{enumerate}
}




\subsubsection{Security against a corrupt committer}

\begin{lemma}
\label{lem:ts-id-one}
\proref{fig:ideal} computationally securely realizes $\cF_{\mathsf{Com}}^{\mathsf{Del}}$ (\cref{def:securerealization}) against a corrupt committer $C$.
\end{lemma}


\begin{lemma}
\label{lem:ts-id-two}
\proref{fig:ideal} satisfies statistical security against a corrupt committer $C$ that does not initiate deletion. That is, there exists a polynomial $p(\cdot)$ such that for every (potentially unbounded) adversary $\{\cC^*_\secp \coloneqq (\cC^*_{\secp,\Com},\cC^*_{\secp,\Rev},\cC^*_{\secp,\Del})\}_{\secp \in \bbN}$ corrupting $C$, there exists a simulator $\{\cS_\secp \coloneqq (\cS_{\secp,\Com},\cS_{\secp,\Rev},\cS_{\secp,\Del})\}_{\secp \in \bbN}$ with size at most $p(\secp)$ times the of size of $\{\cC^*_\secp\}_{\secp \in \bbN}$, such that for any (potentially unbounded) environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\cZ_{\secp,2},\cZ_{\secp,3})\}_{\secp \in \bbN}$ and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelReq} = 0}_{\cF_{\mathsf{Com}}^\Del}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to equal $\Pi_{\cF_{\mathsf{Com}}^\Del}[\cC^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if the receiver's output $\mathsf{DelReq}$ is set to 0, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelReq} = 0}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.
\end{lemma}

\begin{proof} (of Lemmas \ref{lem:ts-id-one} and \ref{lem:ts-id-two})\\

\noindent {\bf \underline{The Simulator.}} The simulator $(\cS_{\Com},\cS_{\Rev}, \cS_{\Del})$ is defined as follows. 
\begin{enumerate}
    \item {\bf Commit Phase.} $\cS_\Com$ does the following.
    \begin{itemize}
        \item For all $i \in [\secp]$,
        \begin{itemize}
            \item Execute four sequential simulated Commit phases where the simulator for the commitment $\Com$ is run on the part of the committer $\cC^*_\Com$ participating in each of the four sequential sessions. Denote the bit output by the simulator in each session by $(d_{i,0,0},d_{i,0,1},d_{i,1,0},d_{i,1,1})$.
            \item Sample and send choice bit $c_i \leftarrow \{0,1\}$ to $\cC^*_\Com$.
            \item Execute two simulated Reveal phases where the simulator is run on the part of the committer $\cC^*_\Com$ corresponding to sessions $(i, c_i, 0)$ and $(i, c_i, 1)$. If the simulator outputs $(\text{Reveal},\mathsf{sid})$ for both sessions and $d_{i,c_i,0} = d_{i,c_i,1}$, continue, and otherwise abort.
        \end{itemize}
        \item Obtain $\{b_i\}_{i \in [\secp]}$ from $\cC^*_\Com$.
        Fix $b^*$ to be the most frequently occuring bit in $\{b_i \oplus d_{i,1-c_i,0}\}_{i \in [\secp]}$. Send $(\text{Commit},\mathsf{sid},b^*)$ to the commitment ideal functionality.
    \end{itemize}
    \item {\bf Reveal Phase.}
    $\cS_\Rev$ does the following.
    \begin{enumerate}
        \item Obtain $b$ from $\cC^*_\Rev$. Additionally, for $i \in [\secp]$,
        \begin{itemize}
            \item Obtain $\alpha_i$ from $\cC^*_\Rev$.
            \item Execute the simulated Reveal phase where simulator is run on the part of the committer $\cC^*_\Rev$ corresponding to session $(i, 1-c_i, \alpha_i)$. If $\cS_\Rev$ outputs $(\text{Reveal},\mathsf{sid})$ and  $d_{i,1-c_i,\alpha_i} = b \oplus b_i$, continue. Otherwise, abort.
        \end{itemize}
        \item Send $(\text{Reveal},\mathsf{sid})$ to the ideal functionality.
    \end{enumerate}
    \item {\bf Delete Phase.}
   If $\cC^*$ makes a delete request, $\cS_\Del$ sends $(\mathsf{DelRequest},\mathsf{sid})$ to the ideal functionality, and upon obtaining $(\mathsf{DelResponse},\mathsf{sid})$, it does the following.
   \begin{itemize}
       \item If the Reveal phase was executed, then for every $i \in [\secp]$, run the simulator on the part of $\cC^*_\Del$ that interacts in the delete phase of session $(i, 1-c_i, 1-\alpha_i)$.
       \item If the Reveal phase was not executed, then for every $i \in [\secp]$, run the simulator on the part of $\cC^*_\Del$ that interacts (sequentially) in the delete phases of sessions $(i, 1-c_i, 0)$ and $(i, 1-c_i, 1)$.
   \end{itemize}
\end{enumerate}

\noindent{\bf \underline{Analysis.}\\}

Note that there are a total of $4\lambda$ commitment sessions. Denote the real experiment by $\mathsf{Hybrid}_{0,1,1}$.
For each $i \in [\lambda], j \in [0,1], k \in [0,1]$, define $\mathsf{Hybrid}_{i,j,k}$ to be the distribution obtained as follows.
%, and note that $\mathsf{Hybrid}_{\lambda, 1, 1}$ is the $\mathsf{Ideal}$ distribution. 

\paragraph{Commit Phase.}
Set $\counternew = 1$, $\mathsf{DelReq}= 0$ and do the following:
\begin{enumerate}
    \item If $\counternew = \lambda + 1$, obtain $\{b_i\}_i$ from $\cC^*_\Com$ and end.
    \item If $\counternew < i$,
    \begin{enumerate}
    \item Execute four sequential simulated Commit phases where the simulator for the commitment $\Com$ is run on the part of the committer $\cC^*_\Com$ participating in each of the four sequential sub-sessions.
    Denote the bit output by the the simulator in each sub-session respectively by $(d_{\counternew,0,0},d_{\counternew,0,1},d_{\counternew,1,0},d_{\counternew,1,1})$.
    \item Sample and send choice bit $c_\counternew \leftarrow \{0,1\}$ to $\cC^*_\Com$.
    \item Execute two simulated Reveal phases where the simulator is run on the part of the committer $\cC^*_\Com$ corresponding to sub-sessions $(\counternew, c_\counternew, 0)$ and $(\counternew, c_\counternew, 1)$. If the simulator outputs $(\text{Reveal},\mathsf{sid})$ for both sub-sessions and $d_{\counternew,c_\counternew,0} = d_{\counternew,c_\counternew,1}$, continue, and otherwise abort.
    \end{enumerate}
    \item If $\counternew = i$, 
    \begin{enumerate}
    %Execute four sessions sequentially, namely:
    %, set $(x,y) = (0,0)$ and do:
    %\begin{itemize}
        \item 
        %If $(j,k) = (0,0)$, set $\bx_{0,0}, \by_{0,0} \leftarrow \extcommit \langle \sC^*(\brho), \cR \rangle$.
        Do the same as above (i.e., for the case $\counternew <i$) except execute simulated Commit (and if needed, Reveal) phases where the simulator for the commitment $\mathsf{Com}$ is run on the part of the committer $\cC^*_\Com$ participating in  sequential sub-sessions
        $(\counternew,j',k')$ whenever $(j',k') \leq (j,k)$ where we have $(0,0) \leq (0,1) \leq (1,0) \leq (1,1)$ for transitive relation $\leq$. But for $(j',k') \not \leq (j,k)$, follow honest receiver strategy in sub-session $(i,j',k')$.
    \end{enumerate}
    \item If $\counternew > i$,
    \begin{enumerate}
        \item Execute honest receiver strategy for all Commit (and Reveal) phases for all sessions $(i, j', k')$ for every $j', k' \in \{0,1\}^2$.
    \end{enumerate}
    %\item Obtain $\{b_i\}_{i \in [\secp]}$ from $\cC^*_\Com$.
    \item Set $\gamma = \gamma + 1$.
\end{enumerate}
%
\paragraph{Reveal Phase.}
    Do the following.
    \begin{itemize}
        \item Obtain $b$ from $\cC^*_\Rev$. Additionally, for $\counternew \in [\secp]$,
        \begin{itemize}
            \item Obtain $\alpha_\gamma$ from $\cC^*_\Rev$.
            \item If $\counternew < i$, execute the simulated Reveal phase where the simulator is run on the part of the committer $\cC^*_\Rev$ corresponding to session $(\gamma, 1-c_\gamma, \alpha_\gamma)$.
            If the simulator outputs $(\text{Reveal},\mathsf{sid})$ and if $d_{\gamma,1-c_\gamma,\alpha_\gamma} = b \oplus b_i$, continue. Otherwise, abort.
            \item If $\gamma = i$, do the same as above when $(1-c_\gamma,\alpha_\gamma) \leq (j,k)$ otherwise follow honest receiver strategy.
            If $\gamma > i$, follow honest receiver strategy.
        \end{itemize}
        \item Set $b^* = b$. %and send $(\text{Reveal},\mathsf{sid})$ to the ideal functionality.
    \end{itemize}



\noindent {\bf Delete Phase.}
   If $\cC^*$ makes a delete request, send $(\mathsf{DelRequest},\mathsf{sid})$ to the ideal functionality, and upon obtaining $(\mathsf{DelResponse},\mathsf{sid})$, do the following.
   \begin{itemize}
        \item If the Reveal phase was executed, then
        \begin{itemize}
           \item For every $\gamma \in [1,i-1]$, run the simulator on the part of $\cC^*_\Del$ that interacts in the delete phase of session $(\gamma, 1-c_\gamma, 1-\alpha_\gamma)$.
           \item For $\gamma = i$, if $(1-c_\gamma, 1-\alpha_\gamma) \leq (j,k)$, run the simulator on the part of $\cC^*_\Del$ that interacts in the delete phase of session $(\gamma, 1-c_\gamma, 1-\alpha_\gamma)$. Otherwise run honest receiver strategy on session $(\gamma, 1-c_\gamma, 1-\alpha_\gamma)$.
           \item For $\gamma \in [i+1,\lambda]$, follow honest receiver strategy.
        \end{itemize}
        \item If the Reveal phase was not executed, then 
        \begin{itemize}
            \item For every $\gamma \in [1,i-1]$, run the simulator on the part of $\cC^*_\Del$ that interacts in the delete phases (sequentially) of $(\gamma, 1-c_\gamma, 0)$ and $(\gamma, 1-c_\gamma, 1)$.
            \item For $\gamma = i$, run the simulator on the part of $\cC^*_\Del$ that interacts in the delete phases (sequentially) of $(\gamma, 1-c_\gamma, b)$ for all $b \in \{0,1\}$ for which $(1-c_\gamma, b) \leq (j,k)$, and use honest receiver strategy on other sessions.
            %and $(\gamma, 1-c_\gamma, 1)$. Otherwise run honest receiver strategy on sessions $(\gamma, 1-c_\gamma, 0)$ and $(\gamma, 1-c_\gamma, 1)$. 
            \item For $\gamma \in [i+1,\lambda]$, follow honest receiver strategy.
        \end{itemize}
        \item Set $\mathsf{DelReq} = 1$.
   \end{itemize}
\underline{The output} of $\mathsf{Hybrid}_{i,j,k}$ is the final state of $\cC^*$ together with the bit $b^*$ (which is set to $\bot$ if the game aborted before $b^*$ was set), and the bit $\mathsf{DelReq}$.

We consider the interaction of $\cC^*$ with an honest receiver, and denote the state output by $\cC^*$ jointly with the bit output by the honest receiver in this interaction by $\mathsf{Hybrid}_{0,1,1}$. 
We now prove the following claim about consecutive hybrids.
%Sequentially run the extractor $\cE_{C_{a,b}}(\brho_{a,b})$ for all $a<i$ and $a=i, b<=j$ where $C_{a,b}$  denotes the part of the committer that participates in commitment session $(a,b)$, and $\brho_{a,b} = \brho$ when $(a,b) = (1,1)$, and otherwise $\brho_{a,b}$ denotes $(\bx_\com)$ where $(\bx_\com, \by_\com, b^*)$ is the output of $\cE_{C_{a,b}}$ in the commitment session just prior to session $(a,b)$.

%on all commitments in sessions $1, \ldots, i-1$ and on the first $j$ commitments in the $i^{th}$ session, but computing the receiver's output as in the honest protocol. 

%\dakshita{edit below. also add how to compute openings.}

%
\begin{claim}
There exists a negligible function $\mu(\cdot)$ such that for every $i \in [\lambda]$,  every $(\iota, j, k, \iota', j', k') \in \{(i - 1, 1, 1, i, 0, 0), (i, 0, 0, i, 0, 1), (i, 0, 1, i, 1, 0), (i, 1, 0, i, 1, 1)\}$,
\begin{itemize}
\item for every QPT distinguisher $\cD$,
$$|\Pr[\cD(\mathsf{Hybrid}_{\iota, j, k}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{\iota', j',k'}) = 1]| = \mu(\lambda)$$
\item and furthermore, for every unbounded distinguisher $\cD$,
$$|\Pr[\cD(\mathsf{Hybrid}_{\iota, j, k}^{\mathsf{DelReq}=0}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{\iota', j',k'}^{\mathsf{DelReq}=0}) = 1]| = \mu(\lambda)$$
where $\mathsf{Hybrid}_{\iota, j, k}^{\mathsf{DelReq}=0}$ is defined to be equal to $\mathsf{Hybrid}_{\iota,j,k}$ when $\mathsf{DelReq}$ is set to $0$, and defined to be $\bot$ otherwise, and likewise for $\mathsf{Hybrid}_{\iota', j',k'}^{\mathsf{DelReq}=0}$.
\end{itemize}
%$$|\Pr[\cD(\mathsf{Hybrid}_{i, 0, 0}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{i, 0,1}) = 1]| = \mu(\lambda),$$ $$|\Pr[\cD(\mathsf{Hybrid}_{i, 0, 1}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{i, 1, 0}) = 1]| = \mu(\lambda),$$ and $$|\Pr[\cD(\mathsf{Hybrid}_{i, 1, 0}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{i, 1, 1}) = 1]| = \mu(\lambda).$$
%and for every $i \in [\lambda]$ and every QPT distinguisher $\cD$, 
%$$|\Pr[\cD(\mathsf{Hybrid}_{i, 3}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{i+1, 0}) = 1]| = \mu(\lambda).$$
\end{claim}
\begin{proof} Suppose this is not the case. Then there exists an adversarial QPT committer $\cC^*$,  a polynomial $p(\cdot)$, and an initial committer state $\ket{\psi}$ that corresponds to a state just before the beginning of commitment $(\iota', j', k')$
where for some QPT distinguisher $\cD$,
%$(\iota, j, k, \iota', j', k') \in \{(i - 1, 1, 1, i, 0, 0), (i, 0, 0, i, 0, 1), (i, 0, 1, i, 1, 0), (i, 1, 0, i, 1, 1)\}$
%and where 
\begin{equation}
\label{eq:hybdone}
\Pr[\cD(\mathsf{Hybrid}_{\iota, j, k}) = 1] -  \Pr[\cD(\mathsf{Hybrid}_{\iota', j',k'}) = 1]| \geq \frac{1}{p(\lambda)}.
\end{equation}
or for unbounded $\cC^*$ and some unbounded distinguisher $\cD'$,
\begin{equation}
\label{eq:hybdtwo}
|\Pr[\cD'(\mathsf{Hybrid}_{\iota, j, k}^{\mathsf{DelReq}=0}) = 1] -  \Pr[\cD'(\mathsf{Hybrid}_{\iota', j',k'}^{\mathsf{DelReq}=0}) = 1]| \geq \frac{1}{p(\lambda)}
\end{equation}
Consider a reduction/adversarial committer $\widetilde{\cC}$ that obtains initial state $\ket{\psi}$, then internally runs $\cC^*$, forwarding all messages between an external receiver and $\cC^*$ for the $(\iota', j', k')^{th}$ commitment session, while running all other sessions according to the strategy in $\mathsf{Hybrid}_{\iota,j,k}$. 
The commit phase then ends, %with committer and receiver states resp. $(\bx_\com, \by_\com)$.
and $\widetilde{C}$ initiates the opening phase with the external receiver.
%, and on input $\bx_\com$, 
Internally, it continues to run the remaining commit sessions with $\cC^*$ -- generating for it the messages on behalf of the receiver according to the strategy in $\mathsf{Hybrid}_{\iota, j, k}$. 
The only modification is that it forwards $\cC^*$'s opening of the $(\iota', j', k')^{th}$ commitment (if and when it is executed) to the external challenger.
Finally, $\widetilde{\cC}$ behaves similarly if there is a delete phase, i.e., it forwards $\cC^*$'s deletion request and any messages generated in the delete phase of the $(\iota', j', k')^{th}$ commitment between $\cC^*$ and the external challenger.

Then, equation~(\ref{eq:hybdone}) and equation~(\ref{eq:hybdtwo}) respectively contradict the security of one-sided ideal commitments with EST against the committer $\cC^*$ (\cref{def:one-sided}). More specifically, equation~(\ref{eq:hybdone}) contradicts the computationally secure realization of $\cF_{\Com}^{\Del}$ whereas equation~(\ref{eq:hybdtwo}) contradicts the statistical security of $\Com$ against a corrupt committer that does not initiate deletion. This completes the proof of the claim.
%
%\cref{lem:os-id-one} and  contradicts \cref{lem:os-id-two}.
%, and records the opened bit $b'$.
%After the experiment is complete including the rest of the decommit phase, $\sC^*$ outputs the final state $\bx_\final = \brho$ of the committer.
%
%Then there is a distinguisher $\cD'$ that obtains the challenger's state $(\bx_\final, b)$ (or the variable $\mathsf{FAIL}$),  runs the distinguisher $\cD$ on $(\bx_\final, b)$, and by construction, obtains advantage $\frac{1}{p(\lambda)}$ in distinguishing the real and ideal experiments for the $(\iota', j', k')$ commitment, concluding the proof of the claim.
%which denote the final state of the committer and the opened bit $b$ in the real (resp. ideal) distributions for the extractable commitment.
%and executes the rest of the experiment according to $\mathsf{Hybrid}_{\iota, j, k}$.
%The claim being false implies that $\widetilde{\cC}^*$ contradicts extractability of the bit commitment.
\end{proof}
To complete the proof of the two lemmas, we observe that 
the only difference between $\mathsf{Hybrid}_{\lambda,1,1}$ and $\mathsf{Ideal}$ is the way the bit $b^*$ (output by the honest receiver) is computed. In more detail, in  $\mathsf{Hybrid}_{\lambda,1,1}$, the bit $b^*$ is computed as the majority of $\{b_i \oplus d_{i,1-c_i,0}\}_{i \in [\secp]}$.
%, where $e_{1-c_a,\alpha_a}^{(a)}$ is the bit extracted from commitment $e_{1-c_a,\alpha_a}$ in the $a^{th}$ iteration.
Now for every commitment strategy and every $i \in [\lambda]$, by correctness of extraction (which follows from the indistinguishability between real and ideal distributions for every commitment),
%\dakshita{the previous phrase is still a bit handwavy but I ran out of steam, its a statistical argument so I dont feel too uncomfortable about leaving it this way. but of course it would be better to write out the proof}
the probability that $d_{i,1-c_i,0} \neq d_{i,1-c_i,1}$ and yet the receiver does not abort in Step 2(c) in the $i^{th}$ sequential repetition, is $\leq \frac{1}{2} + \negl(\secp)$. 
Thus, this implies that the probability that $\mathsf{Hybrid}_{\lambda,1,1}$ and $\mathsf{Ideal}$ output different bits $b^*$ is at most $2^{-\secp/2} + \negl(\secp) = \negl(\secp)$, which implies that the two are statistically close. 
%This implies that $\mathsf{Hybrid}_{\secp,2}$ is indistinguishable from the $\mathsf{Ideal}$ distribution defined by the extractor defined above, since the only difference lies in the computation of the receiver's output $b^*$. 
%Since $\mathsf{Real}$ is identical to $\mathsf{Hybrid}_{0,1,1}$, this completes the proof.

This, combined with the claim above, completes the proof.
\end{proof}

\subsubsection{Security against a corrupt receiver}
\begin{lemma}
\label{lem:ts-idthree}
\proref{fig:ideal} computationally securely realizes $\cF_{\mathsf{Com}}^{\mathsf{Del}}$ (\cref{def:securerealization}) against a corrupt $R$.
%correctness of deletion (\cref{def:correctness-deletion}). 
\end{lemma}


\begin{lemma}
\label{lem:ts-idfour}
\proref{fig:ideal} satisfies certified everlasting security against $R$.
That is, for every QPT adversary $\{\cR_\secp^* \coloneqq (\cR^*_{\secp,\Com}, \cR^*_{\secp,\Rev}, \cR^*_{\secp,\Del})\}_{\secp \in \bbN}$ corrupting party $R$, there exists a QPT simulator $\{\cS_\secp \coloneqq (\cS_{\secp,\Com},\cS_{\secp,\Rev},\cS_{\secp,\Del})\}_{\secp \in \bbN}$ such that for any QPT environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\cZ_{\secp,2},\cZ_{\secp,3})\}_{\secp \in \bbN}$, and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelRes} = 1}[\cR^*_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF_{\mathsf{Com}}^\Del}^{\mathsf{DelRes} = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] where $\Pi^{\mathsf{DelRes} = 1}_{\cF_{\mathsf{Com}}^\Del}[\cR^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to be equal to $\Pi_{\cF_{\mathsf{Com}}^\Del}[\cR^*_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if the committer's output $\mathsf{DelRes}$ is set to 1, and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF_\Com^\Del}^{\mathsf{DelRes} = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$.
\end{lemma}
\begin{proof} (of Lemmas \ref{lem:ts-idthree} and \ref{lem:ts-idfour})\\

\noindent{\textbf{\underline{The simulator.}}}
The first stage of the simulator $\cS_{\Com}$, defined based on $\cR^*_\Com$, will be obtained via the use of the Watrous rewinding lemma (Lemma \ref{lem:qrl})~\cite{STOC:Watrous06}.
For the purposes of defining the simulation strategy, it will be sufficient (w.l.o.g.) to consider a restricted receiver $\cR^*_\Com$ that operates as follows in the $i^{th}$ sequential step of the commitment phase of the protocol.
In the simulation, the state of this step of $\cR^*_\Com$ will be initialized to the final state at the end of simulating the $(i-1)^{th}$ step.

\begin{enumerate}
\item $\cR^*_\Com$ takes a quantum register $\mathsf{W}$, representing its auxiliary quantum input. $\cR^*_\Com$ will use two additional quantum registers that function as work space: $\mathsf{V}$, which is an arbitrary (polynomial-size) register, and $\mathsf{A}$, which is a single qubit register. The registers $\mathsf{V}$ and $\mathsf{A}$ are initialized to the all-zero state before the protocol begins.

\item Let
$\textsf{M}$ denote the polynomial-size register used by the committer $C$ to send messages to $\cR^*_\Com$. After carrying out step 2(a) by running on registers $(\mathsf{W},\mathsf{V},\mathsf{A},\mathsf{M})$, $\cR^*_\Com$ measures the register $\mathsf{A}$ to obtain a bit $c_i$ for Step 2(b), which it sends back to $C$.

\item Next, $\cR^*_\Com$ computes the reveal phases (with messages from $C$ placed in register $\mathsf{M}$) according to Step 2(c). $\cR^*_\Com$ outputs registers $(\mathsf{W},\mathsf{V},\mathsf{A}, \mathsf{M})$.
\end{enumerate}

Any QPT receiver can be modeled as a receiver of this restricted form followed by some polynomial-time post-processing of the restricted receiver’s output. The same post-processing can be applied to the output of the simulator that will be constructed for the given restricted receiver.

Following~\cite{STOC:Watrous06}, we define a simulator that uses two additional registers, $\mathsf{C}$ and $\mathsf{Z}$, which are both initialized to the all-zero state. $\mathsf{C}$ is a one qubit register, while $\mathsf{Z}$ is an auxiliary register used to implement the computation that will be described next. Consider a quantum procedure $\cS_{\mathsf{partial}}$ that implements the strategy described in  \proref{fig:eqsimulator} using these registers.

\protocol
{\proref{fig:eqsimulator}}
{Partial Equivocal Simulator.}
{fig:eqsimulator}
{
%\textbf{Equivocal Simulator $\equivsim_{\sR^*}$:} Message $m \in \{0,1\}$

\underline{\textbf{Circuit $\cS_{\mathsf{partial}}$.}}
\begin{enumerate}
\item Sample a uniformly random classical bit $\widehat{c}$, and store it in register $\mathsf{C}$.
\item Sample uniformly random bits $(z,d)$.
\item 
If $\widehat{c} = 0$, initialize committer input as follows, corresponding to four sequential sessions:
\begin{itemize}
    \item For the first two sessions, set committer input to $z$.
    \item For the third and fourth sessions, set committer input to $d$ and $1-d$ respectively.
\end{itemize}
\item 
If $\widehat{c} = 1$, initialize committer input as follows, corresponding to four sequential sessions:
\begin{itemize}
    \item For the first and second sessions, set committer input to $d$ and $1-d$ respectively.
    \item For the last two sessions, set committer input to $z$.
\end{itemize}
\item Run the commitment phase interaction between the honest committer and $\cR^*_\Com$'s sequence of unitaries on registers $(\sW,\sV,\sA,\sM)$ initialized as above.
\item Measure the qubit register $A$ to obtain a bit $c$. If $c=\widehat{c}$, output 0, otherwise output $1$.
%For every $i \in [\lambda]$, $\cC$ and $R$ sequentially perform the following steps.
%\begin{enumerate}
%\item 
%apply unitary $R'$ on the following four sequential sessions:
\end{enumerate}
}

Next, we apply the Watrous rewinding lemma to the $\cS_{\mathsf{partial}}$ circuit to obtain a circuit $\widehat{\cS}_{\mathsf{partial}}$. To satisfy the premise of \cref{lem:qrl}, we argue that the probability $p(\ket{\psi})$ that $\cS_{\mathsf{partial}}$ outputs $0$ is such that $|p(\ket{\psi})-\frac{1}{2}| = \mathsf{negl}(\lambda)$, regardless of the auxiliary input $\ket{\psi}$ to the $i$'th sequential stage of $\cR^*_\Com$. This follows from the fact that the commitments are computationally hiding.
In more detail, by definition, Step 5 produces a distribution on $\cR^*_\Com$'s side that is identical to the distribution generated by $\cR^*_\Com$ in its interaction with the committer, who either has input $(z,z,d,1-d)$ (if $\widehat{c} = 0$) or input $(d,1-d,z,z)$ (if $\widehat{c} = 1$). If $|p(\ket{\psi})-\frac{1}{2}|$ were non-negligible, then the sequence of unitaries applied by $\cR^*_\Com$ could be used to distinguish commitments generated according to the case $\widehat{c} = 0$ from commitments generated according to the case $\widehat{c} = 1$, which would contradict the hiding of the commitment.

Now consider the residual state on registers $(\sW,\sV,\sA,\sM,\sC,\sZ)$ of $\cS_{\mathsf{partial}}$ conditioned on a measurement of its output register $\sA$ being $0$. The output state of $\widehat{\cS}_{\mathsf{partial}}$ will have negligible trace distance from the state on these registers. Now, the simulator $\cS_{\Com}$ must further process this state as follows.
\begin{itemize}
\item Measure the register $\mathsf{C}$, obtaining challenge $c$. Place the classical bits $(c,d)$ in the register $\sZ$, which also contains the current state of the honest committer algorithm.
\item Use information in register $\sZ$ to execute Step 2(c) of \proref{fig:ideal}.
\item Discard register $\sC$, re-define register $\sZ_i \coloneqq \sZ$ to be used later in the Reveal / Delete phases, and output registers $(\mathsf{W}, \mathsf{V}, \mathsf{A}, \mathsf{M})$ to be used in the next sequential step of the Commit phase. 
\end{itemize}

%Finally, after simulating $\lambda$ sequential sessions, sample $d_1, \ldots, d_{\lambda} \leftarrow \{0,1\}^{\lambda}$ and run the receiver's unitary on the resulting protocol. 

The simulator $\cS_\Com$ for the commit phase executes all $\lambda$ sequential interactions in this manner, and then samples $b_1, \ldots, b_{\lambda} \leftarrow \{0,1\}^{\lambda}$, as the committer messages for Step 3 of \proref{fig:ideal}. It then outputs the final state of $\cR^*_\Com$ on registers $(\mathsf{W}, \mathsf{V}, \mathsf{A}, \mathsf{M})$, and additionally outputs a private state on registers $(\sZ_1,\dots,\sZ_\secp)$, which consist of the honest committer's state after each of the $i$ sequential steps, as well as bits $(b_1,c_1,d_1,\dots,b_\secp,c_\secp,d_\secp)$.

%\dakshita{fix this. $\alpha_i = d_i \oplus ..$}
The reveal stage of the simulator $\cS_\Rev$ takes as input a bit $b$, and a state on registers $(\sZ_1,\dots,\sZ_\secp,\allowbreak\sW,\allowbreak\sV,\sA,\sM)$, and does the following for each $i \in [\secp]$. 
%samples 
%$%e'_1, \ldots e'_\lambda$ uniformly subject to $\bigoplus_{i \in [\lambda]}e'_i = b$ \andrea{I might be missing something, but I am confused about this last condition, and how $\alpha_i$ is obtained later: shouldn't there be a unique choice of $\alpha_i$ given the committing information sent earlier and the bit $b$?}.
%parses $\mathsf{st}$ as $(c_1,d_1,\ldots, c_\lambda,d_\lambda)$.
\begin{itemize}
\item Let $\widehat{d}_i = b \oplus b_i$.
\item If $c_i = 0$, it executes the decommitment phase for the $((\widehat{d}_i \oplus d_i)+2)^{th}$ session with $\cR^*_\Rev$.
\item If $c_i = 1$, it executes the decommitment phase for the $(\widehat{d}_i \oplus d_i)^{th}$ session with $\cR^*_\Rev$.
\item Output $\cR^*_\Rev$'s resulting state. Note that each decommitment will be to the bit $\widehat{d}_i = b \oplus b_i$.
\end{itemize}
%
Finally, the simulator $\cS_\Del$ for the delete phase executes the honest committer's algorithm on the commitments that were not revealed above.\\


\noindent{\textbf{\underline{Analysis.}}}
%To complete the proof of equivocality, we must establish that the distributions $\mathsf{Real}_b$ (the view of the receiver interacting with an honest committer) and $\mathsf{Ideal}_b$ (the view of the receiver interacting with the equivocator) of Definition \ref{def:eqcom}, are indistinguishable. This 
%
Lemma \ref{lem:ts-idthree} follows from the computational hiding of the underlying commitment scheme $\Com$, via an identical proof to~\cite{BCKM2021}. We have already argued above that the distribution produced by $\cS_\Com$ is statistically close to the distribution that would result from conditioning on the output of $\cS_{\mathsf{partial}}$ being 0 in each sequential step. Thus, it remains to argue that this is computationally indistinguishable from the real distribution. If not, then there exists a session $i \in [\lambda]$ such that the distribution in the real experiments up to the ${i-1}^{th}$ session is indistinguishable, but up to the $i^{th}$ session is distinguishable. However, this directly contradicts the computational hiding of the underlying commitment scheme.

%This contradicts the above guarantee given by the quantum rewinding lemma, since for any $i$, the post-processed residual qubits of $\cS_{\mathsf{partial}}$ are indistinguishable from the state of $\sR^*$ after the $i^{th}$ sequential session in the real protocol (due to the computational hiding of the commitment scheme).

In what follows, we prove Lemma \ref{lem:ts-idfour}. This only considers executions where $\mathsf{DelRes} = 1$, i.e., executions where $\cR^*$ successfully completes the delete phase. We again consider a sequence of $\lambda$ intermediate hybrids between the real and ideal executions.
We will let $\mathsf{Hybrid}_0^{\mathsf{DelRes} = 1}$ denote the final state of $\cR^*$ in the real experiment when the honest party output $\mathsf{DelRes} = 1$ and $\bot$ otherwise. Let $\mathsf{Hybrid}_i$ denote the final state of $\cR^*$ when the first $i$ (out of $\lambda$) sequential commit sessions are simulated using the $\widehat{\cS}_{\mathsf{partial}}$ circuit, defined based on $\cS_{\mathsf{partial}}$ from \proref{fig:eqsimulator}. Let $\mathsf{Hybrid}_i^{\mathsf{DelRes} = 1}$ denote the output of $\mathsf{Hybrid}_i$ when the honest party output $\mathsf{DelRes} = 1$ and $\bot$ otherwise. 

For every $i \in [\lambda]$, statistical indistinguishability between $\mathsf{Hybrid}_{i-1}^{\mathsf{DelRes} = 1}$ and $\mathsf{Hybrid}_{i}^{\mathsf{DelRes} = 1}$ follows by a reduction to the certified everlasting security of $\Com$ (according to \cref{def:one-sided}), as follows. The reduction $\mathsf{Red}$ is different depending on whether or not the Reveal phase is executed.
\begin{itemize}
    \item \underline{Case 1: The Reveal Phase is not executed.}
    $\mathsf{Red}$ acts as receiver in one session of $\Com$, interacting with an external challenger. 
    $\mathsf{Red}$ samples a uniformly random bit $d$ and sends it to the challenger. The challenger samples a uniformly random bit $b'$. If $b' = 0$, the challenger participates as a committer in a commit session to $d$ and otherwise to $(1-d)$.
    
    $\mathsf{Red}$ internally follows the strategy in $\mathsf{Hybrid}_{i-1}$ in the Commit phase for sessions $1, \ldots, i-1$ and $i+1, \ldots, \lambda$, based on the adversary $\cR^*_\Com$. During the $i^{th}$ session, $\mathsf{Red}$ interacts with the challenger and the adversary. In particular, it runs the strategy $\cS_{\mathsf{partial}}$ from \proref{fig:eqsimulator}, with the following exception. For $\widehat{c}$ sampled uniformly at random, if $\widehat{c} = 0$, it 
    forwards messages between $\cR^*_\Com$ and the challenger for either the third or fourth commitment (sampled randomly) and commits to $d$ in the other session and otherwise forwards messages between $\cR^*_\Com$ and the challenger for either the first or second commitment (sampled randomly) and commits to $d$ in the other session. If $\cR^*_\Com$'s challenge $c_i = \widehat{c}$, $\mathsf{Red}$ continues the experiment, otherwise it aborts. 
    $\mathsf{Red}$ continues to follow the strategy in $\mathsf{Hybrid}_{i-1}$, except setting $b_i = b \oplus d$.
    Note that the %subsequent to rewinding, %to ensure that $c = \widehat{c}$, it opens the commitments corresponding to $\widehat{c}$, which implies that the 
    challenge commitment is never opened.
    
    In the Delete phase, $\mathsf{Red}$ again follows the strategy in $\mathsf{Hybrid}_{i-1}$ except that it executes the Delete phase for the (two) unopened commitments in the $i^{th}$ session, one that it generated on its own, and the other by forwarding messages between $\cR^*_\Del$ and the external challenger. 
    
    By computational hiding of the challenger's commitment, the probability that the reduction aborts is at most $\frac{1}{2} + \negl(\secpar)$. Furthermore, conditioned on not aborting, the distribution output by $\mathsf{Red}$ is identical to $\mathsf{Hybrid}_{i-1}^{\mathsf{DelRes} = 1}$ 
    when $b' = 0$ and is statistically close to $\mathsf{Hybrid}_{i}^{\mathsf{DelRes} = 1}$ when $b' = 1$ (the latter follows because the output of $\widehat{\cS}_{\mathsf{partial}}$ and $\cS_{\mathsf{partial}}$ conditioned on $c_i = \widehat{c}$ are statistically close, due to Watrous rewinding).
    Thus if $\mathsf{Hybrid}_{i-1}^{\mathsf{DelRes} = 1}$ and $\mathsf{Hybrid}_{i}^{\mathsf{DelRes} = 1}$ are not negligibly close in trace distance, $\mathsf{Red}$ breaks certified everlasting hiding of $\mathsf{Com}$, as desired. 
    Finally, we observe that $\mathsf{Hybrid}_{\lambda}$ is identical to the ideal experiment.
    
    \item \underline{Case 2: The Reveal Phase is executed.}
    $\mathsf{Red}$ acts as receiver in one session of $\Com$, interacting with an external challenger. 
    $\mathsf{Red}$ samples a uniformly random bit $d$ and sends it to the challenger.
    The challenger samples a uniformly random bit $b'$. If $b' = 0$, the challenger generates a commitment to $d$, and otherwise to $1-d$.
    
    $\mathsf{Red}$ internally follows the strategy in $\mathsf{Hybrid}_{i-1}$ in the Commit phase for sessions $1, \ldots, i-1$ and $i+1, \ldots, \lambda$. For the $i^{th}$ session $\mathsf{Red}$ runs the strategy $\cS_{\mathsf{partial}}$ from \proref{fig:eqsimulator}, with the following exception. For bits $\widehat{c}, \widehat{b}$ sampled uniformly at random, it sets the commitment in sub-session $(2\widehat{c} + 1 + \widehat{b})$ as the external commitment, and generates the commitment in sub-session $(2\widehat{c} + 1 + (1-\widehat{b}))$ as a commitment to $d$. It sets commitments in the remaining two sessions according to the strategy in $\mathsf{Hybrid}_{i - 1}$.
    %if $\widehat{c} = 0$, it uniformly sets the third and fourth  and the fourth as the externally obtained challenge commitment, and otherwise sets the first commitment to $d$ and the second commitments as the externally obtained challenge commitments. 
    If $\cR^*_\Com$'s challenge $c_i = \widehat{c}$, $\mathsf{Red}$ continues the experiment, otherwise it aborts.
    $\mathsf{Red}$ continues to follow the strategy in $\mathsf{Hybrid}_{i-1}$, except setting $b_i = b \oplus d$.
    Note that the challenge commitment is not opened in the Commit phase.

    
    In the Reveal phase, $\mathsf{Red}$ behaves identically to $\mathsf{Hybrid}_{i-1}$ in sessions $(1, \ldots, i-1, i+1, \ldots, \lambda)$, and for session $i$ it runs the Reveal phase of the commitment in sub-session $(2\widehat{c} + 1 + (1-\widehat{b}))$. 
    %Note that %subsequent to rewinding, %to ensure that $c = \widehat{c}$, it opens the commitments corresponding to $\widehat{c}$, which implies that the 
    %challenge commitments are never opened.
    
    In the Delete phase, $\mathsf{Red}$ again follows the strategy of $\mathsf{Hybrid}_{i-1}$ except that it executes the Delete phase for the unopened commitments in the $i^{th}$ session by forwarding messages between $\cR^*_\Del$ and the external challenger. Thus, if $\mathsf{Hybrid}_{i-1}^{\mathsf{DelRes} = 1}$ and $\mathsf{Hybrid}_{i}^{\mathsf{DelRes} = 1}$ are not negligibly close in trace distance, $\mathsf{Red}$ breaks certified everlasting hiding of $\mathsf{Com}$, as desired. 
    Finally, we observe that $\mathsf{Hybrid}_{\lambda}$ is identical to the ideal experiment.
\end{itemize}
This completes the proof.
%When the Delete phase is executed, if $b_{\mathsf{guess}\text{-}\mathsf{rev}} = 0$, (both sessions)
%and if $b_{\mathsf{guess}\text{-}\mathsf{rev}} = 1$, (just the one remaining session).
%Since both experiments output $\bot$ when the Delete phase is not executed, the reduction
%We split the analysis into two cases, one where the Reveal phase occured before the Delete phase, and the other where it did not. In the first
\end{proof}


%\james{Hybrids: (1) Switch the first set of commitments to be generated using Watrous rewinding. We need standard computational hiding to show that the premise of the rewinding theorem is met. We need CEH to show statistical indistinguishability if deletion passes. This is only applied to the commitment $(1,1-c_1,1-\alpha_1)$. The reduction needs to condition on guessing the correct $c_1$, or instruct the distinguisher to output 0. The fact that conditioning succeeds with constant probability again requires standard computational hiding. (2) Switch $b_i$ to be a uniformly random bit. Here, we consider two cases. In the first case, Reveal is executed, and perfect indistinguishability follows by the randomness of $\alpha_1$. In the second case, Reveal is not executed, only Delete. This requires a reduction to CEH of the commitment $(1,1-c_1,\alpha_1)$. Finally, (1) and (2) are repeated for each $i \in [\secp]$.}





\subsection{Secure computation}\label{subsec:secure-computation}

In this section, we show that, following compilers in previous work, ideal commitments with EST imply oblivious transfer with EST and thus two-party computation of arbitrary functionalities with EST. Since prior compilers in the commitment hybrid model actually make use of ``commitments with selective opening'', we will first discuss this primitive, then describe a simple (deletion-composable) protocol that securely realizes commitments with selective opening. Next, we will invoke prior results~\cite{EC:GLSV21} that together with our composition theorem imply secure two-party computation with EST.

Finally, we define the notion of multi-party computation with EST, and again show that it follows from ideal commitments with EST.

\subsubsection{Two-party computation}\label{subsec:two-party-computation}

\protocol{Ideal functionality $\cF_{\socom}$}{Specification of the bit commitment with selective opening ideal functionality.}{fig:socom}{
Parties: committer $C$ and receiver $R$\\
Parameters: security parameter $\secp$ and function $r(\cdot)$\\
\begin{itemize}
    \item Commit phase: $\cF_{\socom}$ receives a query $(\text{Commit},\mathsf{sid},b_1,\dots,b_{r(\secp)})$ from $C$, where each $b_i \in \{0,1\}$, records this query, and sends $(\text{Commit},\mathsf{sid})$ to $R$.
    \item Reveal phase: $\cF_{\socom}$ receives a query $(\text{Reveal},\mathsf{sid},I)$ from $R$, where $I$ is an index set of size $|I| \leq r(\secp)$. $\cF_{\socom}$ ignores this message if no $(\text{Commit},\mathsf{sid},b_1,\dots,b_{r(\secp)})$ is recorded. Otherwise, $\cF_{\socom}$ records $I$ and sends a message $(\text{Reveal},\mathsf{sid},\{b_i\}_{i \in I})$ to $R$, and a message $(\text{Choice},\mathsf{sid},I)$ to $C$.
\end{itemize}
\noindent}

We define the ``commitment with selective opening'' ideal functionality $\cF_{\socom}$ in \proref{fig:socom}, and we describe a simple (deletion-composable) protocol $\Pi^{\cF_\com^\Del}$ that statistically securely realizes $\cF_{\socom}^\Del$.

\begin{itemize}
    \item The committer, with input $(b_1,\dots,b_{r(\secp)})$, sequentially sends $(\mathsf{Commit},i,b_i)$ to $\cF_\Com^\Del$ for $i \in [r(\secp)]$.
    \item The receiver, with input $I$, sends $I$ to the committer.
    \item The committer sequentially sends $(\mathsf{Reveal},i)$ for $i \in I$ to $\cF_\com^\Del$.
    \item The receiver obtains output $\{(\mathsf{Reveal},i,b_i)\}_{i \in I}$ from $\cF_\com^\Del$.
    \item The parties perform the delete phase as follows.
    \begin{itemize}
    \item If the committer is instructed to request a deletion, it sends $\{(\mathsf{DelRequest},i)\}_{i \in [r(\secp)]}$ to $\cF_\com^\Del$, which are forwarded to the receiver. %and sets it output $\DelReq = 1$. 
    \item If the receiver obtains \emph{any} $(\mathsf{DelRequest},i)$ for $i \in [r(\secp)]$, it sets its output $\mathsf{DelReq} = 1$.
    \item For each $(\mathsf{DelRequest},i)$ obtained by the receiver, it sends $(\mathsf{DelResponse},i)$ to $\cF_\com^\Del$, which are forwarded to the committer. %If the receiver sent $\{(\mathsf{DelResponse},i)\}_{i \in [r(\secp)]}$, it sets its output $\DelRes = 1$.
    \item If the committer obtains \emph{all} $\{(\mathsf{DelResponse},i)\}_{i \in [r(\secp)]}$, it sets its output $\DelRes = 1$.
    \end{itemize}
\end{itemize}

It is clear by definition that the above protocol statistically securely realizes $\cF_{\socom}^\Del$. Thus, by combining \cref{thm:CHSEE}, \cref{thm:one-sided}, and \cref{thm:ideal}, which together show that there exists a protocol that realizes $\cF_\com^\Del$ with EST assuming computationally-hiding statistically-binding commitments, and \cref{thm:composition}, which is our composition theorem, we obtain the following theorem.

\begin{theorem}\label{thm:socom}
There exists a protocol that securely realizes $\cF_{\socom}^\Del$ with EST that makes black-box use of a computationally-hiding statistically-binding commitment (\cref{def:comp-hiding} and \cref{def:SB}).
\end{theorem}

Note that it was necessary that our composition theorem handled reactive functionalities in order to establish this claim. Moreover, it is crucial in the definition of a reactive functionality with a deletion phase that we allow the deletion phase to be run after any phase of the reactive functionality. Indeed, in the above construction, some underlying commitments are not revealed but they still must be deleted. 

Finally, it was shown in \cite{EC:GLSV21} (building on the work of \cite{FOCS:CreKil88,C:DFLSS09}, among others) that using quantum communication, it is possible to statistically realize the primitive of \emph{oblivious transfer} in the $\cF_{\socom}$-hybrid model. Moreover, the work of \cite{STOC:Kilian88} showed how to statistically realize \emph{arbitrary two-party computation} in the oblivious transfer hybrid model. Since it is straightfoward to make these protocols deletion-composable with a delete phase at the end, we have the following corollary.

\begin{corollary}
Secure two-party computation of any polynomial-time functionality with Everlasting Security Transfer (\cref{def:security-with-EST}) exists, assuming only black-box use of a computationally-hiding statistically-binding commitment (\cref{def:comp-hiding} and \cref{def:SB}).
\end{corollary}

\subsubsection{Multi-party computation}

In order to define and construct multi-party computation with EST, we first have to specify a multi-party version of the Delete phase, which is described in \proref{fig:multidelPhase}.

\protocol{Muti-party Deletion phase}{A specification of a generic multi-party deletion phase that can be added to any multi-party ideal functionality $\cF$.}{fig:multidelPhase}{
Parties: $\{P_i\}_{i \in [n]}$
\begin{itemize}
    \item Receive a sequence of queries $(\mathsf{DelRequest},\mathsf{sid},i,j)$ which indicate that party $i$ is requesting party $j$ to delete their data. For each such query received, record it and send $(\mathsf{DelRequest},\mathsf{sid},i,j)$ to party $j$.
    \item Receive a sequence of queries $(\mathsf{DelResponse},\mathsf{sid},i,j)$ which indicate that party $i$ has deleted party $j$'s data. For each such query received, if there does not exist a recorded $(\mathsf{DelRequest},\mathsf{sid},j,i)$, then ignore the query. Otherwise, send $(\mathsf{DelResponse},\mathsf{sid},i,j)$ to party $j$.
\end{itemize}
}

To define security, we first note that it is straightforward to extend the discussion on the ``real-ideal paradigm'' from \cref{subsec:2PC-defs} to handle multi-party protocols where the adversary may corrupt any subset $M \subset [n]$ of $n$ parties. One can similarly generalize the definitions of computational and statistical secure realization (\cref{def:securerealization} and \cref{def:statsecurerealization}) to apply to multi-party protocols. Finally, we note that the multi-party Deletion phase introduced above adds $2(n-1)$ bits to each honest party $i$'s output, which we denote by $\{\DelReq_{j \to i},\DelRes_{j \to i}\}_{j \in [n] \setminus \{i\}}$, where each $\DelReq_{j \to i}$ indicates whether party $j$ requested that party $i$ delete its data, and each $\DelRes_{j \to i}$ indicates whether party $j$ deleted party $i$'s data. Now, we can generalize the notion of secure realization with EST (\cref{def:security-with-EST}) to the multi-party setting.

\begin{definition}[Secure realization with Everlasting Security Transfer: Multi-party protocols]\label{def:EST-multiparty}
A protocol $\Pi_\cF$ securely realizes the $\ell$-phase $n$-party functionality $\cF$ with EST if $\Pi_\cF$ computationally securely realizes $\cF^\Del$ (\cref{def:securerealization}) and the following holds. For every QPT adversary $\{\cA_\secp \coloneqq (\cA_{\secp,1},\dots,\cA_{\secp,\ell})\}_{\secp \in \bbN}$ corrupting a subset of parties $M \subset [n]$, there exists a QPT simulator $\{\cS_\secp \coloneqq (\cS_{\secp,1},\dots,\cS_{\secp,\ell})\}_{\secp \in \bbN}$ such that for any QPT environment $\{\cZ_{\secp} \coloneqq (\cZ_{\secp,1},\dots,\cZ_{\secp,\ell})\}_{\secp \in \bbN}$, and polynomial-size family of advice $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$, \[\TD\left(\Pi_{\cF^\Del}^{\mathsf{Del}_M = 1}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}], \widetilde{\Pi}_{\cF^\Del}^{\mathsf{Del}_M = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]\right) = \negl(\secp),\] 


where $\Pi^{\mathsf{Del}_M = 1}_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ is defined to be equal to $\Pi_{\cF^\Del}[\cA_\secp,\cZ_\secp,\ket{\psi_\secp}]$ if the bit $\mathsf{Del}_M = 1$ and defined to be $\bot$ otherwise, and likewise for $ \widetilde{\Pi}_{\cF^\Del}^{\mathsf{Del}_M = 1}[\cS_\secp,\cZ_\secp,\ket{\psi_\secp}]$. The bit $\mathsf{Del}_M$ is computed based on the honest party outputs, and is set to 1 if and only if for all $i \in [n] \setminus M$ and $j \in M$, $\DelReq_{j \to i} = 0$ and $\DelRes_{j \to i} = 1$.

\end{definition}

Note that we here we did not include a designated party (or parties) against whom statistical security should hold by default (as in \cref{def:security-with-EST}), but in principle one could define security in this manner. The definition as written in the multi-party case captures a type of \emph{dynamic} statistical security property, where after the completion of the protocol, any arbitrary subset of parties can comply with a deletion request and certifiably remove information about the other party inputs from their view.

Finally, we can prove the following corollary of \cref{thm:socom}.

\begin{corollary}
Secure multi-party computation of any polynomial-time functionality with Everlasting Security Transfer (\cref{def:EST-multiparty}) exists, assuming only black-box use of a computationally-hiding statistically-binding commitment (\cref{def:comp-hiding} and \cref{def:SB}).
\end{corollary}

\begin{proof}
It was shown by \cite{C:CreVanTap95} that multi-party computation of any polynomial-time functionality can be statistically realized in the oblivious transfer hybrid model, where each pair of parties has access to an ideal oblivious transfer functionality. The stand-alone composition theorem (\cref{thm:composition}) shows that this is also true in the quantum setting, so it remains to argue that the resulting multi-party protocol can be made to satisfy security with EST, assuming that the underlying oblivious transfers do. This only requires extending the notion of deletion-composability to this setting, which can be achieved with the following deletion phase.
\begin{itemize}
    \item If party $i$ is instructed to issue a deletion request to party $j$, they issue deletion requests for \emph{all} oblivious transfers that occurred between party $i$ and $j$ that were not already statistically secure against $j$. %, and they output $\DelReq_{i \to j} = 1$.
    \item If party $i$ obtains a deletion request from \emph{any} one of the oblivious transfers between party $i$ and party $j$, they output $\DelReq_{j \to i} = 1$.
    \item For each deletion request obtained by party $i$ from party $j$, party $i$ is instructed to send a deletion response to party $j$. %If party $i$ sent a deletion response to $j$ for \emph{all} oblivious transfers between party $i$ and party $j$ that were not already statistically secure against $i$, they output $\DelRes_{i \to j} = 1$.
    \item If party $i$ obtains a deletion response from party $j$ for \emph{all} oblivious transfers between party $i$ and party $j$ that were not already statistically secure against $j$, they output $\DelRes_{j \to i} = 1$.
\end{itemize}
This completes the proof.
\end{proof}


\section*{Acknowledgments}
We thank Bhaskar Roberts and Alex Poremba for comments on an earlier draft, and for noting that quantum fully-homomorphic encryption is not necessary for our FHE with certified deletion scheme, classical fully-homomorphic encryption suffices.

D.K. was supported in part by DARPA and NSF QIS award 2112890.
This material is based on work supported by DARPA under Contract No. 
HR001120C0024. Any opinions, findings and conclusions or recommendations expressed in
this material are those of the author(s) and do not necessarily reflect the views of the United States
Government or DARPA.

\iffalse
\paragraph{Oblivious transfer.} $\cF[\OT]$ is a two-party functionality between a sender $\cS$ with input $m_0,m_1 \in \{0,1\}^\ell$ and a receiver $\cR$ with input $b \in \{0,1\}$. The functionality delivers $m_b$ as output to the receiver. 

We will consider the following ideal functionality $\cF[\OT]_\Del$ where only the receiver $\cR$ has the ability to delete data. That is, in the ``deletion'' phase, $\cF[\OT]_\Del$ will take as input a bit $d_\cR$ from the receiver and deliver it to the sender $\cS$. 

\begin{definition}[Statistically sender private (SSP) OT with everlasting security transfer]\label{def:SSP-transfer}
An SSP OT with everlasting security transfer is a protocol $\Pi_{\cF[\OT]_\Del}$ such that the following two properties hold.
\begin{itemize}
    \item For any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the receiver $\cR$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$ such that for any sender inputs $\{(m_{0,\secp},m_{1,\secp})\}_{\secp \in \bbN}$, it holds that 
    \begin{itemize}
        \item For any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
        \item For any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,\begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1 \ | \ d_\cR = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1 \ | \ d_\cR = 1\right]\bigg| = \negl(\secp).\end{align*}
    \end{itemize}
    \item For any \emph{unbounded} adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the sender $\cS$, there exists a simulator $\{\cS_\secp\}_{\secp \in \bbN}$ with run-time at most polynomially larger than $\cA_\secp$, such that for any receiver inputs $\{b_\secp,d_\cR \coloneqq 0\}_{\secp \in \bbN}$, it holds that for any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,0)\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,0)\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
    \item For any \emph{QPT} adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the sender $\cS$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$ such that for any receiver inputs $\{b_\secp,d_\cR \coloneqq 1\}_{\secp \in \bbN}$, it holds that for any \emph{QPT} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,1)\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,1)\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

    
\end{itemize}
\end{definition}
\fi










%\begin{definition}[Secure computation with abort]\label{def:MPC}
%A protocol $\Pi_\cF$ securely realizes a functionality $\cF$ with abort if for any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any subset of parties $M \subset [n]$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, it holds that for any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_\cF\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_\cF\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

%Moreover, we say that a protocol $\Pi_\cF$ realizes a functionality with \emph{statistical} security against some subset of parties $P \subseteq [n]$, if for any \emph{unbounded} adversary $\{\cA_{\secp},\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any set of parties $M \subseteq P$, there exists a simulator $\{\cS_{\secp},\}_{\secp \in \bbN}$ whose run-time is at most polynomially larger than $\cA_\secp$'s run-time, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, and any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,
%\begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_\cF\left[\cA_{\secp},\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_\cF\left[\cS_{\secp},\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

%\end{definition}


%\paragraph{Certified everlasting security.} We will also consider the notion of \emph{certified everlasting security}. Here, $\cF$ is further modified to include a ``deletion'' phase after the abort phase described above, and we refer to the resulting ideal functionality as $\cF_{\Del}$. In this phase, $\cF_\Del$ takes as input a set of bits from each party $P_i$. For each honest party $P_i$, $\cF_\Del$ receives a set $\{d_{i,j}\}_{j \in [n] \setminus \{i\}}$, where each $d_{i,j}$ indicates whether $P_i$ deleted $P_j$'s input data. For each malicious party $P_i$, $\cF_\Del$ receives a set $\{d_{i,j}\}_{j \in H}$, where again each $d_{i,j}$ indicates whether $P_i$ deleted $P_j$'s input data. Then, $\cF_\Del$ returns to each party a set of bits. For each honest party $P_i$, $\cF_\Del$ returns a set of bits $\{d^*_{i,j}\}_{j \in [n] \setminus \{i\}}$, where $d^*_{i,j} \coloneqq d_{j,i}$ indicates whether party $P_j$ deleted $P_i$'s input data. For each malicious party $P_i$, $\cF_\Del$ returns a set of bits $\{d^*_{i,j}\}_{j \in H}$, where $d^*_{j,i} \coloneqq d_{j,i}$ indicates whether party $P_j$ deleted $P_i$'s data. 

%Note that now each honest party $P_i$ is initialized with an additional input $\{d_{i,j}\}_{j \in [n] \setminus \{i\}}$, and obtains an additional output $\{d^*_{i,j}\}_{j \in [n] \setminus \{i\}}$. Given a set of malicious parties $M \subset [n]$, the honest party inputs $\{\{d_{i,j}\}_j\}_{i \in H}$, and the $\{\{d^*_{i,j}\}_j\}_{i \in H}$ included in each honest party output, define a flag $\mathsf{DEL}$ to be equal to $\top$ if $d_{i,j} = 0$ for all  $i \in H, j \in M$ and $d^*_{i,j} = 1$ for all $i \in H,j \in M$, and equal to $\bot$ otherwise. That is $\mathsf{DEL} = \top$ when (i) none of the honest parties deleted the malicious party input data and (ii) all of the malicious parties deleted the honest party input data. Note that $\mathsf{DEL}$ can be computed as a predicate on the outcome of random variables $\Pi_\cF$ or $\widetilde{\Pi}_\cF$, so below we will consider conditioning the output of these random variables on the outcome of $\mathsf{DEL}$. 

%\paragraph{Two-phase adversaries.} To realize our definitions of secure computation with certified everlasting security, we will construct protocols with two separate phases: an \emph{online} phase in which the ``original'' functionality is computed, and a \emph{deletion} phase in which parties exchange messages with the purpose of realizing the deletion phase of the ideal functionality described above. It will sometimes be convenient to explicitly consider two-phase adversaries $\{\cA_{1,\secp},\cA_{2,\secp}\}_{\secp \in \bbN}$, where $\cA_{1,\secp}$ interacts in the online phases, and then passes on a state to $\cA_{2,\secp}$, who interacts in the deletion phase. The reason for this is that we will sometimes want to consider adversaries that are \emph{unbounded} in the online phase but \emph{QPT} as soon as they receive honest party messages in the deletion phase.



%\begin{definition}[Secure multi-party computation with certified everlasting security]\label{def:MPC-everlasting} A protocol $\Pi_{\cF_\Del}$ \emph{securely realizes} a functionality $\cF_\Del$ with abort and with certified everlasting security if for any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any subset of parties $M \subset [n]$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, it holds that
%\begin{itemize}
    %\item For any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
    %\item For any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,
    %\begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1 \ | \ \mathsf{DEL} = \top\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1 \ | \ \mathsf{DEL} = \top\right]\bigg| = \negl(\secp).\end{align*}
%\end{itemize}

%\end{definition}

==> IT-applications.tex <==
\section{Information-theoretic applications}

\subsection{One-time pad encryption}

\james{TODO, though maybe this should just be a remark after the section 3 theorem}

\subsection{Threshold secret sharing}

\begin{definition}[Threshold secret sharing]\label{def:TSS}
A $k$-out-of-$n$ threshold secret sharing scheme (for classical messages) is a tuple of two algorithms $(\Share,\Rec)$ with the following syntax.
\begin{itemize}
    \item $\Share(1^\secp,m) \to (\sh_1,\dots,\sh_n)$ takes as input a security parameter $\secp$ and a classical message $m \in \{0,1\}^*$, and outputs $n$ secret shares $\sh_1,\dots,\sh_n$.
    \item $\Rec(\{\sh_i\}_{i \in S}) \to m$ takes as input a set $S$ of shares of size at least $k$ and outputs a message $m$.
\end{itemize}
These algorithms should satisfy the following properties.
\begin{itemize}
    \item \textbf{Correctness.} For any $m$ and any $S \subseteq [n]$ of size at least $k$, with probability $1-\negl(\secp)$ over $\sh_1,\dots,\sh_n \gets \Share(1^\secp,m)$ it holds that $\Rec(\{\sh_i\}_{i \in S}) = m$.
    \item \textbf{Security.} For any $m_0,m_1$ of the same size, and any $S \subset [n]$ of size at most $k-1$, it holds that \[\left\{\{\sh_i\}_{i \in S} : \sh_1,\dots,\sh_n \gets \Share(1^\secp,m_0)\right\} \approx_s \left\{\{\sh_i\}_{i \in S} : \sh_1,\dots,\sh_n \gets \Share(1^\secp,m_1)\right\},\] where $\approx_s$ denotes negligible statistical distance.
\end{itemize}
\end{definition}

\begin{definition}[Threshold secret sharing with certified deletion]\label{def:CDTSS}
A $k$-out-of-$n$ quantum threshold secret sharing scheme (for classical messages) is a tuple of algorithms $(\CDShare,\CDRec,\CDDel,\CDVer)$ with the following syntax.
\begin{itemize}
\item $\CDShare(1^\secp,m) \to \ket{\psi}^{\sH_1,\dots,\sH_n},\vk$ takes as input a security parameter $\secp$ and a classical message $m \in \{0,1\}^*$, and outputs a quantum state on $n$ registers $\sH_1,\dots,\sH_n$, and a (potentially quantum) verification key $\vk$.
\item $\CDRec(\ket{\psi}^{\{\sH_i\}_{i \in S}}) \to m$ takes as input a quantum state on a set $S$ of registers $\sH_i$ of size at least $k$ and outputs a message $m$.
\item $\CDDel(\ket{\psi}^{\sH_i}) \to \cert$ takes as input a quantum state on register $\sH_i$ and outputs a (potentially quantum) deletion certificate $\cert$.
\item $\CDVer(\vk,i,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$, an index $i \in [n]$, and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
\end{itemize}

These algorithms should satisfy the following properties.
\begin{itemize}
    \item \textbf{Correctness.} For any $m$ and any $S \subseteq [n]$ of size at least $k$, with probability $1-\negl(\secp)$ over $\ket{\psi}^{\sH_1,\dots,\sH_n} \gets \Share(1^\secp,m)$ it holds that $\Rec(\ket{\psi}^{\{\sH_i\}_{i \in S}}) = m$.
    \item \textbf{Security.} \james{this is the static definition} For any unbounded adversary $\{\cA_\secp\}_{\secp \in \bbN}$, it holds that \[\TD\left(\SSEXP_\secp^{\cA}(0),\SSEXP_\secp^{\cA}(1)\right) = \negl(\secp),\] where the experiment $\SSEXP_\secp^{\cA}(b)$ is defined as follows.
    \begin{itemize}
        \item Sample $\ket{\psi}^{\sH_1,\dots,\sH_n},\vk \gets \CDShare(1^\secp,b)$. %and initialize empty sets $C \coloneqq \{\}$ and $D \coloneqq \{\}$.
        \item $\cA_\secp$ requests a set $S \subset [n]$ of shares of size $< k$, and receives the registers $\{\sH_i\}_{i \in S}$.
        \item $\cA_\secp$ outputs a set $\{\cert_i\}_{i \in D}$ of deletion certificates, a sequence $S' \subseteq [n] \setminus S$ of new share requests, and a final quantum state $\rho$.
        \item Let $d$ be the number of $i \in D$ such that $\CDVer(\vk,i,\cert_i) = \top$. If $d \leq n-k$, the experiment outputs $\rho$ along with registers $\sH_i$ for the first $d$ indices $i \in S'$. Otherwise, if $d > n-k$, the experiment outputs $\rho$ along with all the remaining registers $\{\sH_i\}_{i \in [n] \setminus S}$.
        %\item If $\cA_\secp$ halted, then output $\cA_\secp$'s current state $\rho$. Otherwise, if $|D| > n-k$, the output $\cA_\secp$'s current quantum state $\rho$ along with the remaining uncorrupted shares on registers $\{\sH_i\}_{i \in [n] \setminus C}$.
    \end{itemize}
\end{itemize}

\end{definition}

Now, we give a construction of $k$-out-of-$n$ secret sharing with certified deletion. Let $(\Share_{k,n},\Rec_{k,n})$ be Shamir's $k$-out-of-$n$ threshold secret sharing scheme (\cref{def:TSS}). We will use the fact that in Shamir secret sharing, any set of less than $k$ shares are uniformly and independently distributed over some alphabet.

\begin{itemize}
    \item $\CDShare(1^\secp,m):$ 
    \begin{itemize}
        \item Sample $\sh_1,\dots,\sh_n \gets \Share_{k,n}(1^\secp,m)$. Let $p$ be the number of bits in each $\sh_i$.
        \item For each $i \in [n]$, sample $\left\{x_{i,\ell},\theta_{i,\ell} \gets \{0,1\}^\secp\right\}_{\ell \in [p]}$ and  \[\left\{\sh_i^j\right\}_{j \in [n] \setminus \{i\}} \gets \Share_{k-1,n-1}(1^\secp,(\theta_{i,1},\dots,\theta_{i,p})).\]
        \item Let the $i$'th share on register $\sH_i$ consist of \[\left\{\ket{x_{i,\ell}}_{\theta_{i,\ell}}, \sh_{i,\ell} \oplus \bigoplus_{t: \theta_{i,\ell,t} = 0}x_{i,\ell,t}\right\}_{\ell \in [p]}, \left\{\sh_{j}^i\right\}_{j \in [n] \setminus \{i\}}.\]
        \item Let $\vk$ consist of $\{x_{i,\ell},\theta_{i,\ell}\}_{i \in [n],\ell \in [p]}$.
    \end{itemize}
    \item $\CDRec(\{\sH_i\}_{i \in S})$:
    \begin{itemize}
        \item Parse the state on each $\sH_i$ as $\{\ket{\psi_{i,\ell}},\sh_{i,\ell}'\}_{\ell \in [p]}, \{\sh_j^i\}_{j \in [n] \setminus \{i\}}$.
        \item For each $i \in S$, first compute $(\theta_{i,1},\dots,\theta_{i,p}) \gets \Rec_{k-1,n-1}(\{\sh_i^j\}_{j \in S \setminus \{i\}})$. Then, for each $\ell \in [p]$, obtain $\{x_{i,\ell,t}\}_{t : \theta_{i,\ell,t} = 0}$ by measuring $\ket{\psi_{i,\ell}}$ in basis $\theta_{i,\ell}$, and compute $\sh_{i,\ell} = \sh'_{i,\ell} \oplus \bigoplus_{t: \theta_{i,\ell,t} = 0}x_{i,\ell,t}$. Finally, set $\sh_i = (\sh_{i,1},\dots,\sh_{i,p})$.
        \item Compute $m \gets \Rec_{k,n}(\{\sh_i\}_{i \in S})$.
    \end{itemize}
    \item $\CDDel(\sH_i)$: parse the state on $\sH_i$ as $\{\ket{\psi_{i,\ell}},\sh_{i,\ell}'\}_{\ell \in [p]}, \{\sh_j^i\}_{j \in [n] \setminus \{i\}}$, measure each $\ket{\psi_{i,\ell}}$ in the Hadamard basis to obtain $x'_{i,\ell}$, and set $\cert = (x'_{i,0},\dots,x'_{i,p})$.
    \item $\CDVer(\vk,i,\cert):$ parse $\vk$ as $\{x_{i,\ell},\theta_{i,\ell}\}_{i \in [n],\ell \in [p]}$ and $\cert$ as $\{x'_{i,\ell}\}_{\ell \in [p]}$. Output $\top$ if and only if $x_{i,\ell,t} = x'_{i,\ell,t}$ for all $\ell,t$ such that $\theta_{i,\ell,t} = 1$.
\end{itemize}


\begin{theorem}
The above construction is a $k$-out-of-$n$ secret sharing scheme with certified deletion, satisfying \cref{def:CDTSS}.
\end{theorem}

\begin{proof}
We consider a simulated experiment $\mathsf{Sim}\text{-}\mathsf{EXP}_\secp^{\cA}$, which is identical to $\SSEXP_\secp^{\cA}(b)$ except that all of the shares $\sh_1,\dots,\sh_n$ are sampled independently and uniformly random over the alphabet for $\Share_{k,n}$. Note that $\mathsf{Sim}\text{-}\mathsf{EXP}_\secp^{\cA}$ has no dependence on $b$. However, we argue that the trace distance between $\mathsf{Sim}\text{-}\mathsf{EXP}_\secp^{\cA}$ and $\SSEXP_\secp^{\cA}(b)$ for either $b \in \{0,1\}$ is negligible, which completes the proof.

\james{TODO}



%\begin{itemize}
    %\item Sample $\sh_1,\dots,\sh_n$ each uniformly random and independent over the alphabet used for $\Share_{k,n}$. Sample $\{\theta_{i,\ell} \gets \{0,1\}^\secp\}_{i \in [n],\ell \in [p]}$.
    %\item Receive a request $S \subset [n]$ from $\cA_\secp$.
    %\item For $i \in [S]$, sample $\{\sh_i^j\}_{j \in S \setminus \{i\}}$ each uniformly random and independent over the alphabet used for $\Share_{k-1,n-1}$. For $i \notin S$, sample $\{\sh_i^j\}_{j \in [n] \setminus \{i\}} \gets \Share_{k-1,n-1}(1^\secp,(\theta_{i,1},\dots,\theta_{i,p}))$. For each $i \in S$, output \[\left\{\ket{x_{i,\ell}}_{\theta_{i,\ell}}, \sh_{i,\ell} \oplus \bigoplus_{t:\theta_{i,\ell,t} = 0}x_{i,\ell,t}\right\}_{\ell \in [p]}, \{\sh_j^i\}_{j \in [n] \setminus \{i\}}\] to $\cA_\secp$.
    %\item Receive a set $\{\cert_i\}_{i \in D}$ from $\cA_\secp$
%\end{itemize}
\end{proof}


\subsection{Client-server MPC}

\james{TODO}

==> OT-EST.tex <==
\section{Outline}

\begin{itemize}
    \item We start with a computationally hiding statistically efficiently extractable (CHSEE) commitment, which we will argue can be built from black-box use of one-way functions or psuedorandom quantum states. The notion of statistically efficiently extractable means that there exists a polynomial $p(\secp)$ such that for any adversarial committer, there exists an extractor with run time at most $p(\secp)$ times that of the committer, that extracts the bit committed and produces a committer view that is statistically close to the real view.
    \item We add BB84 states and then one-sided statistical 2PC to obtain a CHSEE commitment with everlasting security transfer (EST). Here, hiding is the same as hiding for a certified everlasting hiding commitment, and binding is the efficiently extractable notion above, except that after deletion, the view is only guaranteed to be computationally indistinguishable. For the syntax, after the Commit phase, either Delete or Open can be run, but not both. \james{We don't need secret sharing, but we do need the committer to open its commitments to $\theta$ under the 2PC functionality}
    \dakshita{But delete can be run after open technically, right?}
    \item We apply the BCKM equivocality compiler to obtain an ideal commitment with EST. We define an ideal commitment with an ideal functionality that takes a bit $b$ from the committer in the Commit phase, and delivers it to the receiver in the Open phase. In addition, there is a Delete phase which may be run either after the Commit phase or after the Open phase. When this is run, the ideal functionality takes as input a bit from the adversarial party which determines whether deletion passes, and outputs this bit to both parties. In the case that deletion passes, the ideal views will now be statistical for an adversarial receiver and computational for an adversarial committer. \james{An alternative equivocality compiler would run the Open phase under 2PC - but this seems to require 2PC with EST, which is what we are trying to construct}
    \item Apply the CK compiler to show that ideal commitment with EST implies SSP OT with EST.
\end{itemize}


\james{old below}

\begin{itemize}
    %\item Begin with a statistically binding (SB) commitment with certified everlasting (CE) hiding: \[\Com(b): \ket{x}_{\theta}, \com\left(\theta, b \oplus \bigoplus_{i : \theta_i = 0} x_i\right),\] where $\com$ is a standard SB commitment scheme. The deletion certificate $x'$ is produced by measuring the quantum state in the Hadamard basis, and passes if $x_i = x'_i$ for all $i$ such that $\theta_i = 1$ . The opening is just the opening for $\com$. Our notion of statistical binding in the quantum setting will follow AQY, which asks that there is an unbounded extractor during the commit phases that produces $b$. This already implies zero-knowledge proofs for NP (and QMA) with CE zero-knowledge via HMNY. Would be good to check if this also gives a NIZK.
    %\item Next, we will enhance the above commitment scheme to a commitment with \emph{everlasting security transfer} (EST). To do so, we ask the receiver to actually sample a random set of bases $\theta'$ and measure to obtain $x'$. Then the delete phase consists of an SFE where the committer inputs $(\theta,x)$, the receiver inputs $(\theta',x')$, and the functionality outputs 1 to the sender if $x_i = x_i'$ for all $i$ such that $\theta_i = \theta_i' = 1$ (and there are sufficient number of $i$ such that $\theta_i' = 1$). This SFE should be implemented with statistical security against a malicious receiver and computational security against a malicious committer. The opening is now the opening for $\com$ (which in particular reveals $\theta$), and additionally the string $x$. Verification will check that $x_i = x'_i$ for all $i$ such that $\theta_i = \theta_i' = 0$. Now, the committer can actually cheat with probability roughly 1/2, we so we will parallel repeat the commitment scheme $\secp$ times.
    \item First, we run the commitment scheme with EST through the BCKM equivocality compiler to obtain an equivocal commitment with EST. This means that if deletion is not invoked then the scheme is SB and computationally equivocal. If deletion passes, then it satisfies the following notions:
    \begin{itemize}
        \item Binding: there is an inefficient extractor during the commit phase that outputs $b$. Then, no computationally bounded committer during the delete and open phase can cause the receiver to output $1-b$.
        \item Hiding: for any adversarial receiver that is computationally bounded during the commit and delete phase, there exists an (efficient) equivocal simulator that produces a distribution that is statistically close to the real distribution.
    \end{itemize}
    \item Next, we run the equivocal commitment with EST through the BCKM extractability compiler to obtain an extractable commitment with EST. Now, the deletion phase has a different ``direction'', and is invoked from the committer to the receiver. If deletion is not invoked then the scheme is (efficiently) extractable and statistically hiding. If deletion passes, then it satisfies the following notions:
    \begin{itemize}
        \item Binding: for any adversarial committer that is computationally bounded during the commit and delete phase, there exists an efficient extractor that outputs $b$ and a state that is statistically close to the real distribution. This distribution given to the distinguisher is set to FAIL if the bit opened during the open phase is not $b$. 
        \item Hiding: standard computational hiding.
    \end{itemize}
    \item Next, we run the extractable commitment with EST through the BCKM equivocality compiler to obtain an extractable and equivocal commitment with EST. Here, the deletion phase is from the receiver to the committer. If deletion is not invoked then the scheme is (efficiently) extractable against computationally bounded committers and equivocal against unbounded receivers. If deletion passes, then it satisfies the same notion of binding as the previous commitment and is equivocal against computationally bounded receivers.
    \item Finally, we plug the above into the CK template to obtain an OT with EST, which is statistically receiver private, and can become statistically sender private after an everlasting security transfer phase. Then, we can use this OT via IPS08 to obtain MPC with EST.
\end{itemize}

==> SKE.tex <==
\subsection{Sketch for SKE proof}

\begin{theorem}
Consider the following experiment $\EVEXP_\secp^{\cA}(b)$, initialized with an unbounded adversary $\cA_\secp$.
\begin{itemize}
    \item Sample $x,\theta \gets \{0,1\}^\secp$, and initialize $\cA_\secp$ with \[\ket{x}_\theta, b \oplus \bigoplus_{i:\theta_i = 0}x_i.\]
    \item $\cA_\secp$'s output is parsed as a bitstring $x' \in \{0,1\}^\secp$ and a residual quantum state $\rho$.
    \item If $x_i = x_i'$ for all $i$ such that $\theta_i = 1$ then output $(\top,\rho)$, and otherwise output $(\bot,\rho)$.
\end{itemize}
Then,
\[\TD\left(\EVEXP_\secp^\cA(0),\EVEXP_\secp^\cA(1)\right) = \negl(\secp).\]
\end{theorem}

\begin{proof}

First, we again consider a hybrid where $\cA_\secp$ is initialized with $b' \gets \{0,1\}$, and then the experiment aborts if $b' \neq b \oplus \bigoplus_{i:\theta_i = 0}x_i$. So the output of the experiment is now either $\abort, (\top,\rho),$ or $(\bot,\rho)$. We will also purify the experiment so that $x,\theta$ are not measured until $\cA_\secp$ returns $x'$. Finally, we can remove $b'$ and $b$ from the experiment and just consider the trace distance between the reduced density matrices on $\cA_\secp$'s registers conditioned on whether $\bigoplus_{i:\theta_i = 0}x_i$ is equal to 0 or 1. For $\theta \in \{0,1\}^\secp$, let $\theta_1 \subseteq [\secp]$ be the subset of indices $i$ such that $\theta_i = 1$. So we are interested in the trace distance between the reduced density matrices on the $\sA$ registers of following two states for $b=0$ and $b=1$.

\[\frac{1}{2^\secp}\sum_{\substack{(\theta,x):\bigoplus_{i:\theta_i = 0}x_i = b,\\ x' \in \{0,1\}^\secp,u \in \{0,1\}^{|\theta_1|}}}\frac{(-1)^{u \cdot x_{\theta_1}}}{2^{|\theta_1|/2}}\ket{\theta}\ket{x}\ket{u}\ket{x'}\ket{\mathbbm{1}_{x'_{\theta_1} = u}}^{\sA}\ket{\phi_{x,x'}}^{\sA},\] where $\ket{\phi_{x,x'}}$ are arbitrary such that for each $x$, $\sum_{x'} \ket{\phi_{x,x'}}$ is normalized. Note that this state is the result of initializing the adversary with the $\sA$ register of \[\frac{1}{2^\secp}\sum_{x,\theta}\ket{\theta}\ket{x}\ket{x}^\sA,\] applying an arbitrary operation on $\sA$ to map to outputs $x'$ along with residual states, conditioning on $\bigoplus_{i:\theta_i = 0}x_i =b$, and returning to the adversary whether measuring the positions of $x$ where $\theta_i = 1$ in the Hadamard basis is equal to $x'$.

Thus, we want to bound the trace distance between

\[\frac{1}{2^{2\secp}}\sum_{\substack{(\theta,x) : \bigoplus_{i:\theta_i = 0}x_i = 0,\\x' \in \{0,1\}^\secp,u \in \{0,1\}^{|\theta_1|}}}\frac{1}{2^{|\theta_1|}}\ket{\mathbbm{1}_{x'_{\theta_1} = u}}\bra{\mathbbm{1}_{x'_{\theta_1} = u}}\ket{\phi_{x,x'}}\bra{\phi_{x,x'}}\]

and \[\frac{1}{2^{2\secp}}\sum_{\substack{(\theta,x) : \bigoplus_{i:\theta_i = 0}x_i = 1,\\x' \in \{0,1\}^\secp,u \in \{0,1\}^{|\theta_1|}}}\frac{1}{2^{|\theta_1|}}\ket{\mathbbm{1}_{x'_{\theta_1} = u}}\bra{\mathbbm{1}_{x'_{\theta_1} = u}}\ket{\phi_{x,x'}}\bra{\phi_{x,x'}}.\]

To show that this trace distance is negligible, we will actually condition on the Hamming weight of $x$ being between $(1/2-\epsilon)\secp$ and $(1/2-\epsilon)\secp$, and the Hamming weight of $\theta$ being at least $(1/2-\delta)\secp$ for some constants $\epsilon < \delta$, which occurs with overwhelming probability (I'm not sure if we have to be this strict with the conditioning yet). Then we can show that for every $x,x'$, it holds that \[\TD\left(\sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 0,u \in \{0,1\}^{|\theta_1|}}\frac{\ket{\mathbbm{1}_{x'_{\theta_1} = u}}\bra{\mathbbm{1}_{x'_{\theta_1} = u}}}{2^{|\theta_1|}},\sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 1,u \in \{0,1\}^{|\theta_1|}}\frac{\ket{\mathbbm{1}_{x'_{\theta_1} = u}}\bra{\mathbbm{1}_{x'_{\theta_1} = u}}}{2^{|\theta_1|}}\right) = \negl(\secp).\]

This trace distance is simply \begin{align*}&\bigg|\sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 0}\frac{1}{2^{|\theta_1|}} - \sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 1}\frac{1}{2^{|\theta_1|}}\bigg|\\ &\leq \frac{\secp}{2^{(1/2-\delta)\secp}}\bigg|\big|\{\theta: |\theta_1| \geq (1/2-\delta)\secp, \bigoplus_{i \in \theta_0}x_i = 0\}| - |\{\theta: |\theta_1| \geq (1/2-\delta)\secp, \bigoplus_{i \in \theta_0}x_i = 1\}\big|\bigg|.\end{align*}

Thus, it suffices to show that any fixed $x$ of Hamming weight between $(1/2-\epsilon)\secp$ and $(1/2-\epsilon)\secp$ is a balanced enough predicate over all binary strings of Hamming weight at most $(1/2+\delta)\secp$. We know that $x$ is perfectly balanced over all binary string and that strings of Hamming weight at most $(1/2+\delta)\secp$ make up an overwhelming fraction of all strings.

\begin{conjecture}
Let $\delta > 0$ be a small enough constant and fix an $x \in \{0,1\}^\secp$ (we can assume if we need to that $x$ is somewhat balanced, in the sense that its Hamming weight is between $(1/2-\epsilon)\secp$ and $(1/2+\epsilon)\secp$ for some constant $\epsilon$ that could even be set smaller than $\delta$). Let $T_\delta \subset \{0,1\}^\secp$ be the set of binary strings of Hamming weight at most $(1/2+\delta)\secp$. Then it holds that \[\frac{\bigg||\{y \in T_\delta : x \cdot y = 0\}| - |\{y \in T_\delta : x \cdot y = 1\}|\bigg|}{2^{(1/2-\delta)\secp}} = \negl(\secp).\]

Notes:
\begin{itemize}
    \item If $\delta$ is too large, then we cannot hope for the difference to be negligible, because of the denominator.
    \item The difference is 0 (for all $x \neq 0^\secp$) if we consider all $y \in \{0,1\}^\secp$, but we are restricting to $y$ of bounded Hamming weight.
    \item If $x$ has very low Hamming weight (say 1), I don't think that the expression will be negligible, because a significant fraction of $y$ with bounded Hamming weight will not overlap with the coordinate of $x$ that is 1, making the set where $x\cdot y = 0$ much larger. This is why we might need to consider restricting to fixed $x$ that have somewhat high Hamming weight, which would still suffice.
\end{itemize}

For context, we would be using the above claim to bound the expression 

\[\bigg|\sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 0}\frac{1}{2^{\cH\cW(\theta)}} - \sum_{\theta:\bigoplus_{i:\theta_i = 0}x_i = 1}\frac{1}{2^{\cH\cW(\theta)}}\bigg|\] for \emph{every} fixed $x$ in some set of strings that make up an overwhelming fraction of $\secp$ bit strings. And we are allowed to restrict to any set of $\theta$ that make up an overwhelming fraction of $\secp$ bit strings.
\end{conjecture}

%It suffices to show that this is negligible for any $x$ with Hamming weight at least $(1/2-\delta)\secp$ for some constant $\delta$, since such $x$ make up an overwhelming fraction of all binary strings. Now, if $|\theta_0| + |x_1| > \secp$, then the difference over $\theta$ is 0, so we only need to worry about $j \geq (1/2-\delta)\secp$. Moreover, for any $j \geq (1/2+\delta)\secp$, the difference is negligible, since the number of $\theta$ of Hamming weight $\geq (1/2+\delta)\secp$ is negligible compared to $1/2^{(1/2+\delta)\secp}$. Thus, it remains to bound the differences for $x$ of Hamming weight at least $(1/2-\delta)\secp$, and $\theta$ of Hamming weight between $(1/2-\delta)\secp$ and $(1/2+\delta)\secp$.

\end{proof}


==> applications-deprecated.tex <==
\section{Cryptography with Certified Everlasting Security}
\label{sec:app}

\subsection{Secret sharing}\label{subsec:ss}

We give a simple construction of a 2-out-of-2 secret sharing scheme where there exists a designated party that the dealer can ask to produce a certificate of deletion of their share. If this certificate verifies, then the underlying plaintext is information theoretically deleted, even given the other share.

\paragraph{Definition.}
First, we augment the standard syntax of secret sharing to include a deletion algorithm $\Del$ and a verification algorithm $\Ver$. Formally, consider a secret sharing scheme $\CD$-$\SSS = (\Share,\Rec,\Del,\Ver)$ with the following syntax.

\begin{itemize}
    %\item $\Share(1^\secp) \to (\pk,\sk)$ is a classical algorithm that takes as input the security parameter and outputs a public key $\pk$ and secret key $\sk$.
    \item $\Share(m) \to (s_1, s_2, \vk)$ is a quantum algorithm that takes as input a classical message $m$, and outputs a quantum share $s_1$, a classical share $s_2$ and a (potentially quantum) verification key $\vk$.
    \item $\Rec(s_1,s_2) \to \{m,\bot\}$ is a quantum algorithm that takes as input two shares and outputs either a message $m$ or a $\bot$ symbol.
    \item $\Del(s_1) \to \cert$ is a quantum algorithm that takes as input a quantum share $s_1$ and outputs a (potentially quantum) deletion certificate $\cert$.
    \item $\Ver(\vk,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$ and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
\end{itemize}

We say that $\CD$-$\SSS$ satisfies correctness of deletion if the following holds.

\begin{definition}[Correctness of deletion]\label{def:CD-correctness-SS}
$\CD$-$\SSS = (\Share,\Rec,\Del,\Ver)$ satisfies \emph{correctness of deletion} if for any $m$, it holds with $1-\negl(\secp)$ probability over $(s_1,s_2,\vk) \gets \Share(m),\cert \gets \Del(s_1), \mu \gets \Ver(\vk,\cert)$ that $\mu = \top$.
\end{definition}

Next, we define certified deletion security for a secret sharing scheme.

\iffalse{
\begin{definition}[Computational No-Signaling Adversary]
An adversary $\cA = \{\cA_{\secp}\}_{\secp \in \bbN}$ 
that on input a quantum-classical state $(s_1, s_2) \in \bbC^{2^{\secp+1}} \times \{0,1\}^\secp$ produces a quantum (mixed) state $\rho$
is a {\em no-signaling} adversary if for every pure state $s_1 \in \bbC^{2^{\secp+1}}$ and every
pair of strings $(s_2, s_2') \in \{0,1\}^\secp \times \{0,1\}^\secp$,
the distributions $\cA_\secp(s_1, s_2)$ and $\cA_\secp(s_1, s_2')$ are computationally indistinguishable.
\end{definition}
}\fi

\begin{definition}[Certified deletion security]\label{def:CD-security}

%and
%\[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
Let $\cA = \{\cA_\secp\}_{\secp \in \bbN}$ denote a computational no-signaling adversary and $b$ denote a classical bit. Consider experiment $\EVEXP_\secp^{\cA}(b)$ which describes everlasting security given a deletion certificate, and is defined as follows.
\begin{itemize}
    \item Sample $(s_1,s_2,\vk) \gets \Share(b)$.
    \item Initialize $\cA_{\secp}$ with $(s_1, s_2)$.
    %, and $\cA_{2,\secp}(\ket{\psi_\secp})$ with $s_2$.
    \item Parse $\cA_{\secp}$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ then output $(\rho, s_2)$, and otherwise output $\bot$.
\end{itemize}
Then $\CD$-$\SSS = (\Share,\Rec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any computational {\em no-signaling} adversary $\cA$, 
it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp),\]
%
\iffalse{
and the experiment $\CEXP_\secp^{\cA}(b)$ is a strengthening of semantic security, defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$ and $(\ct,\vk) \gets \Enc(\pk,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item Output $\cA_\secp \left(\rho, \Ver(\vk,\cert) \right)$.
    %\item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
}\fi
\end{definition}

\begin{corollary}
The scheme $\CD$-$\SSS = (\Share,\Rec,\Del,\Ver)$ defined as follows is a secret sharing scheme with certified deletion.
\begin{itemize}
    \item $\Share(m):$ sample $x,\theta \gets \{0,1\}^\secp$ and output \[s_1 \coloneqq \ket{x}_\theta,
    s_2 \coloneqq  \left(\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\right), \ \ \ \vk \coloneqq (x,\theta).\]
    \item $\Rec(s_1, s_2):$ parse $s_1 \coloneqq \ket{x}_\theta, s_2 \coloneqq \left(\theta,b'\right)$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(s_1):$ parse $s_1 \coloneqq \ket{x}_\theta$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}
\begin{proof}
    Correctness of deletion follows immediately from the description of the scheme. Certified deletion security, i.e. 
    \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp)\]
    follows by following the proof strategy of \cref{thm:main}. This setting is slightly different than the setting considered in the proof of \cref{thm:main} since here we consider unbounded $\cA_\secp$ that are not given access to $\theta$ while \cref{thm:main} considers bounded $\cA_\secp$ that are given access to an encryption of $\theta$. However, the proof is almost identical, defining hybrids as follows.
    \item $\Hyb_0(b):$ This is the distribution $\left\{\EVEXP_\secp^{\cA_\secp}(b)\right\}_{\secp \in \bbN}$ described above.
    
    \item $\Hyb_1(b):$ This distribution is sampled as follows.
    \begin{itemize}
        \item Prepare $\secp$ EPR pairs $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$ on registers $(\sC_1,\sA_1),\dots,(\sC_\secp,\sA_\secp)$. Define $\sC \coloneqq \sC_1,\dots,\sC_\secp$ and $\sA \coloneqq \sA_1,\dots,\sA_\secp$.
        \item Sample $\theta \gets \{0,1\}, b' \gets \{0,1\}$, measure register $\sC$ in basis $\theta$ to obtain $x \in \{0,1\}^\secp$, and initialize $\cA_{\secp}$ with register $\sA$.
        %and $\cA_{2,\secp}$ with $b',\theta$.
        \item If $b' = b \oplus \bigoplus_{i: \theta_i = 0} x_i$ then proceed as in $\Hyb_0$ and otherwise output $\bot$.
    \end{itemize}
    \item $\Hyb_2(b):$ This is the same as $\Hyb_1(b)$ except that measurement of register $\sC$ to obtain $x$ is performed after $\cA_{\secp}$ outputs $x'$ and $\rho$.
    
    Indistinguishability between these hybrids closely follows the proof of \cref{thm:main}. The key difference is that  $\Hyb_2'(b)$ is identical to $\Hyb_2(b)$ except that $s_2$ is set to $(b',0^\secp)$. Then, $\Pr[\Pi_{x',\theta},\Hyb_2'(b)] = \negl(\secp)$ follows identically to the proof in \cref{thm:main}, whereas 
    $\Pr[\Pi_{x',\theta},\Hyb_2(b)] = \negl(\secp)$ follows because the view of $\cA_{\secp}$ is identical in both hybrids.
    The final claim, that $\Advt(\Hyb_2) = \negl(\secp)$ follows identically to the proof in \cref{thm:main}.
    %instead of semantic security of $\cZ_\secp(\cdot)$, we rely on the fact that 
    %setting the distribution $\cZ_\secp(b)$ to be $\bot$ until before $\cA_\secp$ produces a certificate of deletion, and $\cZ_\secp(b) = b$ after, and setting the class of adversaries $\mathscr{A}$ to be all non-uniform families of QPT adversaries $\{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$.
\end{proof}

\begin{remark}[One-time pad encryption]
We observe that the above proof, which considers unbounded $\cA_\secp$ who don't have access to $\theta$ until after they produce a valid deletion certificate, can also be used to establish the security of a simple one-time pad encryption scheme with certified deletion. The encryption of a bit $b$ would be the state $\ket{x}_\theta$ together with a one-time pad encryption $k \oplus b \oplus \bigoplus_{i:\theta_i = 0}x_i$ with key $k \gets \{0,1\}$. The secret key would be $(k,\theta)$. Semantic security follows from the one-time pad, while certified deletion security follows from the above secret-sharing proof. This somewhat simplifies the construction of one-time pad encryption with certified deletion of \cite{10.1007/978-3-030-64381-2_4}, who required a seeded extractor.\end{remark}



\subsection{Public-key encryption}\label{subsec:PKE}

In this section, we define and construct post-quantum public-key encryption with certified deletion for classical messages, assuming the existence of post-quantum public-key encryption for classical messages.

\iffalse{
\paragraph{Semantic Security.}
First, consider a standard public-key encryption scheme $\PKE = (\Gen,\Enc,\Dec)$. We recall the definition of semantic security.

\begin{definition}[Semantic security]\label{def:semantic}
For any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$, it holds that \[\Bigg|\Pr\left[\cA_\secp(\ket{\psi_\secp},\pk,\ct) = 1 : \begin{array}{r}(\pk,\sk) \gets \Gen(1^\secp)\\ \ct \gets \Enc(\pk,0)\end{array}\right] - \Pr\left[\cA_\secp(\ket{\psi_\secp},\pk,\ct) = 1 : \begin{array}{r}(\pk,\sk) \gets \Gen(1^\secp)\\ \ct \gets \Enc(\pk,1)\end{array}\right]\Bigg| = \negl(\secp).\]
\end{definition}
}\fi

\paragraph{Public-Key encryption with certified deletion.}
First, we augment the standard syntax to include a deletion algorithm $\Del$ and a verification algorithm $\Ver$. Formally, consider a public-key encryption scheme $\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ with syntax

\begin{itemize}
    \item $\Gen(1^\secp) \to (\pk,\sk)$ is a classical algorithm that takes as input the security parameter and outputs a public key $\pk$ and secret key $\sk$.
    \item $\Enc(\pk,m) \to (\ct,\vk)$ is a quantum algorithm that takes as input the public key $\pk$ and a message $m$, and outputs a (potentially quantum) verification key $\vk$ and a quantum ciphertext $\ct$.
    \item $\Dec(\sk,\ct) \to \{m,\bot\}$ is a quantum algorithm that takes as input the secret key $\sk$ and a quantum ciphertext $\ct$ and outputs either a message $m$ or a $\bot$ symbol.
    \item $\Del(\ct) \to \cert$ is a quantum algorithm that takes as input a quantum ciphertext $\ct$ and outputs a (potentially quantum) deletion certificate $\cert$.
    \item $\Ver(\vk,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$ and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
\end{itemize}

We say that $\CD$-$\PKE$ satisfies correctness of deletion if the following holds.

\begin{definition}[Correctness of deletion]\label{def:CD-correctness}
$\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{correctness of deletion} if for any $m$, it holds with $1-\negl(\secp)$ probability over $(\pk,\sk) \gets \Gen(1^\secp), (\ct,\vk) \gets \Enc(\pk,m),\cert \gets \Del(\ct), \mu \gets \Ver(\vk,\cert)$ that $\mu = \top$.
\end{definition}

Next, we define certified deletion security. Our definition has multiple parts, which we motivate as follows. The first experiment is the everlasting security experiment, which requires that conditioned on the (computationally bounded) adversary producing a valid deletion certificate, their left-over state is information-theoretically independent of $b$. However, we still want to obtain meaningful guarantees against adversaries that do not produce a valid deletion certificate. That is, we hope for standard semantic security against arbitrarily malicious but computationally bounded adversaries. Since such an adversary can query the ciphertext generator with an arbitrarily computed deletion certificate, we should include this potential interaction in the definition, and require that the response from the ciphertext generator still does not leak any information about $b$.\footnote{One might expect that the everlasting security definition described above already captures this property, since whether the certificate accepts or rejects is included in the output of the experiment. However, this experiment does not include the output of the adversary in the case that the certificate is rejected. So we still need to capture the fact that the \emph{joint} distribution of the final adversarial state and the bit indicating whether the verification passes semantically hides $b$.} Note that, in our constructions, the verification key $\vk$ is actually completely independent of the plaintext $b$, and thus for our schemes this property follows automatically from semantic security.

\begin{definition}[Certified deletion security]\label{def:CD-security}
$\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp),\]
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
where the experiment $\EVEXP_\secp^{\cA}(b)$ considers everlasting security given a deletion certificate, and is defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$ and $(\ct,\vk) \gets \Enc(\pk,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
and the experiment $\CEXP_\secp^{\cA}(b)$ is a strengthening of semantic security, defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$ and $(\ct,\vk) \gets \Enc(\pk,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item Output $\cA_\secp \left(\rho, \Ver(\vk,\cert) \right)$.
    %\item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

Now we can formally define the notion of public-key encryption with certified deletion.

\begin{definition}[Public-key encryption with certified deletion]
$\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ is a secure \emph{public-key encryption scheme with certified deletion} if it satisfies (i) correctness of deletion (\cref{def:CD-correctness}), and (ii) certified deletion security (\cref{def:CD-security}).
\end{definition}

Then, we have the following corollary of \cref{thm:main}. %and \cref{thm:main-C}.

\begin{corollary}
Given any post-quantum semantically-secure public-key encryption scheme $\PKE = (\Gen,\Enc,\Dec)$, the scheme $\CD$-$\PKE = (\Gen,\Enc',\Dec',\Del,\Ver)$ defined as follows is a public-key encryption scheme with certified deletion.
\begin{itemize}
    \item $\Enc'(\pk,m):$ sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ct \coloneqq \left(\ket{x}_\theta,\Enc\left(\pk, \left(\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\right)\right)\right), \ \ \ \vk \coloneqq (x,\theta).\]
    \item $\Dec'(\sk,\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$, compute $(\theta,b') \gets \Dec(\sk,\ct')$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}

\begin{proof}
%Semantic security follows immediately from the semantic security of $\PKE$. 
Correctness of deletion follows immediately from the description of the scheme. For certified deletion security, we consider the following:
\begin{itemize}
\item First, we observe that 
\[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp)\]
follows from \cref{thm:main} and the semantic security of $\PKE$ by setting the distribution $\cZ_\secp(b)$ to sample $(\pk,\sk) \gets \Gen(1^\secp)$, $\ct \gets \Enc(\pk,b)$ and output $(\pk,\ct)$, and setting the class of adversaries $\mathscr{A}$ to be all non-uniform families of QPT adversaries $\{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$.
\item Next, we observe that \[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp)\]
follows from the fact that the encryption scheme remains (computationally) semantically secure even when the adversary is given the verification key $x$ corresponding to the challenge ciphertext, since the bit $b$ remains encrypted with $\Enc$.
\end{itemize}
This completes our proof.
\end{proof}
%
The notion of certified deletion security can be naturally generalized to consider multi-bit messages, as follows.

\begin{definition}[Certified deletion security for multi-bit messages]\label{def:CD-security-multi}
$\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp),\]
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
where the experiment $\EVEXP_\secp^{\cA}(b)$ considers everlasting security given a deletion certificate, and is defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$.
    Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and parse its output as $(m_0, m_1)$.
    \item Sample $(\ct,\vk) \gets \Enc(\pk,m_b)$.
    \item Run $\cA_\secp$ on input $\ct$ and parse $\cA_\secp$'s output as a deletion certificate $\cert$, and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
and the experiment $\CEXP_\secp^{\cA}(b)$ is a strengthening of semantic security, defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$.
    Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and parse its output as $(m_0, m_1)$.
    \item Sample $(\ct,\vk) \gets \Enc(\pk,m_b)$.
    \item Run $\cA_\secp$ on input $\ct$ and parse $\cA_\secp$'s output as a deletion certificate $\cert$, and a left-over quantum state $\rho$.
    \item Output $\cA_\secp \left(\rho, \Ver(\vk,\cert) \right)$.
    %\item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

A folklore method converts any public-key bit encryption scheme to a public-key string encryption scheme, by separately encrypting each bit in the underlying string one-by-one and appending all resulting ciphertexts. Semantic security of the resulting public-key encryption scheme follows by a hybrid argument, where one considers intermediate hybrid experiments that only modify one bit of the underlying plaintext at a time.
We observe that the same transformation from bit encryption to string encryption also preserves certified deletion security, and this follows by a similar hybrid argument. That is, as long as the encryption scheme for bits satisfies certified deletion security for single-bit messages per Definition~\ref{def:CD-security}, 
the resulting scheme for multi-bit messages 
satisfies certified deletion security according to Definition~\ref{def:CD-security-multi}.

%\begin{remark}
\paragraph{Attribute-based encryption with certified deletion.}
We observe that if the underlying scheme $\PKE$ is an \emph{attribute-based encryption} scheme, then the scheme with certified deletion that results from the above compiler inherits these properties. Thus, we obtain an attribute-based encryption scheme with certified deletion, assuming any standard (post-quantum) attribute-based encryption. The previous work of \cite{10.1007/978-3-030-92062-3_21} also constructs an attribute-based encryption scheme with certified deletion, but under the assumption of (post-quantum) indistinguishability obfuscation. We formalize our construction below.

We first describe the syntax of an attribute-based encryption scheme with certified deletion $\CD\text{-}\ABE = (\Gen,\KG,\Enc,\Dec,\Del,\Ver)$. This augments the syntax of an ABE scheme $\ABE = (\Gen,\KG,\Enc,\Dec)$ by adding the $\Del$ and $\Ver$ algorithms. 
Let $p = p(\secp)$ denote a polynomial.
\begin{itemize}
    \item $\Gen(1^\secp) \to (\pk,\msk)$ is a classical algorithm that takes as input the security parameter and outputs a public key $\pk$ and master secret key $\msk$.
    \item $\KG(\msk,P) \to \sk_P$ is a classical key generation algorithm that on input the master secret key and a predicate $P:\{0,1\}^{p(\secp)} \rightarrow \{0,1\}$, outputs a secret key $\sk_P$. 
    \item $\Enc(\pk, X, m) \rightarrow (\ct_X,\vk)$ is a quantum algorithm that on input a message $m$ and an attribute $X$ outputs a (potentially quantum) verification key $\vk$ and quantum ciphertext $\ct_X$.
    \item $\Dec(\sk_P, \ct_X) \to \{m',\bot\}$ on input a secret key $\sk_P$ and a quantum ciphertext $\ct_X$ outputs either a message $m'$ or a $\bot$ symbol.
    \item $\Del(\ct) \to \cert$ is a quantum algorithm that takes as input a quantum ciphertext $\ct$ and outputs a (potentially quantum) deletion certificate $\cert$.
    \item $\Ver(\vk,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$ and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
\end{itemize}
Correctness of decryption for $\CD\text{-}\ABE$ is the same as that for $\ABE$. We define correctness of deletion, and certified deletion security for $\CD\text{-}\ABE$ below. 


\begin{definition}[Correctness of deletion]
$\CD$-$\ABE = (\Gen,\KG,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{correctness of deletion} if for any $m,X$, it holds with $1-\negl(\secp)$ probability over $(\pk,\msk) \gets \Gen(1^\secp), (\ct,\vk) \gets \Enc(\pk,X,m),\cert \gets \Del(\ct), \mu \gets \Ver(\vk,\cert)$ that $\mu = \top$.
\end{definition}

\begin{definition}[Certified deletion security]
\label{def:CD-sec-ABE}
$\CD$-$\ABE = (\Gen,\KG,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp),\] 
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\] 
where the experiments $\EVEXP_\secp^{\cA}(b)$ and $\CEXP_\secp^{\cA}(b)$ are defined as follows.
Both experiments take an input $b$, and interact with $\cA$ as follows.
\begin{itemize}
    \item Sample $(\pk,\msk) \gets \Gen(1^\secp)$
    and %send $\pk$ to $\cA$.
    %and $(\ct,\vk) \gets \Enc(\pk,b)$.
    %\item Initialize 
    initialize
    $\cA_\secp(\ket{\psi_\secp})$ with $\pk$.
    %and $\ct$.
    \item Set $i = 1$.
    \item If $\cA_\secp$ outputs a key query $P_i$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ and set $i = i + 1$. This process can be repeated polynomially many times.
    \item If $\cA_\secp$ outputs an attribute $X^*$ and a pair of messages $(m_0, m_1)$ where $P_i(X^*) = 0$ for all predicates $P_i$ queried so far, then compute $(\vk,\ct) = \Enc(\pk, X^*, m_b)$ and return $\ct$ to $\cA_\secp$, else exit and output $\bot$.
    \item If $\cA_\secp$ outputs a key query $P_i$ such that $P_i(X^*) = 0$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ (otherwise return $\bot$) and set $i = i + 1$. This process can be repeated polynomially many times.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ then $\EVEXP_\secp^{\cA}(b)$ outputs $\rho$, and otherwise $\EVEXP_\secp^{\cA}(b)$ outputs $\bot$, and ends.
    \item $\CEXP_\secp^{\cA}(b)$ sends the output $\Ver(\vk,\cert)$ to $\cA_\secp$. Again, upto polynomially many times, $\cA_\secp$ sends key queries $P_i$. For each $i$, if $P_i(X^*) = 0$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ (otherwise return $\bot$) and set $i = i + 1$.
    Finally, $\cA_\secp$ generates an output bit, which is set to be the output of $\CEXP_\secp^{\cA}(b)$.
    %$\CEXP_\secp^{\cA}(b)$ outputs $(\rho, \Ver(\vk,\cert))$.
\end{itemize}
\end{definition}

\begin{corollary}
Given any post-quantum attribute-based encryption scheme $\ABE = (\Gen,\KG,\Enc,\Dec)$, the scheme $\CD$-$\ABE = (\Gen,\KG,\Enc',\Dec',\Del,\Ver)$ defined as follows is an attribute-based encryption scheme with certified deletion.
\begin{itemize}
    \item $\Enc'(\pk,X,m):$ sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ct \coloneqq \left(\ket{x}_\theta,\Enc\left(\pk, X, \left(\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\right)\right)\right), \ \ \ \vk \coloneqq (x,\theta).\]
    \item $\Dec'(\sk_P,\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$, compute $(\theta,b') \gets \Dec(\sk_P,\ct')$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}
\begin{proof}
Correctness of decryption and deletion follow from the description of the scheme. For certified deletion security, we consider the following:
\begin{itemize}
\item First, we observe that 
\[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp)\]
follows from \cref{thm:main} and the semantic security of $\ABE$. To see this, we imagine splitting $\cA_\secp$ into two parts: $\cA_{\secp,0}$ which interacts in the $\ABE$ security game until it obtains its challenge ciphertext and all the keys $\sk_{P_i}$ that it wants, and $\cA_{\secp,1}$ which takes the final state of $\cA_{\secp,0}$ and produces a deletion certificate $\cert$ and final state $\rho$. We set the distribution $\cZ_\secp(b)$ to run the $\EVEXP_\secp^{\cA_\secp}(b)$ game with $\cA_{\secp,0}(\ket{\psi_\secp})$, and output $\cA_{\secp,0}$'s final state. Then, we set the class of adversaries $\mathscr{A}$ to include all $\cA_{\secp,1}$, which is the class of all  uniform families of QPT adversaries. By the semantic security of $\ABE$, $\cA_{\secp,1}$ cannot distinguish between $\cZ_\secp(0)$ and $\cZ_{\secp}(1)$, and thus the guarantees of \cref{thm:main} apply.
\item Next, we observe that \[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp)\]
follows from the fact that the encryption scheme remains semantically secure even when the adversary is given the verification key corresponding to the challenge ciphertext.
\end{itemize}
This completes our proof.
\end{proof}



\begin{remark}
Similarly to the setting of public-key encryption, single-bit certified deletion security for ABE implies multi-bit certified deletion security.
\end{remark}

\paragraph{Relation with  \cite{10.1007/978-3-030-92062-3_21}'s definitions.} 
%\dakshita{todo formalize}
The definition of certified deletion security for public-key (resp., attribute-based) encryption in \cite{10.1007/978-3-030-92062-3_21} is
different than our definition in two primary respects: (1) it only considers \emph{computationally-bounded} adversaries even after the deletion certificate is computed, and (2) explicitly gives the adversary the secret key $\sk$ after the deletion certificate is computed.

Our definition allows the adversary to be unbounded after deletion, which gives a strong \emph{everlasting security} property. 
Indeed, in Appendix \ref{sec:implication}, we show that our definition implies \cite{10.1007/978-3-030-92062-3_21}'s definition for public-key (attribute-based) encryption schemes.
%To see this, we first note that our notion of security is trivially equivalent to a definition that hands the output of $\EXP_\secp^\cA(b)$ for a uniformly random bit $b$ to an unbounded distinguisher, and requires that any such distinguisher can only guess $b$ with probability $1/2 + \negl(\secp)$. Now, 
To see this, we consider any adversary $\cA$ that contradicts \cite{10.1007/978-3-030-92062-3_21}'s notion of security and construct a reduction $\cR$ that contradicts our notion of security. $\cR$ will run $\cA$ on the challenge that it receives from its challenger, and forward the deletion certificate $\cert$ received from $\cA$. $\cR$ will then, in unbounded time, reverse sample a $\sk$ such that $(\pk,\sk)$ is identically distributed to the output of the honest $\Gen$ algorithm. Finally, $\cR$ runs $\cA$ on $\sk$ to obtain $\cA$'s guess for $b$. We can show that the view of $\cA$ produced by such an $\cR$ matches its view in the \cite{10.1007/978-3-030-92062-3_21} challenge, thus the
advantage of $\cR$ in contradicting our definition will match that of $\cA$ in contradicting~\cite{10.1007/978-3-030-92062-3_21}'s definition.


\paragraph{Witness encryption for NP with certified deletion.}
Finally, we observe that if the underlying scheme $\PKE$ is a \emph{witness encryption} scheme, then the scheme with certified deletion that results from the above compiler becomes a witness encryption scheme with certified deletion. That is, we compile any (post-quantum) witness encryption into a witness encryption scheme with certified deletion.
Similar to the case of PKE and ABE, we can augment the syntax of any witness encryption scheme to include a deletion algorithm $\mathsf{Del}$ and a verification algorithm $\mathsf{Ver}$.
That is, the scheme consists of algorithms $(\mathsf{Enc}, \mathsf{Dec})$ with syntax and properties identical to standard witness encryption schemes~\cite{STOC:GGSW13}, except where the ciphertexts are potentially quantum, and where the encryption algorithm outputs a (potentially quantum) verification key $\mathsf{vk}$ along with a ciphertext.
$\Ver(\vk,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$ and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
$\mathsf{Del}(\mathsf{ct}) \rightarrow \mathsf{cert}$ is a quantum algorithm that on input a quantum ciphertext $\mathsf{ct}$ outputs a (potentially quantum) deletion certificate $\mathsf{cert}$.

Correctness of decryption is the same as that for (regular) witness encryption. We define correctness of deletion, and certified deletion security for $\CD\text{-}\WE$ below. 


\begin{definition}[Correctness of deletion]
$\CD$-$\WE = (\Enc,\Dec,\Del,\Ver)$ satisfies \emph{correctness of deletion} if for every statement $X$ and message $m$, it holds with $1-\negl(\secp)$ probability over $(\ct,\vk) \gets \Enc(X,m),\cert \gets \Del(\ct), \mu \gets \Ver(\vk,\cert)$ that $\mu = \top$.
\end{definition}

\begin{definition}[Certified deletion security]
\label{def:CD-sec-ABE}
$\CD$-$\WE = (\Enc,\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, there is a negligible function $\negl(\cdot)$ for which it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp),\] 
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\] 
where the experiments $\EVEXP_\secp^{\cA}(b)$ and $\CEXP_\secp^{\cA}(b)$ are defined as follows.
Both experiments take an input $b$, and interact with $\cA$ as follows.
\begin{itemize}
    \item Obtain statement $X$, language $\cL$ and messages $(m_0, m_1)$ from $\cA_\secp(\ket{\psi}_\secp)$. If $X \in L$, abort, otherwise continue.
    \item Set $(\ct,\vk) \gets \Enc(X,m_b)$.
    \item Run $\cA_\secp$ on input $\ct$ and parse $\cA_\secp$'s output as a deletion certificate $\cert$, and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
and the experiment $\CEXP_\secp^{\cA}(b)$ is a strengthening of semantic security, defined as follows.
\begin{itemize}
    \item Obtain statement $X$, language $\cL$ and messages $(m_0, m_1)$ from $\cA_\secp(\ket{\psi}_\secp)$. If $X \in L$, abort, otherwise continue.
    \item Set $(\ct,\vk) \gets \Enc(X,m_b)$.
    \item Run $\cA_\secp$ on input $\ct$ and parse $\cA_\secp$'s output as a deletion certificate $\cert$, and a left-over quantum state $\rho$.
    \item Output $\cA_\secp \left(\rho, \Ver(\vk,\cert) \right)$.
    %\item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

\begin{corollary}
Given any post-quantum semantically-secure witness encryption scheme $\WE = (\Enc,\Dec)$, the scheme $\CD$-$\WE = (\Enc',\Dec',\Del,\Ver)$ defined as follows is a witness encryption scheme with certified deletion.
\begin{itemize}
    \item $\Enc'(X,m):$ sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ct \coloneqq \left(\ket{x}_\theta,\Enc\left(X, \left(\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\right)\right)\right), \ \ \ \vk \coloneqq (x,\theta).\]
    \item $\Dec'(W,\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$, compute $(\theta,b') \gets \Dec(W,\ct')$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}

\begin{proof}
%Semantic security follows immediately from the semantic security of $\PKE$. 
Correctness of deletion follows immediately from the description of the scheme. For certified deletion security, we consider the following:
\begin{itemize}
\item First, we observe that 
\[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP_\secp^{\cA}(1)\right) = \negl(\secp)\]
follows from \cref{thm:main} and the semantic security of $\WE$ by setting the distribution $\cZ_\secp(b)$ to sample $\ct \gets \Enc(X,b)$ and output $(X,\ct)$, and setting the class of adversaries $\mathscr{A}$ to be all non-uniform families of QPT adversaries $\{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$.
\item Next, we observe that \[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp)\]
follows from the fact that the witness encryption scheme remains (computationally) semantically secure even when the adversary is given the verification key corresponding to the challenge ciphertext.
\end{itemize}
This completes our proof.
\end{proof}



\subsection{Fully-homomorphic encryption}


Next, we consider the syntax of a \emph{fully-homomorphic encryption} scheme (for classical circuits) with certified deletion. Such a scheme consists of algorithms $\CD$-$\FHE$ = ($\CD$-$\FHE.\Gen$, $\CD$-$\FHE.\Enc$, $\CD$-$\FHE.\Eval$, $\CD$-$\FHE.\Dec$, $\CD$-$\FHE.\Del$, $\CD$-$\FHE.\Ver$) with the same syntax as $\CD$-$\PKE$ (\cref{subsec:PKE}), but including the additional algorithm $\CD$-$\FHE.\Eval$.
\begin{itemize}
    \item $\CD$-$\FHE.\Eval(\pk,C,\ct) \to \widetilde{\ct}:$ On input the public key $\pk$, a classical circuit $C$, and a quantum ciphertext $\ct$, the evaluation algorithm returns a (potentially quantum) evaluated ciphertext $\widetilde{\ct}$.
\end{itemize}

We say that $\CD$-$\FHE$ satisfies evaluation correctness if the following holds.

\begin{definition}[$\CD$-$\FHE$ evaluation correctness]\label{def:eval-correctness}
A $\CD$-$\FHE$ scheme satisfies evaluation correctness if for any message $x$, and all polynomial-size circuits $C$, it holds with $1-\negl(\secp)$ probability over $(\pk,\sk) \gets \CD$-$\FHE.\Gen(1^\secp), \ct \gets \CD$-$\FHE.\Enc(\pk,x)$, $\widetilde{\ct} \gets \CD$-$\FHE.\Eval(\pk,C,\ct), y \gets \CD$-$\FHE.\Dec(\sk,\widetilde{\ct})$ that $y = C(x)$.
\end{definition}

Now we can formally define the notion of fully-homomorphic encryption with certified deletion.

\begin{definition}[Fully-homomorphic encryption with certified deltion]
$\CD$-$\FHE$ = ($\CD$-$\FHE.\Gen$, $\CD$-$\FHE.\Enc$, $\CD$-$\FHE.\Eval$, $\CD$-$\FHE.\Dec$, $\CD$-$\FHE.\Del$, $\CD$-$\FHE.\Ver$) is a secure \emph{fully-homomorphic encryption scheme with certified deletion} if it satisfies 
%(i) semantic security (\cref{def:semantic}), 
(i) correctness of deletion (\cref{def:CD-correctness}), (ii) certified deletion security (\cref{def:CD-security}), and (iii) evaluation correctness (\cref{def:eval-correctness}).
\end{definition}



\subsubsection{Blind delegation with certified deletion} 

So far, we have described a $\PKE$ scheme with certified deletion augmented with a procedure that allows for homomorphic evaluation over ciphertexts. A fascinating application for such a scheme, as discussed by \cite{10.1007/978-3-030-64381-2_4,cryptoeprint:2022:295}, is the following. A computationally weak client wishes to use the resources of a powerful server to peform some intensive computation $C$ on their input data $x$. However, they would like to keep $x$ private from the server, and, moreover, they would like to be certain that their data is \emph{deleted} by the server after the computation takes place. Here, by deleted, we mean that the original input $x$ becomes \emph{information-theoretically} hidden from the server after the computation has taken place.

While it is not necessarily clear from the syntax described so far that the server can both compute on \emph{and later} delete the client's input data, we demonstrate, via an interaction pattern described by \cite{cryptoeprint:2022:295}, a protocol that achieves this functionality. We refer to such a protocol as a ``blind delegation with certified deletion'' protocol, and describe it in \proref{fig:private-delegation}.

\protocol{Blind delegation with certified deletion}{A generic construction of blind delegation with certified deletion, from any $\CD$-$\FHE$ scheme.}{fig:private-delegation}{
\begin{itemize}
    \item Parties: client with input $x$, and server.
    \item Ingredients: a $\CD$-$\FHE$ scheme.
\end{itemize}

\underline{Encryption phase}
\begin{itemize}
    \item The client samples $(\pk,\sk) \gets \CD$-$\FHE.\Gen(1^\secp)$, $(\ct,\vk) \gets \CD$-$\FHE.\Enc(\pk,x)$ and sends $(\pk,\ct)$ to the server.
\end{itemize}

\underline{Computation phase} (this may be repeated arbitrarily many times)
\begin{itemize}
    \item The client sends the description of a circuit $C$ to the server.
    \item The server runs the algorithm $\CD$-$\FHE.\Eval(\pk,\ct,C)$ \emph{coherently}. Let $\sO$ be the (unmeasured) register that holds the output ciphertext $\widetilde{\ct}$. Send $\sO$ to the client.
    \item The client runs $\CD$-$\FHE.\Dec(\sk,\cdot)$ \emph{coherently} on register $\sO$, and then measures the output register of this computation in the standard basis to obtain the output $y$. Then, it reverses the computation of $\CD$-$\FHE.\Dec(\sk,\cdot)$ and sends the register $\sO$ back to the server.
    \item The server reverses the computation of $\CD$-$\FHE.\Eval(\pk,\ct,C)$ to obtain the original input $(\pk,\ct,C)$.
\end{itemize}

\underline{Deletion phase}
\begin{itemize}
    \item The server runs $\cert \gets \CD$-$\FHE.\Del(\ct)$ and sends $\cert$ to the client.
    \item The client runs $\Ver(\vk,\cert)$ and outputs the result ($\top$ or $\bot$).
\end{itemize}
}


A blind delegation with certified deletion protocol should satisfy the following notions of correctness and security. We present each definition for the case of a single circuit $C$ queried by the client (one repetition of the computation phase), but they easily extend to considering multiple repetitions of the computation phase.

\begin{definition}[Correctness for blind delegation with certified deletion]\label{def:delegation-correctness}
A blind delegation with certified deletion protocol is \emph{correct} if the honest client and server algorithms satisfy the following properties. First, for any $x,C$, the client obtains $y = C(x)$ after the computation with probability $1-\negl(\secp)$. Second, for any $x,C$, the client outputs $\top$ after the deletion phase with probability $1-\negl(\secp)$.
\end{definition}

\begin{definition}[Security for blind delegation with certified deletion]\label{def:delegation-security}
A blind delegation with certified deletion protocol is \emph{secure} against a class of adversarial servers $\mathscr{S}$ if for any $x_0,x_1$, circuit $C$, and $\{\cS_{\secp}\}_{\secp \in \bbN} \in \mathscr{S}$, the following two properties hold.
\begin{itemize}
    \item \textbf{Privacy:} For any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, it holds that \[\bigg|\Pr\left[\cD_\secp(\rho^{\sS}_{x_0,C}) = 1\right] - \Pr\left[\cD_\secp(\rho^{\sS}_{x_1,C}) = 1\right]\bigg| = \negl(\secp),\] where $\rho^{\sS}_{x,C} \gets \langle \cC(x,C),\cS_\secp \rangle$ is the output state of adversary $\cS_\secp$ after interacting (in the Encryption, Computation, and Delete phases) with an honest client $\cC$ with input $x$ and circuit $C$.
    \item \textbf{Certified deletion:} It holds that \[\TD\left(\EVEXP_\secp^{\cS}(x_0,C),\EVEXP_\secp^{\cS}(x_1,C)\right) = \negl(\secp),\] where the experiment $\EVEXP_\secp^{\cS}(x,C)$ is defined as follows.
    \begin{itemize}
        \item Run the Encryption, Computation, and Deletion phases between client $\cC(x,C)$ and server $\cS_\secp$, obtaining the server's final state $\rho^{\sS}_{x,C}$ and the client's decision $\top$ or $\bot$. If $\top$ output $\rho^{\sS}_{x,C}$, and otherwise output $\bot$.
    \end{itemize}
\end{itemize}
\end{definition}

Next, we define a class of adversaries $\mathscr{S}$ that we call \emph{evaluation-honest}. The defining feature of an evaluation-honest adversary $\{\cS_\secp\}_{\secp \in \bbN}$ is that, for any client input $x$ and circuit $C$, the state on register $\sO$ returned by $\cS_\secp$ during the Computation phase is within negligible trace distance of the state on register $\sO$ returned by the \emph{honest} server. Otherwise, $\cS_\secp$ may be arbitrarily malicious, including during the Deletion phase and after. Morally, evaluation-honest adversaries are those that are \emph{specious} \cite{C:DupNieSal10} (which is a quantum analogue of semi-honest) during the Computation phase, and \emph{malicious} afterwards.\footnote{Roughly, a specious adversary is one who may, at any step of the computation, apply an operation to their private state such that the joint state of the resulting system is negligibly close to the joint state of an honest interaction. Note that for any specious adversary, the registers they send to the honest party during any round must be negligibly close to the register sent by the honest party during this round, since after transmission, this register is no longer part of their private state. Thus, our definition of evaluation-honest adversaries includes all specious adversaries. }

Then, we have the following theorem.

\begin{theorem}
When instantiated with any $\CD$-$\FHE$ scheme, \proref{fig:private-delegation} is a blind delegation with certified deletion scheme, secure against any \emph{evaluation-honest} adversarial server $\{\cS^*_{\secp}\}_{\secp \in \bbN}$. 
\end{theorem}

\begin{proof}
First, we argue that correctness (\cref{def:delegation-correctness}) holds. The evaluation correctness of the underlying $\CD$-$\FHE$ scheme (\cref{def:eval-correctness}) implies that the register measured by the client during the computation phase is within negligible trace distance of $\ket{y}$ for $y = C(x)$. This implies the first property of correctness for blind delegation with certified deletion, and it also implies that the state on register $\sO$ returned to the server is negligibly close to the original state on register $\sO$. So, after reversing the computation, the server obtains a $\ct'$ that is negligibly close to the original $\ct$ received from the client. Thus, the second property of correctness for blind delegation with certified deletion follows from the correctness of deletion property of $\CD$-$\FHE$ (\cref{def:CD-correctness}).

Next, we argue that security (\cref{def:delegation-security}) holds against any evaluation-honest server $\{\cS^*_\secp\}_{\secp \in \bbN}$. Consider a hybrid experiment in which there is no interaction between client and server during the Computation phase, that is, the register $\sO$ is not touched by the client and is immediately return the the server. By the evaluation-honesty of the server, and the above arguments, it follows that the server's view of this hybrid experiment is negligibly close to its view of the real interaction. But now observe that this hybrid experiment is equivalent to the experiment described in \cref{def:CD-security-multi} for defining certified deletion security for standard public-key encryption for multi-bit messages. Thus, the Privacy and Certified Deletion properties of blind delegation follow directly from the certified deletion properties (\cref{def:CD-security-multi}) of the underlying $\CD$-$\FHE$ scheme.
\end{proof}

\subsubsection{Construction of $\CD$-$\FHE$} 

Now, to obtain a blind delegation with certified deletion protocol, it suffices to construct a $\CD$-$\FHE$ scheme. In this section, we show that such a scheme follows from a standard fully-homorphic encryption scheme, and our main theorem. 

%First, we define an appropriate notion of quantum fully-homomorphic encryption.

%\paragraph{Quantum fully-homomorphic encryption.} We consider a flavor of quantum fully-homomorphic encryption (QFHE) that supports encryption of classical messages, and evaluation of quantum circuits $Q(\ket{\psi},\cdot)$, where $Q$ is a quantum operation that is applied to some quantum state $\ket{\psi}$ and classical input $x$, and outputs a classical string $y$. Such a scheme consists of algorithms $\QFHE = (\QFHE.\Gen,\allowbreak\QFHE.\Enc,\allowbreak \QFHE.\Eval,\allowbreak \QFHE.\Dec)$ with the following syntax.

%\begin{itemize}
    %\item $\QFHE.\Gen(1^\lambda) \to (\pk,\sk)$: On input the security parameter $1^\secp$, the key generation algorithm outputs a public key $\pk$ and secret key $\sk$.
    %\item $\QFHE.\Enc(\pk, x) \to \ct$: On input the public key $\pk$ and a message $x$, the encryption algorithm outputs a ciphertext $\ct$.
    %\item $\QFHE.\Eval(\pk, Q(\ket{\psi},\cdot), \ct) \to \widetilde{\ct}$: On input the public key $\pk$, a quantum circuit $Q$, a quantum state $\ket{\psi}$, and a ciphertext $\ct$, the evaluation algorithm outputs an evaluated  ciphertext $\widetilde{\ct}$.
    %\item $\QFHE.\Dec(\sk, \widetilde{\ct}) \to \{y,\bot\}$: On input the secret key $\sk$ and a ciphertext $\ct$, the decryption algorithm outputs either a message $y$ or a $\bot$ symbol.
%\end{itemize}


%Analogously to the classical case~\cite{STOC:Gentry09}, we say that the scheme is fully homomorphic if the evaluation algorithm supports all polynomial-size quantum circuits. We say that the scheme is leveled if the maximum depth of the homomorphically evaluated circuits is bounded by the key generation algorithm (formally, the key generation algorithm takes as input an additional $1^d$ depth parameter). In this work, we are only interested in levelled schemes, so we drop the adjective wherever it is clear from the context. Next we define the notion of (single-hop) evaluation correctness for QFHE.

%A quantum fully-homomorphic encryption scheme should satisfy standard semantic security, plus the following correctness guarantee.

%\begin{definition}[$\QFHE$ evaluation correctness]
%A $\QFHE$ scheme satisfies evaluation correctness if for all messages $x$, and all polynomial-size circuits $Q(\ket{\psi},\cdot)$, the distribution over output $y \gets C(\ket{\psi},x)$ is within negligible statistical distance of the following random variable: sample $(\pk,\sk) \gets \QFHE.\Gen(1^\secp)$, encrypt $\ct \gets \QFHE.\Enc(\pk,x)$, evalute $\widetilde{\ct} \gets \QFHE.\Eval(\pk,Q(\ket{\psi},\cdot),\ct)$, decrypt and output $y \gets \QFHE.\Dec(\sk,\widetilde{\ct})$.
%\end{definition}

%We remark that (levelled)\footnote{``Levelled'' refers to the requirement that a bound on the depth of circuits to be evaluated must be known when generating the parameters and ciphertext. One can also relax this requirement by additionally assuming a particular circular-security property.} $\QFHE$ schemes satisfying the above requirements are known from the learning with errors assumption \cite{FOCS:Mahadev18b,C:Brakerski18}.

%We now state a corollary of \cref{thm:main}.

\begin{corollary}
Given any classical fully-homomorphic encryption scheme $\FHE = (\FHE.\Gen,\allowbreak\FHE.\Enc,\allowbreak \FHE.\Eval,\allowbreak \FHE.\Dec)$, the scheme defined below $\CD$-$\FHE$ = $(\FHE.\Gen,\Enc,\Eval,\Dec,\allowbreak\Del,\Ver)$ is an $\FHE$ scheme with certified deletion. We define encryption, decryption, deletion, and verification for one-bit plaintexts, and evaluation over ciphertexts encrypting $n$ bits (which is simply a concatenation of $n$ ciphertexts each encrypting one bit).
\begin{itemize}
    \item $\Enc(\pk,b):$ Sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ct \coloneqq \left(\ket{x}_{\theta},\FHE.\Enc\left(\theta,b \oplus \bigoplus_{i: \theta_{i} = 0} x_{i}\right)\right), \ \ \ \vk \coloneqq (x,\theta).\] 
    \item $\Eval(\pk,C,\ct):$ Parse $\ct \coloneqq (\ket{x_1}_{\theta_1},\ct'_1),\dots,(\ket{x_n}_{\theta_n},\ct'_n)$. Consider the circuit $\widetilde{C}$ that takes $(x'_1,\theta_1,b_1'),\dots,(x'_n,\theta_n,b_n')$ as input, for each $i \in [n]$ computes $b_i = b_i' \oplus \bigoplus_{j:\theta_{i,j} = 0}x'_j$, and then computes and outputs $C(b_1,\dots,b_n)$. Then, apply $\widetilde{C}$ homomorphically in superposition to $\ct$ to obtain $\widetilde{\ct}$. Optionally, measure $\widetilde{\ct}$ in the standard basis to obtain a classical output ciphertext.
    
    
    
    
    %Define the quantum circuit $Q_C((\ket{x_1}_{\theta_1},\allowbreak\dots,\allowbreak\ket{x_n}_{\theta_n}),\cdot)$ to take a classical input $(\theta_1,b'_1),\dots,(\theta_n,b'_n)$, then for each $j \in [n]$ measure $\ket{x_j}_{\theta_j}$ in the $\theta_j$ basis to obtain $x_j$ and compute $b_j = b_j' \oplus \bigoplus_{i:\theta_{j,i} = 0}x_{j,i}$, and finally set $m = (b_1,\dots,b_n)$ and compute and output $C(m)$. Compute and output $\widetilde{\ct} \gets \QFHE.\Eval(\pk,Q_C((\ket{x_1}_{\theta_1},\dots,\ket{x_n}_{\theta_n}),\cdot),\ct)$.
    \item $\Dec(\sk,\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$, compute $(\theta,b') \gets \FHE.\Dec(\sk,\ct')$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}

\begin{proof}
Semantic security follows immediately from the semantic security of $\FHE$. Correctness of deletion follows immediately by definition the scheme. Certified deletion security follows from \cref{thm:main} and the semantic security of $\FHE$ by setting the distribution $\cZ_\secp(b)$ to sample $(\pk,\sk) \gets \FHE.\Gen(1^\secp)$, $\ct \gets \FHE.\Enc(\pk,b)$ and output $(\pk,\ct)$, and setting the class of adversaries $\mathscr{A}$ to be all non-uniform families of QPT adversaries $\{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$.
\end{proof}


\input{fe}



\subsection{Commitments and zero-knowledge}\label{subsec:com-ZK}


A bit commitment scheme is an interactive protocol between two (potentially quantum) interactive machines, a committer $\cC = \{\cC_{\Com,\secp},\cC_{\Rev,\secp}\}_{\secp \in \bbN}$ and a receiver $\cR = \{\cR_{\Com,\secp},\cR_{\Rev,\secp}\}_{\secp \in \bbN}$. It operates in two stages.

\begin{itemize}
    \item In the Commit phase, the committer $\cC_{\Com,\secp}(b)$ with input bit $b$ interacts with the receiver $\cR_{\Com,\secp}$. This interaction results in a joint state on a committer and receiver register, which we denote $(\sC,\sR) \gets \Com\langle \cC_{\Com,\secp}(b),\allowbreak\cR_{\Com,\secp} \rangle$.
    \item In the Reveal phase, the parties continue to interact, and the receiver outputs a trit $\mu \in \{0,1,\bot\}$, which we denote by $\mu \gets \Rev\langle \cC_{\Rev,\secp}(\sC),\cR_{\Rev,\secp}(\sR)\rangle$.
    
    %, or after the Delete phase, which we denote by $\mu \gets \Rev\langle \cC_{\Rev,\secp},\cR_{\Rev,\secp},\rho_d^{\sC,\sR}\rangle$.
\end{itemize}

A commitment scheme that is \emph{statistically binding and computationally hiding} is one that satisfies the following three properties.

\begin{definition}[Correctness of decommitment]\label{def:correctness-decommitment}
A commitment scheme satisfies \emph{correctness of decommitment} if for any $b \in \{0,1\}$, it holds with overwhelming probability over $(\sC,\sR) \gets \Com\langle\cC_{\Com,\secp}(b),\allowbreak\cR_{\Com,\secp}\rangle, \mu \gets \Rev\langle\cC_{\Rev,\secp}(\sC),\cR_{\Rev,\secp}(\sR)\rangle$ that $\mu = b$.
\end{definition}

\begin{definition}[Computational hiding]\label{def:comp-hiding}
A commitment scheme satisfies \emph{computational hiding} if for any non-uniform QPT adversary and distinguisher $\cR^* = \{\cR^*_{\Com,\secp},\cD^*_{\secp},\ket{\psi_\secp}\}_{\secp \in \bbN}$, where $\ket{\psi_\secp}$ is a state on two registers $(\sR^*,\sD^*)$, it holds that 
\begin{align*}
    &\bigg|\Pr\left[\cD^*_\secp(\sR^*,\sD^*) = 1 : (\sC,\sR^*) \gets \Com\langle\cC_{\Com,\secp}(0),\cR^*_{\Com,\secp}(\sR^*)\rangle \right] \\ &- \Pr\left[\cD^*_\secp(\sR^*,\sD^*) = 1 : (\sC,\sR^*) \gets \Com\langle\cC_{\Com,\secp}(1),\cR^*_{\Com,\secp}(\sR^*)\rangle \right]\bigg| = \negl(\secp).
\end{align*}
\end{definition}

We follow \cite{cryptoeprint:2021:1663}'s notion of statistical binding, which asks for an unbounded extractor that obtains the committer's bit during the Commit phase.

\begin{definition}[Statistical binding]\label{def:SB}
A commitment scheme satisfies \emph{statistical binding} if for any unbounded adversary $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase, there exists an unbounded extractor $\cE = \{\cE_\secp\}_{\secp \in \bbN}$ such that for every unbounded adversary $\{\cC^*_{\Rev,\secp}\}_{\secp \in \bbN}$ in the Reveal phase, \[\TD\left(\Real_\secp^{\cC^*},\Ideal_\secp^{\cC^*,\cE}\right) = \negl(\secp),\] where $\Real_\secp^{\cC^*}$ and $\Ideal_\secp^{\cC^*,\cE}$ are defined as follows.
\begin{itemize}
    \item $\Real_\secp^{\cC^*}$: Execute the Commit phase $(\sC^*,\sR) \gets \Com\langle \cC^*_{\Com,\secp},\cR_{\Com,\secp}\rangle$. Execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the updated committer's state on register $\sC^*$. Output $(\mu,\sC^*)$.
    \item $\Ideal_\secp^{\cC^*,\cE}$: Run the extractor $(\sC^*,\sR,b^*) \gets \cE_\secp$, which outputs a joint state on registers $\sC^*,\sR$ along with a bit $b^*$. Next, execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle \cC^*_{\Rev,\secp}(\sC^*),\cR_{\Rev,\secp}(\sR)\rangle$ along with the updated committer's state on register $\sC^*$. If $\mu \in \{\bot,b^*\}$ output $(\mu,\sC^*)$, and otherwise output a special symbol $\Fail$.
\end{itemize}
\end{definition}


We will also consider commitment schemes with an additional (optional) \emph{Delete} phase. That is, the committer and receiver will be written as three components: $\cC_\secp = \{\cC_{\Com,\secp},\cC_{\Del,\secp},\cC_{\Rev,\secp}\}$, and $\cR_\secp = \{\cR_{\Com,\secp},\cR_{\Del,\secp},\cR_{\Rev,\secp}\}$, and the protocol proceeds as follows.

\begin{itemize}
    \item In the Commit phase, the committer $\cC_{\Com,\secp}(b)$ with input bit $b$ interacts with the receiver $\cR_{\Com,\secp}$. This interaction results in a joint state on a committer and receiver register, which we denote $(\sC,\sR) \gets \Com\langle \cC_{\Com,\secp}(b),\allowbreak\cR_{\Com,\secp} \rangle$.
    \item In the Delete phase, the parties continue to interact. The committer outputs a bit $d_\cC \in \{\top,\bot\}$ indicating whether they accept or reject. We denote the resulting output and joint state of the committer and receiver by $(d_\cC,\sC,\sR) \gets \Del\langle \cC_{\Del,\secp}(\sC),\cR_{\Del,\secp}(\sR)\rangle$.
    \item The Reveal phase is only executed if the Delete phase has not been executed, and the receiver outputs a trit $\mu \in \{0,1,\bot\}$, which we denote by $\mu \gets \Rev\langle \cC_{\Rev,\secp}(\sC),\cR_{\Rev,\secp}(\sR)\rangle$.
    
    
    %and the receiver outputs a trit $\mu \in \{0,1,\bot\}$. The parties may run this phase either directly after the Commit phase, which we denote by $\mu \gets \Rev\langle \cC_{\Rev,\secp},\cR_{\Rev,\secp},\rho_c^{\sC,\sR}\rangle$, or after the Delete phase, which we denote by $\mu \gets \Rev\langle \cC_{\Rev,\secp},\cR_{\Rev,\secp},\rho_d^{\sC,\sR}\rangle$.
\end{itemize}

For such commitments, we ask for an additional correctness property, and a stronger hiding property.

\begin{definition}[Correctness of deletion, \cite{cryptoeprint:2021:1315}]\label{def:correctness-deletion}
A bit commitment scheme satisfies \emph{correctness of deletion} if for any $b \in \{0,1\}$, it holds with overwhelming probability over $(\sC,\sR) \gets \Com\langle\cC_{\Com,\secp}(b),\cR_{\Com,\secp}\rangle, \allowbreak(d_\cC,\sC,\sR) \gets \Del\langle\cC_{\Del,\secp}(\sC),\cR_{\Del,\secp}(\sR)\rangle$ that $d_\cC = \top$.
\end{definition}


%\iffull
%\paragraph{Hiding.} We define standard notions of statistical and computational hiding.

%\begin{definition}[Hiding.]\label{def:hiding}
%A commitment scheme satisfies \emph{statistical} (resp. \emph{computational}) \emph{hiding} if for any unbounded adversary $\cR^* = \{\cR^*_{\Com,\secp},\cR^*_{\Del,\secp}\}_{\secp \in \bbN}$ (resp. non-uniform QPT adversary $\cR^* = \{\ket{\psi^*_\secp},\cR^*_{\Com,\secp},\cR^*_{\Del,\secp}\}_{\secp \in \bbN}$) and for any unbounded (resp. QPT) distinguisher $\cD^* = \{\cD^*_\secp\}_{\secp \in \bbN}$, it holds that 
%\begin{align*}
    %&\bigg|\Pr\left[\cD^*_\secp(\rho_d^{\sR^*}) = 1 : \begin{array}{r}\rho_c^{\sC,\sR^*} \gets \Com\langle\cC_{\Com,\secp}(0),\cR^*_{\Com,\secp}\rangle \\ (d_\cC,\rho_d^{\sC,\sR^*}) \gets \Del\langle\cC_{\Del,\secp},\cR^*_{\Del,\secp},\rho_c^{\sC,\sR^*}\rangle\end{array}\right] \\ &- \Pr\left[\cD^*_\secp(\rho_d^{\sR^*}) = 1 : \begin{array}{r}\rho_c^{\sC,\sR^*} \gets \Com\langle\cC_{\Com,\secp}(1),\cR^*_{\Com,\secp}\rangle \\ (d_\cC,\rho_d^{\sC,\sR^*}) \gets \Del\langle\cC_{\Del,\secp},\cR^*_{\Del,\secp},\rho_c^{\sC,\sR^*}\rangle\end{array}\right]\bigg| = \negl(\secp),
%\end{align*}
%where $\rho_d^{\sR^*}$ is obtained by tracing out the register $\sC$ from $\rho_d^{\sC,\sR^*}$.
%\end{definition}
%\else\fi


\begin{definition}[Certified everlasting hiding, \cite{cryptoeprint:2021:1315}]\label{def:CEH}
A commitment scheme satisfies \emph{certified everlasting hiding} if it satisfies the following two properties. First, for any non-uniform QPT adversary and distinguisher $\cR^* = \{\cR^*_{\Com,\secp},\cR^*_{\Del,\secp},\cD^*_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$, where $\ket{\psi_\secp}$ is a state on two registers $(\sR^*,\sD^*)$, it holds that 
\begin{align*}
    &\bigg|\Pr\left[\cD^*_\secp(d_\cC,\sR^*,\sD^*) = 1 : \begin{array}{r}(\sC,\sR^*) \gets \Com\langle\cC_{\Com,\secp}(0),\cR^*_{\Com,\secp}(\sR^*)\rangle \\ (d_\cC,\sC,\sR^*) \gets \Del\langle\cC_{\Del,\secp}(\sC),\cR^*_{\Del,\secp}(\sR^*)\rangle\end{array}\right] \\ &- \Pr\left[\cD^*_\secp(d_\cC,\sR^*,\sD^*) = 1 : \begin{array}{r}(\sC,\sR^*) \gets \Com\langle\cC_{\Com,\secp}(1),\cR^*_{\Com,\secp}(\sR^*)\rangle \\ (d_\cC,\sC,\sR^*) \gets \Del\langle\cC_{\Del,\secp}(\sC),\cR^*_{\Del,\secp}(\sR^*)\rangle\end{array}\right]\bigg| = \negl(\secp).
\end{align*}

Second, for any non-uniform QPT adversary $\cR^* = \{\cR^*_{\Com,\secp},\cR^*_{\Del,\secp},\ket{\psi}\}_{\secp \in \bbN}$, where $\ket{\psi_\secp}$ is a state on two registers $(\sR^*,\sD^*)$, it holds that \[\TD\left(\EVEXP_\secp^{\cR^*}(0),\EVEXP_\secp^{\cR^*}(1)\right) = \negl(\secp),\] where the experiment $\EVEXP_\secp^{\cR^*}(b)$ is defined as follows.
\begin{itemize}
    \item Execute the Commit phase $(\sC,\sR^*) \gets \Com\langle\cC_{\Com,\secp}(b),\cR^*_{\Com,\secp}(\sR^*)\rangle$.
    \item Execute the Delete phase $(d_\cC,\sC,\sR^*) \gets \Del\langle\cC_{\Del,\secp}(\sC),\cR^*_{\Del,\secp}(\sR^*))\rangle$.
    \item If $d_\cC = \top$ then output $(\sR^*,\sD^*)$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

Then, we have the following corollary of \cref{thm:main}.

\begin{corollary}\label{cor:cecom}
Given any statistically binding computationally hiding commitment scheme $\Com$, the commitment defined as follows is a statistically binding commitment scheme with certified everlasting hiding.
\begin{itemize}
    \item The committer, on input $b \in \{0,1\}$, samples $x,\theta \gets \{0,1\}^\secp$. Then, the committer and receiver engage in the Commit phase of $\Com$, where the committer has input $(\theta,b \oplus \bigoplus_{i: \theta_i = 0}x_i)$. Finally, the committer sends $\ket{x}_\secp$ to the receiver.
    \item For the Delete phase, the receiver measures the state $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and sends $x'$ to the committer. The committer outputs $\top$ if and only if $x_i = x'_i$ for all $i$ such that $\theta_i = 1$.
    \item For the Reveal phase, the committer and receiver engage in the Reveal phase of $\Com$, where the committer reveals the committed input $(\theta,b')$. If this passes, the receiver measures $\ket{x}_\theta$ in the $\theta$ basis to obtain $x$ and outputs $b = b' \oplus \bigoplus_{i: \theta_i = 0}x_i$.
\end{itemize}
\end{corollary}

\begin{proof}
First, we show that statistical binding is preserved. Given a malicious committer $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$, consider the experiment $\Ideal_\secp^{\cC^*,\cE}$ specified by an extractor $\cE$ defined as follows. 

\begin{itemize}
    \item Invoke the extractor for the underlying commitment scheme on the first part of $\cC^*_{\Com,\secp}$, which produces a joint state on $(\sC^*,\sR)$ and extracted values $(\theta^*,b^*)$.
    \item Continue running $\cC^*_{\Com,\secp}$ until it outputs a $\secp$-qubit state on register $\sX$, which in the honest case will hold a state of the form $\ket{x}_\theta$.
    \item Measure the register $\sX$ in the $\theta^*$ basis to produce $x^*$, and set the extracted bit $\widehat{b}^* \coloneqq b^* \oplus \bigoplus_{i: \theta_i^* = 0}x^*_i$.
\end{itemize}

Then, the Reveal phase of the underlying commitment scheme is run to produce a final committer's state on register $\sC^*$ and receiver's output, which is either $\bot$ or some $(\theta',b')$. Finally, the receiver either outputs $\bot$ or completes the Reveal phase by measuring register $\sX$ in the $\theta$ basis to obtain $x$, and outputting $b' \oplus \bigoplus_{i: \theta_i = 0}x_i$.

Note that, by the statistical binding property of the underlying commitment, the final state on $\sC^*$ produced by $\cC^*_{\Rev,\secp}$ in this experiment will be within negligible trace distance of the state on $\sC^*$ output in the $\Real_\secp^{\cC^*}$ experiment, and moreover the probability that $\cR_{\Rev,\secp}$ accepts opened values $(\theta',b')$ that are not equal to the previously extracted values $(\theta^*,b^*)$ is negligible. Thus, conditioned on opening accepting, with all but negligible probability the extractor's and receiver's measurement of $\sX$ will be identical. Thus, the extracted bit and receiver's output will be the same, and the outcome $\mathsf{FAIL}$ will only occur with negligible probability.

Next, we show certified everlasting hiding. The first property follows immediately from the hiding of the underlying commitment scheme, since there are no messages from $\cC$ in the delete phase, and the bit $d_\cC$ is computed independently of $b$. The second property follows from hiding of the underlying commitment scheme and \cref{thm:main} by setting  $\cZ_\secp(\theta)$ and $\cA_\secp$ as follows.

\begin{itemize}
    \item $\cZ_\secp(\theta)$ initializes registers $(\sR^*,\sD^*)$ with $\ket{\psi_\secp}$, runs $(\sC_\theta,\sR^*) \gets \Com\langle\cC_{\secp}(\theta),\cR^*_{\Com,\secp}(\sR^*)\rangle$ with the first part of $\cR^*_{\Com,\secp}$ (where $\cC_\secp$ is the commit algorithm of the underlying commitment scheme $\Com$), and outputs the resulting state on register $\sR^*$.
    \item $\cA_\secp$ receives $\ket{x}_\theta, b \oplus \bigoplus_{i: \theta_i = 0} x_i,$ and the state on register $\sR^*$. It first runs $(\sC_b,\sR^*) \gets \Com\langle\cC_{\secp}(b \oplus \bigoplus_{i: \theta_i = 0} x_i),\cR^*_{\Com,\secp}(\sR^*)\rangle$ with the remaining part of $\cR^*_{\Com,\secp}$, and then runs $\cR^*_{\Del,\secp}(\sR^*,\ket{x}_\theta)$, which outputs a classical certificate and a left-over quantum state. 
\end{itemize}
 %and setting the class of adversaries $\mathscr{A}$ to be $\{\cR^*_{\Del,\secp}\}_{\secp \in \bbN}$ which is the class of uniform quantum polynomial-time adversaries. Note that 
\end{proof}

\begin{remark}
We note that the above corollary explicitly considers underlying statistically binding commitment schemes that may include quantum communication, and thus one implication is that statistically binding commitments with certified everlasting hiding can be built just from the assumption that pseudo-random quantum states exist \cite{cryptoeprint:2021:1691,cryptoeprint:2021:1663}.
\end{remark}

\begin{remark}
Similarly to the setting of public-key encryption, single-bit certified everlasting hiding for statistically binding commitments implies multi-bit certified everlasting hiding.
\end{remark}


\subsubsection{Certified everlasting zero-knowledge proofs for QMA}
We begin by defining proofs for QMA with certified everlasting zero-knowledge, introduced in~\cite{cryptoeprint:2021:1315}. Our definition is identical to theirs, except that we also guarantee computational zero-knowledge in the case that the verifier outputs invalid deletion certificates. In what follows, we will assume familiarity with the notion of a (statistically sound) proof for a QMA promise problem. 
%A precise definition of computational ZK proofs for QMA can be found in~\cite{cryptoeprint:2021:1315}.

\begin{definition}\label{def:cehzk}
A certified everlasting zero-knowledge proof for a QMA promise problem $A = (A_{\mathsf{yes}}, A_{\mathsf{no}})$ is a proof for $A$ that
additionally satisfies the following properties.
\begin{itemize}
\item{ \bf (Perfect) Correctness of certified deletion.}
For every instance $x \in A_{\mathsf{yes}}$ and every state $\ket{\psi} \in R_A(x)$, the prover  outputs $\top$ as its output in the interaction $\langle \mathcal{P}(x,\ket{\psi}^{\otimes {k(|x|)}}),\cV(x) \rangle$.

\item{\bf Certified everlasting zero-knowledge.}
Let $\mathsf{REAL}_\secp{\langle \mathcal{P}(x,\ket{\psi}^{\otimes {k(|x|)}}),\cV^*(x)\rangle}$ denote the joint distribution of the output of an honest prover and the state of an arbitrary QPT verifier $\cV^*$ after they execute the proof on instance $x \in A_{\mathsf{yes}}$, where the prover has as quantum input a polynomial number $k(|x|)$ copies of a state $\ket{\psi} \in R_A(x)$.
Then there exists a QPT algorithm $\mathsf{Sim}$ that on input any $x \in A_{\mathsf{yes}}$ and with oracle access to any non-uniform QPT $\cV^* = \{\cV^*_\secp\}_{\secp \in \bbN}$, outputs distribution $\mathsf{Sim}_\secp^{\cV^*}(x)$ such that:
\begin{itemize}
    \item First, we have everlasting zero-knowledge against adversaries that produce a valid deletion certificate, i.e., \[\TD\left(\mathsf{EV}\left(\mathsf{REAL}_\secp{\langle \mathcal{P}\left(x,\ket{\psi}^{\otimes {k(|x|)}}\right),\cV^*(x)\rangle}\right),\mathsf{EV}\left(\mathsf{Sim}_\secp^{\cV^*}(x)\right)\right) = \negl(\secp),\] where 
    %to obtain prover output $o \in \{\top, \bot\}$ and verifier state $\rho$.
    $\mathsf{EV}(\cdot)$ is a quantum circuit that on input a classical string $o \in \{\top, \bot\}$ and a quantum state $\rho$ outputs $(\top, \rho)$ when $o = \top$, and otherwise outputs $(\bot, \bot)$. 
    \item Second, we have computational zero-knowledge against all adversaries, even when they do not necessarily output valid deletion certificates, i.e.,
    for every QPT distinguisher $\cD^* = \{\cD^*_\secp\}_{\secp \in \bbN}$, 
    \[\bigg|\Pr\left[\cD^*_\secp\left(\mathsf{REAL}_\secp{\langle \mathcal{P}\left(x,\ket{\psi}^{\otimes {k(|x|)}}\right), \cV^*(x) \rangle}\right) = 1\right] - \Pr\left[\cD^*_\secp\left(\mathsf{Sim}_\secp^{\cV^*}(x)\right) = 1\right]\bigg| = \negl(\secp)\]
\end{itemize}
\end{itemize}
\end{definition}

Next, we define a notion of classical extractor-based binding for commitments. This definition was introduced in~\cite{cryptoeprint:2021:1315}, and while their definition requires perfect extraction, we observe that their theorem holds even if the underlying commitment satisfies only statistical extraction. As such we allow for $\negl(\secpar)$ statistical error in our definition.

\begin{definition}[Classical extractor-based binding~\cite{cryptoeprint:2021:1315}]
A quantum commitment with classical non-interactive decommitment satisfies classical extractor-based binding if there exists an unbounded-time deterministic algorithm $\mathsf{Ext}$ that on input the classical transcript of a (possibly quantum) commitment $\mathsf{com}$, outputs the only unique classical decommitment string $d$ that will cause the verifier to accept the reveal phase, except with negligible probability.
\end{definition}


Finally, we will rely on the following theorem from~\cite{cryptoeprint:2021:1315}, which we describe below, paraphrased according to our definitions.

\begin{theorem}[\cite{cryptoeprint:2021:1315}] \label{thm:imp}
Assuming the existence of commitments satisfying statistical {\em classical extractor-based} binding and certified everlasting hiding (according to Definition \ref{def:CEH}), there exists a zero-knowledge proof for QMA satisfying certified everlasting zero-knowledge (according to Definition \ref{def:cehzk}).
\end{theorem}

We obtain the following corollary of Theorem \ref{thm:imp} and our Corollary \ref{cor:cecom}.
\begin{corollary}
Assuming the existence of post-quantum one-way functions, there exists a zero-knowledge proof for QMA satisfying certified everlasting zero-knowledge (according to Definition \ref{def:cehzk}).
\end{corollary}
This corollary follows from the observation that our construction of commitments with certified everlasting hiding, when instantiated with any classical statistically binding commitment (and in particular Naor's commitment from one-way functions) satisfies classical extractor-based binding. The extractor simply outputs the decommitment of the classical part of our commitment. The resulting commitment with certified everlasting hiding and classical extractor-based binding can be plugged into Theorem \ref{thm:imp} to obtain the corollary above.

\subsection{Timed-release encryption}

A timed-release encryption scheme \cite{Rivest1996TimelockPA,EC:Unruh14} $\TRE = (\TRE.\Enc,\TRE.\Dec)$  has the following syntax.

\begin{itemize}
    \item $\TRE.\Enc(1^\secp,m) \to \ct$ is a polynomial-time algorithm that takes as input the security parameter $1^\secp$ and a message $m$ and outputs a ciphertext $\ct$.
    \item $\TRE.\Dec(\ct) \to m$ is a polynomial-time algorithm that takes as input a ciphertext $\ct$ and outputs a message $m$.
\end{itemize}

A timed-released encryption scheme is (post-quantum) $T(\secp)$-hiding if the following holds.

\begin{definition}[Hiding time-released encryption]\label{def:TRE-hiding}
A timed-released encryption scheme $\TRE = (\TRE.\Enc,\allowbreak\TRE.\Dec)$ is $T(\secp)$-hiding if for any non-uniform quantum polynomial-time\footnote{As discussed in \cite{EC:Unruh14}, it is important to have a polynomial-time bound on the overall complexity of the adversary, in addition to the $T(\secp)$ parallel time bound.} adversary $\cA = \{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$ with at most $T(\secp)$ parallel time, \[\bigg|\Pr\left[\cA_\secp(\TRE.\Enc(1^\secp,0)) = 1\right] - \Pr\left[\cA_\secp(\TRE.\Enc(1^\secp,1)) = 1\right]\bigg| = \negl(\secp).\]
\end{definition}

Now, we augment the syntax of a $\TRE$ scheme with algorithms $\RTRE.\Del, \RTRE.\Ver$ to arrive at the notion of a \emph{revocable} timed-release encryption scheme $\RTRE$.

\begin{itemize}
    \item $\RTRE.\Enc(1^\secp,m) \to (\ct,\vk)$ is a polynomial-time algorithm that takes as input the security parameter $1^\secp$ and a message $m$ and outputs a quantum ciphertext $\ct$ and a (potentially quantum) verification key $\vk$.
    \item $\RTRE.\Dec(\ct) \to m$ is a polynomial-time algorithm that takes as input a quantum ciphertext $\ct$ and outputs a message $m$.
    \item $\RTRE.\Del(\ct) \to \cert$ is a quantum algorithm that takes as input a quantum ciphertext $\ct$ and outputs a (potentially quantum) deletion certificate $\cert$.
    \item $\RTRE.\Ver(\vk,\cert) \to \{\top,\bot\}$ is a (potentially quantum) algorithm that takes as input a (potentially quantum) verification key $\vk$ and a (potentially quantum) deletion certificate $\cert$ and outputs either $\top$ or $\bot$.
\end{itemize}

We say that $\RTRE$ satisfies revocable hiding if the following holds.

\begin{definition}[Revocably hiding time-released encryption]\label{def:TRE-revocable-hiding}
A timed-released encryption scheme $\RTRE = (\RTRE.\Enc,\RTRE.\Dec,\RTRE.\Del,\RTRE.\Ver)$ is $T(\secp)$-revocably hiding if for any non-uniform quantum polynomial-time adversary $\cA = \{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$ with at most $T(\secp)$ parallel time, it holds that \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP\secp^{\cA}(1)\right) = \negl(\secp),\]
and  \[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
where the experiment $\EVEXP\secp^{\cA}(b)$ is defined as follows.
\begin{itemize}
    \item Sample $(\ct,\vk) \gets \RTRE.\Enc(1^\secp,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\RTRE.\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
and the experiment $\CEXP\secp^{\cA}(b)$ is defined as follows.
\begin{itemize}
    \item Sample $(\ct,\vk) \gets \RTRE.\Enc(1^\secp,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item Output $\cA_\secp(\rho, \Ver(\vk,\cert))$.
\end{itemize}
\end{definition}

We say that $\RTRE$ is a revocable time-released encryption scheme against $T(\secp)$-parallel time adversaries if it satisfies (i) hiding (\cref{def:TRE-hiding}) against $T(\secp)$-parallel time adversaries, (ii) correctness of deletion (\cref{def:CD-correctness}), and (iii) recovable hiding (\cref{def:TRE-revocable-hiding}) against $T(\secp)$-parallel time adversaries.

Then, we have the following corollary of \cref{thm:main}.

\begin{corollary}
Given any post-quantum secure time-released encryption $\TRE = (\TRE.\Enc,\TRE.\Dec)$ against $T(\secp)$-parallel time adversaries, the scheme $\RTRE = (\Enc',\Dec',\Del,\Ver)$ defined as follows is a secure \emph{revocable} time-released encryption scheme against $T(\secp)$-parallel time adversaries.
\begin{itemize}
     \item $\Enc'(\pk,m):$ sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ct \coloneqq \left(\ket{x}_\theta,\TRE.\Enc\left(\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\right)\right), \ \ \ \vk \coloneqq (x,\theta).\]
    \item $\Dec'(\sk,\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$, compute $(\theta,b') \gets \TRE.\Dec(\sk,\ct')$, measure $\ket{x}_\theta$ in the $\theta$-basis to obtain $x$, and output $b = b' \oplus \bigoplus_{i:\theta_i = 0}x_i$.
    \item $\Del(\ct):$ parse $\ct \coloneqq \left(\ket{x}_\theta,\ct'\right)$ and measure $\ket{x}_\theta$ in the Hadamard basis to obtain a string $x'$, and output $\cert \coloneqq x'$.
    \item $\Ver(\vk,\cert):$ parse $\vk$ as $(x,\theta)$ and $\cert$ as $x'$ and output $\top$ if and only if $x_i = x_i'$ for all $i$ such that $\theta_i = 1$.
\end{itemize}
\end{corollary}

\begin{proof}
Hiding follows immediately from the hiding of $\TRE$. Correctness of deletion follows immediately from the description of the scheme. Revocable hiding follows because
\begin{itemize}
\item First, \[\TD\left(\EVEXP_\secp^{\cA}(0),\EVEXP\secp^{\cA}(1)\right) = \negl(\secp),\]
follows from \cref{thm:main} and the hiding of $\TRE$, and by setting the distribution $\cZ(b)$ to sample $(\ct,\vk) \gets \TRE.\Enc(1^\secp,b)$ and output $\ct$, and setting the class of adversaries $\mathscr{A}$ to be all non-uniform QPT adversaries $\{\cA_\secp,\ket{\psi_\secp}\}_{\secp \in \bbN}$ with at most $T(\secp)$ parallel time.
\item Second, \[\bigg|\Pr\left[\CEXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
follows from the fact that the timed-release encryption remains (computationally) semantically secure even when the adversary is given the verification key corresponding to the challenge ciphertext.
\end{itemize}
This completes our proof.
\end{proof}

\begin{remark}
Similarly to the setting of public-key encryption, single-bit certified everlasting hiding for timed-release encryption implies certified everlasting hiding for multi-bit messages.
\end{remark}






%DK was supported in part from a DARPA SIEVE award and NSF under award number 2112890. This material is based upon work supported by the Defense Advanced Research Projects Agency through Award HR00112020024.
%NSF QIS and an award from C3AI.


==> certified-deletion-2.tex <==
\section{Main theorems}

In this section, we present our main theorems, which allows to generically add a certified deletion property to a wide variety of cryptographic primitives.

\subsection{Information-theoretic certified deletion}

First, we present a warm-up to our main theorem, which will also be useful on its own for constructing information-theoretic cryptographic primitives, such as one-time pad encryption and secret sharing, with certified deletion.

\begin{theorem}
For any unbounded adversary $\{\cA_\secp\}_{\secp \in \bbN}$, it holds that \[\TD\left(\ITEXP_\secp^{\cA}(0),\ITEXP_\secp^{\cA}(1)\right) = \negl(\secp),\] where the experiment $\ITEXP_\secp^{\cA}(b)$ is defined as follows.

\begin{itemize}
    \item Sample $x,\theta \gets \{0,1\}^\secp$ and initialize $\cA_\secp$ with \[\ket{x}_\theta, b \oplus \bigoplus_{i:\theta_i = 0}x_i.\]
    \item $\cA_\secp$'s output is parsed as a bitstring $x' \in \{0,1\}^\secp$ and a residual quantum state $\rho$.
    \item If $x_i = x_i'$ for all $i$ such that $\theta_i = 1$ then output $(\theta,\rho)$, and otherwise output a special symbol $\bot$.
\end{itemize}
\end{theorem}

\begin{proof}
\james{TODO}
\end{proof}

\subsection{Certified deletion from computational assumptions}

\begin{theorem}\label{thm:main}Let $\{\cZ_\secp(b)\}_{\secp \in \bbN, b \in \{0,1\}}$ be a family of distributions over either classical bitstrings or quantum states, and let $\mathscr{A}$ be any class of adversaries\footnote{Technically, we require that any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$ has time and space complexity at least linear in $\secp$} such that for any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, it holds that \[\bigg|\Pr\left[\cA_\secp\left(\cZ_\secp(0)\right) = 1\right] - \Pr\left[\cA_\secp\left(Z_\secp(1)\right) = 1\right]\bigg| = \negl(\secp).\] For $m \in \{0,1\}^n$, let $\cZ_\secp(m)$ denote the distribution $\cZ_\secp(m_1),\dots,\cZ_\secp(m_n)$. 

Now, consider the following distribution $\left\{\widetilde{\cZ}_\secp^{\cA_\secp}(b)\right\}_{\secp \in \bbN, b \in \{0,1\}}$ over quantum states, obtained by running $\mathcal{A}_\lambda$ as follows.

\begin{itemize}
    \item Sample $x,\theta \gets \{0,1\}^\secp$ and initialize $\cA_\secp$ with \[\ket{x}_\theta, \cZ_\secp\left(\theta,b \oplus \bigoplus_{i: \theta_i = 0}x_i\right).\]
    \item $\cA_\secp$'s output is parsed as a bitstring $x' \in \{0,1\}^\secp$ and a residual quantum state $\rho$.
    \item If $x_i = x_i'$ for all $i$ such that $\theta_i = 1$ then output $\rho$, and otherwise output a special symbol $\bot$.
\end{itemize}

Then, for any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, it holds that \[\TD\left(\widetilde{\cZ}_\secp^{\cA_\secp}(0), \widetilde{\cZ}_\secp^{\cA_\secp}(1)\right) = \negl(\secp).\]
\end{theorem}



\begin{proof}

We define a sequence of hybrid distributions.

\begin{itemize}
    \item $\Hyb_0(b):$ This is the distribution $\left\{\cZ_\secp^{\cA_\secp}(b)\right\}_{\secp \in \bbN}$ described above.
    
    \item $\Hyb_1(b):$ This distribution is sampled as follows.
    \begin{itemize}
        \item Prepare $\secp$ EPR pairs $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$ on registers $(\sC_1,\sA_1),\dots,(\sC_\secp,\sA_\secp)$. Define $\sC \coloneqq \sC_1,\dots,\sC_\secp$ and $\sA \coloneqq \sA_1,\dots,\sA_\secp$.
        \item Sample $\theta \gets \{0,1\}, b' \gets \{0,1\}$, measure register $\sC$ in basis $\theta$ to obtain $x \in \{0,1\}^\secp$, and initialize $\cA_\secp$ with register $\sA$ along with $\cZ_\secp\left(\theta,b'\right)$.
        \item If $b' = b \oplus \bigoplus_{i: \theta_i = 0} x_i$ then proceed as in $\Hyb_0$ and otherwise output $\bot$.
    \end{itemize}
    \item $\Hyb_2(b):$ This is the same as $\Hyb_1(b)$ except that measurement of register $\sC$ to obtain $x$ is performed after $\cA_\secp$ outputs $x'$ and $\rho$.
\end{itemize}

We define $\Advt(\Hyb_i) \coloneqq \TD\left(\Hyb_i(0),\Hyb_i(1)\right).$ Then, we have that \[\Advt(\Hyb_1) \geq \Advt(\Hyb_0)/2,\] which follows because $\Hyb_1(b)$ is identically distributed to the distribution that outputs $\bot$ with probability 1/2 and otherwise outputs $\Hyb_0(b)$. Next, we have that \[\Advt(\Hyb_2) = \Advt(\Hyb_1),\] which follows because the register $\sC$ is disjoint from the registers that $\cA_\secp$ operates on. Thus, it remains to show that \[\Advt(\Hyb_2) = \negl(\secp).\]

To show this, we first define the following hybrid.

\begin{itemize}
    \item $\Hyb_2'(b):$ This is the same as $\Hyb_2$ except that $\cA_\secp$ is initialized with register $\sA$ and $\cZ_\secp(0^\secp,b')$.
\end{itemize}


Now, for any $b \in \{0,1\}$, consider the state on register $\sC$ immediately after $\cA_\secp$ outputs $(x',\rho)$ in $\Hyb'_2(b)$. Define the projection \[\Pi_{x',\theta} \coloneqq \ket{x'_{i: \theta_i = 1}}_1^{\sC_{i: \theta_i = 1}}\bra{x'_{i : \theta_i = 1}}_1^{\sC_{i: \theta_i = 1}} \otimes \sum_{y: \Delta\left(y,x'_{i: \theta_i = 0}\right) \geq 1/2}\ket{y}^{\sC_{i : \theta_i = 0}}_1\bra{y}^{\sC_{i : \theta_i = 0}}_1,\] where all the basis vectors are in the Hadamard basis, denoted by $\ket{\cdot}_1$, and $\Delta(\cdot,\cdot)$ denotes relative Hamming distance. Then, let $\Pr[\Pi_{x',\theta},\Hyb_2'(b)]$ be the probability that a measurement of $\left\{\Pi_{x',\theta}, \bbI - \Pi_{x',\theta}\right\}$ accepts (returns the outcome associated with $\Pi_{x',\theta}$) in $\Hyb_2'(b)$.

\begin{claim}\label{claim:BF10}
For any $b \in \{0,1\}$, $\Pr[\Pi_{x',\theta},\Hyb_2'(b)] = \negl(\secp)$.
\end{claim}

\begin{proof}
Since $\theta$ is sampled independently of $\cA_\secp$'s input in this experiment, we can consider sampling it after $\cA_\secp$ outputs $x'$ and $\rho$. Thus, we consider the following setup. The experiment is run until $\cA_\secp$ outputs $x'$ and $\rho$, where $\rho$ may be entangled with the challenger's register $\sC$. Then, $\theta \gets \{0,1\}^\secp$ is sampled, which defines a uniformly random subset of the registers in $\sC$ to measure in the Hadamard basis. For each register $\sC_i$ such that $\theta_i = 1$, it is checked if the measurement result $x_i$ is equal to $x'_i$.

Now, one can use the final part of this experiment to define a sampling and estimation strategy (\cref{subsec:quantum-sampling}) that is applied to the state on register $\sC = \sC_1,\dots,\sC_\secp$. Here, the orthonormal basis each subsystem is measured in is the single-qubit Hadamard basis, and the ``reference system''\footnote{\cref{subsec:quantum-sampling} describes an all-zeros reference system, but it is easy to see that this generalizes to any fixed string.} is $\ket{x'_1}_1,\dots,\ket{x'_\secp}_1$. The strategy consists of sampling a uniformly random subset of indices of $[\secp]$, defined by $i$ such that $\theta_i = 1$, measuring $\sC_{i: \theta_i = 1}$ to obtain a string $\widetilde{x}$, and then outputting the relative Hamming weight of $\widetilde{x} \oplus x'_{i: \theta_i = 1}$ as the estimate for ``how close''\footnote{The formal definition of closeness is described in \cref{subsec:quantum-sampling}.} the state on register $\sC_{i: \theta_i = 0}$ is to $\ket{x'_{i: \theta_i = 0}}_1$. Noting that this sampling and estimation strategy is exactly the $\Psi_{\mathsf{uniform}}$ strategy described at the end of \cref{subsec:quantum-sampling}, we have by \cref{corollary:sampling} that the quantum error probability of this strategy is bounded by $2e^{-\secp\delta^2/64} = \negl(\secp)$, for $\delta = 1/2$. By the definition of quantum error probability (\cref{def:quantum-error-probability}), this means that, with overwhelming probability over $\theta \gets \{0,1\}^\secp$, the state on register $\sC$ is within negligible trace distance of a state in the image of $\bbI - \Pi_{x',\theta}$. Indeed, $\Pi_{x',\theta}$ is a projection onto states where the computed estimate for closeness of $\sC_{i: \theta_i = 0}$ to $\ket{x'_{i: \theta_i = 0}}_1$ is 0, yet the actual state on $\sC_{i: \theta_i = 0}$ is supported on vectors with relative Hamming distance $\geq 1/2$ from $x'_{i: \theta_i = 0}$. This completes the proof of the claim.

%This setup defines a ``quantum sampling game'' (\cref{subsec:quantum-sampling}) that checks whether $\sC$ is ``close'' to the state $\ket{x'}_1$, that is, the string $x'$ encoded in the Hadamard basis. Formally, the sampling strategy is defined by setting $P_T$ to be the uniform distribution over subsets of $[\secp]$, setting $P_S = \bot$, and setting $f$ to be the function that outputs the relative Hamming weight on the measured positions as the estimate for the relative Hamming weight on the non-measured positions. Then by \cref{impthm:error-probability}, the probability $\sP[\Pi_{x',\theta},\Hyb_2'(b)]$ is bounded the square root of the error probability of the corresponding classical sampling game with parameter $\delta = 1/2$. This error probability can be bounded with Chernoff, and is analyzed in \cite[Appendix B.3]{C:BouFeh10}, where it is shown to be bounded by $4e^{-\secp\delta^2/32} = \negl(\secp)$ for $\delta = 1/2$. This completes the proof of the claim.
\end{proof}

Now we consider the probability of the corresponding event in $\Hyb_2(b)$, denoted $\Pr[\Pi_{x',\theta},\Hyb_2(b)]$.

\begin{claim}\label{claim:predicate}
For any $b \in \{0,1\}$, $\Pr[\Pi_{x',\theta},\Hyb_2(b)] = \negl(\secp)$.
\end{claim}

\begin{proof}
This follows by a direct reduction to semantic security of the distribution family $\{\cZ_\secp(\cdot)\}_{\secp \in \bbN}$. The reduction samples $\theta \gets \{0,1\}^\secp$, sends $\theta$ to its challenger, and receives either $\cZ_\secp(\theta)$ or $\cZ_\secp(0^\secp)$ from its challenger. Then, it prepares $\secp$ EPR pairs, runs $\cA_\secp$ on halves of the EPR pairs along with the output of the distribution it received from its challenger, and $\cZ_\secp(b')$ for a random $b' \gets \{0,1\}$. After $\cA_\secp$ outputs $(x',\rho)$, it measures $\left\{\Pi_{x',\theta},\bbI - \Pi_{x',\theta}\right\}$ on the other halves of the EPR pairs. Note that the complexity of this reduction is equal to the complexity of $\cA$ plus an extra $\secp$ qubits of space and an extra linear time operation, so it is still in $\mathscr{A}$. If $\Pr[\Pi_{x',\theta},\Hyb_2(b)]$ is non-negligible this can be used to distinguish $\cZ_\secp(\theta)$ from $\cZ_\secp(0^\secp)$, due to \cref{claim:BF10}.
\end{proof}

Finally, we can show the following claim, which completes the proof.

\begin{claim}
$\Advt(\Hyb_2) = \negl(\secp).$
\end{claim}

\begin{proof}
First, we note that for any $b \in \{0,1\}$, the global state of $\Hyb_2(b)$ immediately after $\cA_\secp$ outputs $x'$ is within negligible trace distance of a state $\tau^{\sC,\sA'}_{\mathsf{Ideal}}$ in the image of $\bbI - \Pi_{x',\theta}$, where $\sA'$ is $\cA_\secp$'s quantum output register. This follows immediately from \cref{claim:predicate} and Gentle Measurement (\cref{lemma:gentle-measurement}). Now, consider the measurement of $\tau_{\mathsf{Ideal}}^{\sC,\sA'}$ on $\sC_{i: \theta_i = 1}$ that determines whether the experiment outputs $\bot$. That is, the procedure that measures $\sC_{i:\theta_i = 1}$ in the Hadamard basis and checks if the resulting string is equal to $x'_{i: \theta_i = 1}$. There are two options.

\begin{itemize}
    \item If the measurement fails, then the experiment outputs $\bot$, independent of whether $b=0$ or $b=1$, so there is 0 advantage in this case.
    \item If the measurement succeeds, then we know that the state on registers $\sC_{i: \theta_i = 0}$ is only supported on vectors $\ket{y}_1$ such that $\Delta(y,x'_{i: \theta_i = 0}) < 1/2$, since $\tau_{\mathsf{Ideal}}^{\sC,\sA'}$ was in the image of $\bbI - \Pi_{x',\theta}$. These registers are then measured in the computational basis to produce $\{x_i\}_{i:\theta_i = 0}$, and the experiment outputs $\bot$ if $\bigoplus_{i:\theta_i = 0}x_i \neq b' \oplus b$ and otherwise outputs the state on register $\sA'$. Note that (i) this decision is the \emph{only} part of the experiment that depends on $b$, and (ii) by \cref{thm:XOR-extractor}, the bit  $\bigoplus_{i:\theta_i = 0}x_i$ is \emph{uniformly random and independent} of the register $\sA'$, which is disjoint (but possibly entangled with) $\sC$. Thus, there is also 0 advantage in this case. 
    
    In slightly more detail, \cref{thm:XOR-extractor} says that making a Hadamard basis measurement of a register that is in a superposition of computational basis vectors with relative Hamming weight $< 1/2$ will produce a set of bits $\{x_i\}_{i: \theta_i = 0}$ such that $\bigoplus_{i: \theta_i = 0}x_i$ is a uniformly random bit, even given potentially entangled quantum side information. We can apply this lemma to our system on $\sC_{i: \theta_i = 0},\sA'$ by considering a change of basis that maps $\ket{x'_{i: \theta_i = 0}}_1 \to \ket{0}_0$. That is, the change of basis first applies Hadamard, and then an XOR with the fixed string $x'_{i: \theta_i = 0}$. Applying such a change of basis maps $\sC_{i: \theta_i = 0}$ to a state that is supported on vectors $\ket{y}_0$ such that $\omega(y) < 1/2$, and we want to claim that a \emph{Hadamard} basis measurement of the resulting state produces $\{x_i\}_{i: \theta_i = 0}$ such that $\bigoplus_{i: \theta_i = 0}x_i$ is uniformly random and independent of $\sA$. This is exactly the statement of \cref{thm:XOR-extractor}.
\end{itemize}

This completes the proof, since we have shown that there exists a single distribution, defined by $\tau^{\sC,\sA'}_{\mathsf{Ideal}}$, that is negligibly close to both $\Hyb_2(0)$ and $\Hyb_2(1)$.
\end{proof}

\end{proof}

==> certified-deletion-depracated.tex <==
\section{Main theorem}
\label{sec:main}
%In this section, we present our main theorems, which allow to generically add a certified deletion property to a wide variety of cryptographic primitives.



\begin{theorem}\label{thm:main}
Let $\{\cZ_\secp(m)\}_{\secp \in \bbN, m \in \{0,1\}}$ be a family of distributions over either classical bitstrings or quantum states, and let $\mathscr{A}$ be any class of adversaries\footnote{Technically, we require that for any   $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, every adversary $\cB$ with time and space complexity that is linear in $\secp$ more than that of $\cA_\secp$, is also in $\mathscr{A}$.} such that for any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, it holds that \[\bigg|\Pr\left[\cA_\secp\left(\cZ_\secp(0)\right) = 1\right] - \Pr\left[\cA_\secp\left(\cZ_\secp(1)\right) = 1\right]\bigg| = \negl(\secp).\] For $m \in \{0,1\}^n$, let $\cZ_\secp(m)$ denote the distribution $\cZ_\secp(m_1),\dots,\cZ_\secp(m_n)$.

For any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, consider the following distribution $\left\{\widetilde{\cZ}_\secp^{\cA_\secp}(b)\right\}_{\secp \in \bbN, b \in \{0,1\}}$ over quantum states, obtained by running $\mathcal{A}_\lambda$ as follows.

\begin{itemize}
    \item Sample $x,\theta \gets \{0,1\}^\secp$ and initialize $\cA_\secp$ with \[\ket{x}_\theta, b \oplus \bigoplus_{i:\theta_i = 0}x_i, \cZ_\secp(\theta).\]
    \item $\cA_\secp$'s output is parsed as a bitstring $x' \in \{0,1\}^\secp$ and a residual quantum state $\rho$.
    \item If $x_i = x_i'$ for all $i$ such that $\theta_i = 1$ then output $\rho$, and otherwise output a special symbol $\bot$.
\end{itemize}

Then, 

\[\TD\left(\widetilde{\cZ}_\secp^{\cA_\secp}(0),\widetilde{\cZ}_\secp^{\cA_\secp}(1)\right) = \negl(\secp).\]
\end{theorem}

\begin{remark}
We note that, in fact, the above theorem is true as long as $x,\theta$ are $\omega(\mathsf{log} \secp)$ bits long.
\end{remark}

%\begin{theorem}\label{thm:main-C}
%For any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, it holds that 
%\[\Bigg|\Pr_{x,\theta \gets \{0,1\}^\secp}\left[\cA_\secp\left(\ket{x}_\theta,\bigoplus_{i:\theta_i = 0}x_i,\cZ_\secp(\theta)\right) = 1\right] - \Pr_{x,\theta \gets \{0,1\}^\secp}\left[\cA_\secp\left(\ket{x}_\theta,1 \oplus\bigoplus_{i:\theta_i = 0}x_i,\cZ_\secp(\theta)\right) = 1\right]\Bigg| = \negl(\secp).\]
%\end{theorem}



%Now, consider the following distribution 

%\begin{itemize}
    %\item Sample $x,\theta \gets \{0,1\}^\secp$ and initialize $\cA_\secp$ with \[\ket{x}_\theta, \cZ_\secp\left(\theta,b \oplus \bigoplus_{i: \theta_i = 0}x_i\right).\]
    %\item $\cA_\secp$'s output is parsed as a bitstring $x' \in \{0,1\}^\secp$ and a residual quantum state $\rho$.
    %\item If $x_i = x_i'$ for all $i$ such that $\theta_i = 1$ then output $\rho$, and otherwise output a special symbol $\bot$.
%\end{itemize}

%Then, for any $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, it holds that \[\TD\left(\widetilde{\cZ}_\secp^{\cA_\secp}(0), \widetilde{\cZ}_\secp^{\cA_\secp}(1)\right) = \negl(\secp).\]

%First we prove \cref{thm:main-EV} and then we prove \cref{thm:main-C}.


\begin{proof} We define a sequence of hybrid distributions.

\begin{itemize}
    \item $\Hyb_0(b):$ This is the distribution $\left\{\cZ_\secp^{\cA_\secp}(b)\right\}_{\secp \in \bbN}$ described above.
    
    \item $\Hyb_1(b):$ This distribution is sampled as follows.
    \begin{itemize}
        \item Prepare $\secp$ EPR pairs $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$ on registers $(\sC_1,\sA_1),\dots,(\sC_\secp,\sA_\secp)$. Define $\sC \coloneqq \sC_1,\dots,\sC_\secp$ and $\sA \coloneqq \sA_1,\dots,\sA_\secp$.
        \item Sample $\theta \gets \{0,1\}, b' \gets \{0,1\}$, measure register $\sC$ in basis $\theta$ to obtain $x \in \{0,1\}^\secp$, and initialize $\cA_\secp$ with register $\sA$ along with $b',\cZ_\secp\left(\theta\right)$.
        \item If $b' = b \oplus \bigoplus_{i: \theta_i = 0} x_i$ then proceed as in $\Hyb_0$ and otherwise output $\bot$.
    \end{itemize}
    \item $\Hyb_2(b):$ This is the same as $\Hyb_1(b)$ except that measurement of register $\sC$ to obtain $x$ is performed after $\cA_\secp$ outputs $x'$ and $\rho$.
\end{itemize}

We define $\Advt(\Hyb_i) \coloneqq \TD\left(\Hyb_i(0),\Hyb_i(1)\right).$ Then, we have that \[\Advt(\Hyb_1) \geq \Advt(\Hyb_0)/2,\] which follows because $\Hyb_1(b)$ is identically distributed to the distribution that outputs $\bot$ with probability 1/2 and otherwise outputs $\Hyb_0(b)$. Next, we have that \[\Advt(\Hyb_2) = \Advt(\Hyb_1),\] which follows because the register $\sC$ is disjoint from the registers that $\cA_\secp$ operates on. Thus, it remains to show that \[\Advt(\Hyb_2) = \negl(\secp).\]

To show this, we first define the following hybrid.

\begin{itemize}
    \item $\Hyb_2'(b):$ This is the same as $\Hyb_2$ except that $\cA_\secp$ is initialized with register $\sA$ and $b',\cZ_\secp(0^\secp)$.
\end{itemize}


Now, for any $b \in \{0,1\}$, consider the state on register $\sC$ immediately after $\cA_\secp$ outputs $(x',\rho)$ in $\Hyb'_2(b)$. Define the projection \[\Pi_{x',\theta} \coloneqq \ket{x'_{i: \theta_i = 1}}_1^{\sC_{i: \theta_i = 1}}\bra{x'_{i : \theta_i = 1}}_1^{\sC_{i: \theta_i = 1}} \otimes \sum_{y: \Delta\left(y,x'_{i: \theta_i = 0}\right) \geq 1/2}\ket{y}^{\sC_{i : \theta_i = 0}}_1\bra{y}^{\sC_{i : \theta_i = 0}}_1,\] where all the basis vectors are in the Hadamard basis, denoted by $\ket{\cdot}_1$, and $\Delta(\cdot,\cdot)$ denotes relative Hamming distance. Then, let $\Pr[\Pi_{x',\theta},\Hyb_2'(b)]$ be the probability that a measurement of $\left\{\Pi_{x',\theta}, \bbI - \Pi_{x',\theta}\right\}$ accepts (returns the outcome associated with $\Pi_{x',\theta}$) in $\Hyb_2'(b)$.

\begin{claim}\label{claim:BF10}
For any $b \in \{0,1\}$, $\Pr[\Pi_{x',\theta},\Hyb_2'(b)] = \negl(\secp)$.
\end{claim}

\begin{proof}
Since $\theta$ is sampled independently of $\cA_\secp$'s input in this experiment, we can consider sampling it after $\cA_\secp$ outputs $x'$ and $\rho$. Thus, we consider the following setup. The experiment is run until $\cA_\secp$ outputs $x'$ and $\rho$, where $\rho$ may be entangled with the challenger's register $\sC$. Then, $\theta \gets \{0,1\}^\secp$ is sampled, which defines a uniformly random subset of the registers in $\sC$ to measure in the Hadamard basis. For each register $\sC_i$ such that $\theta_i = 1$, it is checked if the measurement result $x_i$ is equal to $x'_i$.

Now, one can use the final part of this experiment to define a sample-and-estimate strategy (\cref{subsec:quantum-sampling}) that is applied to the state on register $\sC = \sC_1,\dots,\sC_\secp$. Here, the orthonormal basis each subsystem is measured in is the single-qubit Hadamard basis, and the ``reference system''\footnote{\cref{subsec:quantum-sampling} describes an all-zeros reference system, but it is easy to see that this generalizes to any fixed string.} is $\ket{x'_1}_1,\dots,\ket{x'_\secp}_1$. The strategy consists of sampling a uniformly random subset of indices of $[\secp]$, defined by $i$ such that $\theta_i = 1$, measuring $\sC_{i: \theta_i = 1}$ to obtain a string $\widetilde{x}$, and then outputting the relative Hamming weight of $\widetilde{x} \oplus x'_{i: \theta_i = 1}$ as the estimate for ``how close''\footnote{The formal definition of closeness is described in \cref{subsec:quantum-sampling}.} the state on register $\sC_{i: \theta_i = 0}$ is to $\ket{x'_{i: \theta_i = 0}}_1$. Noting that this sample-and-estimate strategy is exactly the $\Psi_{\mathsf{uniform}}$ strategy described at the end of \cref{subsec:quantum-sampling}, we have by \cref{corollary:sampling} that the quantum error probability of this strategy is bounded by $2e^{-\secp\delta^2/64} = \negl(\secp)$, for $\delta = 1/2$. By the definition of quantum error probability (\cref{def:quantum-error-probability}), this means that, with overwhelming probability over $\theta \gets \{0,1\}^\secp$, the state on register $\sC$ is within negligible trace distance of a state in the image of $\bbI - \Pi_{x',\theta}$. Indeed, $\Pi_{x',\theta}$ is a projection onto states where the computed estimate for closeness of $\sC_{i: \theta_i = 0}$ to $\ket{x'_{i: \theta_i = 0}}_1$ is 0, yet the actual state on $\sC_{i: \theta_i = 0}$ is supported on vectors with relative Hamming distance $\geq 1/2$ from $x'_{i: \theta_i = 0}$. This completes the proof of the claim.
%
%This setup defines a ``quantum sampling game'' (\cref{subsec:quantum-sampling}) that checks whether $\sC$ is ``close'' to the state $\ket{x'}_1$, that is, the string $x'$ encoded in the Hadamard basis. Formally, the sampling strategy is defined by setting $P_T$ to be the uniform distribution over subsets of $[\secp]$, setting $P_S = \bot$, and setting $f$ to be the function that outputs the relative Hamming weight on the measured positions as the estimate for the relative Hamming weight on the non-measured positions. Then by \cref{impthm:error-probability}, the probability $\sP[\Pi_{x',\theta},\Hyb_2'(b)]$ is bounded the square root of the error probability of the corresponding classical sampling game with parameter $\delta = 1/2$. This error probability can be bounded with Chernoff, and is analyzed in \cite[Appendix B.3]{C:BouFeh10}, where it is shown to be bounded by $4e^{-\secp\delta^2/32} = \negl(\secp)$ for $\delta = 1/2$. This completes the proof of the claim.
\end{proof}

Now we consider the corresponding event in $\Hyb_2(b)$, denoted $\Pr[\Pi_{x',\theta},\Hyb_2(b)]$.

\begin{claim}\label{claim:predicate}
For any $b \in \{0,1\}$, $\Pr[\Pi_{x',\theta},\Hyb_2(b)] = \negl(\secp)$.
\end{claim}

\begin{proof}
This follows by a direct reduction to semantic security of the distribution family $\{\cZ_\secp(\cdot)\}_{\secp \in \bbN}$. The reduction samples $\theta \gets \{0,1\}^\secp$, sends $\theta$ to its challenger, and receives either $\cZ_\secp(\theta)$ or $\cZ_\secp(0^\secp)$ from its challenger. Then, it prepares $\secp$ EPR pairs, runs $\cA_\secp$ on halves of the EPR pairs along with the output of the distribution it received from its challenger, and $b'$ for a random $b' \gets \{0,1\}$. After $\cA_\secp$ outputs $(x',\rho)$, it measures $\left\{\Pi_{x',\theta},\bbI - \Pi_{x',\theta}\right\}$ on the other halves of the EPR pairs. Note that the complexity of this reduction is equal to the complexity of $\cA$ plus an extra $\secp$ qubits of space and an extra linear time operation, so it is still in $\mathscr{A}$. If $\Pr[\Pi_{x',\theta},\Hyb_2(b)]$ is non-negligible this can be used to distinguish $\cZ_\secp(\theta)$ from $\cZ_\secp(0^\secp)$, due to \cref{claim:BF10}.
\end{proof}

Finally, we can show the following claim, which completes the proof.

\begin{claim}
$\Advt(\Hyb_2) = \negl(\secp).$
\end{claim}

\begin{proof}
First, we note that for any $b \in \{0,1\}$, the global state of $\Hyb_2(b)$ immediately after $\cA_\secp$ outputs $x'$ is within negligible trace distance of a state $\tau^{\sC,\sA'}_{\mathsf{Ideal}}$ in the image of $\bbI - \Pi_{x',\theta}$, where $\sA'$ is $\cA_\secp$'s quantum output register. This follows immediately from \cref{claim:predicate} and Gentle Measurement (\cref{lemma:gentle-measurement}). Now, consider the measurement of $\tau_{\mathsf{Ideal}}^{\sC,\sA'}$ on $\sC_{i: \theta_i = 1}$ that determines whether the experiment outputs $\bot$. That is, the procedure that measures $\sC_{i:\theta_i = 1}$ in the Hadamard basis and checks if the resulting string is equal to $x'_{i: \theta_i = 1}$. There are two options.

\begin{itemize}
    \item If the measurement fails, then the experiment outputs $\bot$, independent of whether $b=0$ or $b=1$, so there is 0 advantage in this case.
    \item If the measurement succeeds, then we know that the state on registers $\sC_{i: \theta_i = 0}$ is only supported on vectors $\ket{y}_1$ such that $\Delta(y,x'_{i: \theta_i = 0}) < 1/2$, since $\tau_{\mathsf{Ideal}}^{\sC,\sA'}$ was in the image of $\bbI - \Pi_{x',\theta}$. These registers are then measured in the computational basis to produce $\{x_i\}_{i:\theta_i = 0}$, and the experiment outputs $\bot$ if $\bigoplus_{i:\theta_i = 0}x_i \neq b' \oplus b$ and otherwise outputs the state on register $\sA'$. Note that (i) this decision is the \emph{only} part of the experiment that depends on $b$, and (ii) by \cref{thm:XOR-extractor}, the bit  $\bigoplus_{i:\theta_i = 0}x_i$ is \emph{uniformly random and independent} of the register $\sA'$, which is disjoint (but possibly entangled with) $\sC$. Thus, there is also 0 advantage in this case. 
    
    In slightly more detail, \cref{thm:XOR-extractor} says that making a Hadamard basis measurement of a register that is in a superposition of computational basis vectors with relative Hamming weight $< 1/2$ will produce a set of bits $\{x_i\}_{i: \theta_i = 0}$ such that $\bigoplus_{i: \theta_i = 0}x_i$ is a uniformly random bit, even given potentially entangled quantum side information. We can apply this lemma to our system on $\sC_{i: \theta_i = 0},\sA'$ by considering a change of basis that maps $\ket{x'_{i: \theta_i = 0}}_1 \to \ket{0}_0$. That is, the change of basis first applies Hadamard, and then an XOR with the fixed string $x'_{i: \theta_i = 0}$. Applying such a change of basis maps $\sC_{i: \theta_i = 0}$ to a state that is supported on vectors $\ket{y}_0$ such that $\omega(y) < 1/2$, and we want to claim that a \emph{Hadamard} basis measurement of the resulting state produces $\{x_i\}_{i: \theta_i = 0}$ such that $\bigoplus_{i: \theta_i = 0}x_i$ is uniformly random and independent of $\sA$. This is exactly the statement of \cref{thm:XOR-extractor}.
\end{itemize}

This completes the proof, since we have shown that there exists a single distribution, defined by $\tau^{\sC,\sA'}_{\mathsf{Ideal}}$, that is negligibly close to both $\Hyb_2(0)$ and $\Hyb_2(1)$.
\end{proof}

\end{proof}



%\input{SKE}



%Now, by gentle measurement, we can claim that the register $\sC$ in $\Hyb_2$ after the adversary sends $x'$ is within negligible trace distance of a state that is orthogonal to the projective measurement defined above. Note that the adversary's view in $\Hyb_2$ is completely independent of $b$, except for the decision made by the challenger of whether to abort, based on whether $\widehat{b} \neq b \oplus \bigoplus_{i: \theta_i = 0} x_i$. But conditioned on above, we know that $\bigoplus_{i: \theta_i = 0} x_i$, for $x_i$ produced by measuring registers $i$ such that $\theta_i = 0$ in the standard basis, is perfectly uniformly random from the adversary's view, even given quantum side information. Thus, $\Hyb_2$ is within negligble trace distance of a game in which the adversay has advantage 0, completing the proof.







%\begin{proof}(of \cref{thm:main-C}) For $b \in \{0,1\}$, let $\Hyb_0(b)$ be the distribution defined by sampling $x,\theta \gets \{0,1\}^\secp$ and outputting \[\ket{x}_\theta, b \oplus \bigoplus_{i:\theta_i = 0}x_i, \cZ_\secp(\theta),\] and let $\Hyb_1(b)$ be the distribution defined by sampling $x,\theta \gets \{0,1\}^\secp$ and outputting \[\ket{x}_\theta, b \oplus \bigoplus_{i:\theta_i = 0}x_i, \cZ_\secp(0^\secp).\]

%Since $\{\cA_\secp\}_{\secp \in \bbN} \in \mathscr{A}$, we have that for any $b \in \{0,1\}$, \[\bigg|\Pr\left[\cA_\secp(\Hyb_0(b)) = 1\right] - \Pr\left[\cA_\secp(\Hyb_1(b)) = 1\right]\bigg| = \negl(\secp).\] To complete the proof, we show that \[\TD\left(\Hyb_1(0),\Hyb_1(1)\right) = \negl(\secp).\] To see this, first note that since $\cZ_\secp(0^\secp)$ is the same in both distributions, we only have the show that \[\ket{x}_\theta,b \oplus \bigoplus_{i: \theta_i = 0} x_i\] for $x,\theta \gets \{0,1\}^\secp$ is a statistically hiding encryption of the bit $b$. Now, since $\frac{1}{2}\ket{+}\bra{+} + \frac{1}{2}\ket{-}\bra{-}$ is identically distributed to $\frac{1}{2}\ket{0}\bra{0} + \frac{1}{2}\ket{1}\bra{1}$ (since they are both maximally mixed), we have that the above distribution is identically distributed to \[x,b \oplus \bigoplus_{i:\theta_i = 0}x_i,\] for $x,\theta \gets \{0,1\}^\secp$. Now, conditioned on $x \neq 0^\secp$, this is a perfectly hiding encryption of $b$. Since $x$ is uniformly random, this occurs with all but negligible probability, completing the proof.
%\end{proof}



%\subsection{Applications}

%\begin{itemize}
    %\item PKE/IBE/ABE etc with everlasting security after deletion. This follows by setting the distribution to sample a public key and ciphertext encrypting $b$. To show this is stronger than previously considered definitions, it is easy to see that an unbounded distinguisher can reverse sample a secret key given the public key. Previous results were based on \emph{receiver non-committing} PKE \cite{10.1007/978-3-030-92062-3_21}, and were not known to provide \emph{everlasting} security after deletion is accepted and the secret key is leaked.
    %\item Commitment with certified everlasting hiding / ZK proofs with certified everlasting deletion. These can now be built from any one-way function, or from pseudo-random quantum states. Previously, these were built from a specific \emph{random oracle}-based commitment scheme \cite{cryptoeprint:2021:1315}.
    %\item Fully-homomorphic encryption with certified deletion, implying a delegation protocol secure against servers that are semi-honest during the computation and malicious during deletion.
    %\item Revocable time-release encryption. Previously, this required either exponential hardness assumptions (for super-logarithmic messages) or the random oracle model, and the deletion certificate was a quantum state \cite{EC:Unruh14}.
%\end{itemize}


%\begin{theorem}
%The following are all secure constructions of primitives with certified deletion. In each scheme, the deletion certificate $x' \in \{0,1\}^\secp$ is produced by measuring the $\secp$-qubit state in the Hadamard basis, and is accepted if $x'_i = x_i$ for all $i$ such that $\theta_i = 1$.
%\begin{itemize}
    %\item The following is a secure secret-key encryption scheme with certified deletion. To encrypt $b \in \{0,1\}$, sample $x,\theta \gets \{0,1\}^\secp, u \gets \{0,1\}$, set $\sk = (\theta,u)$, and output \[\ket{x}_\theta, u \oplus b \oplus \bigoplus_{i: \theta_i = 0} x_i.\]
    %\item Let $\PKE = (\Gen,\Enc,\Dec)$ be \emph{any} public-key encryption scheme. Then, the following is a secure public-key encryption scheme with certified deletion. Generate $(\pk,\sk) \gets \Gen(1^\secp)$. To encrypt $b \in \{0,1\}$, sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ket{x}_\theta, \Enc\left(\theta, b \oplus \bigoplus_{i : \theta_i = 0}x_i\right).\]
    %\item Let $\Com$ be \emph{any} statistically binding computationally hiding commitment scheme. Then, the following is a statistically binding commitment scheme with certified everlasting hiding. To commit to $b \in \{0,1\}$, sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ket{x}_\theta, \Com\left(\theta, b \oplus \bigoplus_{i : \theta_i = 0}x_i\right).\]
    %\item Let $\TRE = (\TRGen,\TREnc,\TRDec)$ be \emph{any} time-release encryption scheme. Then, the following is a time-release encryption scheme with certified deletion (also referred to as a \emph{revocable} time-release encryption scheme \cite{EC:Unruh14}). Generate $(\pk,\sk) \gets \TRGen(1^\secp)$. To encrypt $b \in \{0,1\}$, sample $x,\theta \gets \{0,1\}^\secp$ and output \[\ket{x}_\theta, \TREnc\left(\theta, b \oplus \bigoplus_{i : \theta_i = 0}x_i\right).\]
%\end{itemize}
%\end{theorem}


==> com-EST.tex <==
\section{Commitment with everlasting security transfer}


In this section, we construct a commitment that satisfies \emph{everlasting security transfer} (\cref{def:com-EST}), based only on the assumption that statistically binding computationally hiding commitments exist, which can either be based on the existence of one-way functions, or alternatively on the existence of pseudo-random quantum states. 

\protocol
{\proref{fig:com-EST}}
{Bit commitment with everlasting security transfer.}
{fig:com-EST}
{
Parties: committer $\cC_\secp$ with input $b$, receiver $\cR_\secp$.\\
Parameters: polynomials $n(\cdot)$ and $k(\cdot)$, and function $\gamma(\cdot)$.\\
Ingredients: a statistically binding computationally hiding commitment scheme $\SBCom$, and a secure two-party computation protocol $\Pi$ with one-sided statistical security.\\ \\
\noindent \textbf{Commit phase.}\\
\begin{itemize}
    \item $\cC_\secp$ samples $x_i,\theta_i \gets \{0,1\}^{n(\secp)}$ for each $i \in [k(\secp)]$, and sends $\{\ket{x_i}_{\theta_i}\}_{i \in [k(\secp)]}$ to $\cR_\secp$.
    \item For each $i \in [k(\secp)]$, execute the Commit phase of $\SBCom$, where the committer has input \[\left(\theta_i,b \oplus \bigoplus_{j : \theta_{i,j} = 0} x_{i,j}\right).\]
\end{itemize}
\noindent \textbf{Delete phase.}\\
\begin{itemize}
    \item For each $i \in [k(\secp)]$, $\cR_\secp$ samples $\theta_i' \gets \{0,1\}^{n(\secp)}$ and measures the $i$'th state received in the Commit phase in the $\theta_i'$ basis, obtaining $x_i' \in \{0,1\}^{n(\secp)}$.
    \item $\cC_\secp$ and $\cR_\secp$ engage in $\Pi$ with statistical security against $\cR$ to compute the following functionality. Take input $\{(x_i,\theta_i)\}_{i \in [k(\secp)]}$ from $\cC_\secp$ and input $\{(x_i',\theta_i')\}_{i \in [k(\secp)]}$ from $\cR$. Output 1 to $\cC_\secp$ if and only if the following conditions hold.
    \begin{itemize}
        \item For every $i \in [k(\secp)]$, the fraction of $\theta'_{i,j}$ such that $\theta'_{i,j} = 1$ is at least $1/2 - \gamma(\secp)$.
        \item For every $i \in [k(\secp)]$ and $j \in [n(\secp)]$ such that $\theta_{i,j} = \theta'_{i,j} = 1$, it holds that $x_{i,j} = x'_{i,j}$.
    \end{itemize}
    \item $\cC_\secp$ sets $d_\cC$ equal to the output of $\Pi$.
 \end{itemize}
\noindent \textbf{Reveal phase.}
\begin{itemize}
    \item $\cC_\secp$ sends $\{x_i\}_{i \in [k(\secp)]}$ to $\cR_\secp$. 
    \item For each $i \in [k(\secp)]$, execute the Reveal phase of $\SBCom$. If $\cR_\secp$ obtains $\bot$ from any of these executions, output $\bot$ and terminate. Otherwise, let $\{\theta_i,c_i\}_{i \in [k(\secp)]}$ be the strings obtained by $\cR_\secp$.
    \item $\cR_\secp$ checks that the following conditions holds.
    \begin{itemize}
        \item For each $i \in [k(\secp)]$, the fraction of $\theta_{i,j}$ such that $\theta_{i,j} = 0$ is at least $1/2 - \gamma(\secp)$.
        \item For each $i \in [k(\secp)]$ and $j \in [n(\secp)]$ such that $\theta_{i,j} = \theta'_{i,j} = 0$, it holds that $x_{i,j} = x'_{i,j}$.
        \item There exists a $b$ such that for all $i \in [k(\secp)]$, \[c_i \oplus \bigoplus_{j:\theta_{i,j} = 0}x_{i,j} = b.\]
    \end{itemize}
    If all conditions hold then output $b$, and otherwise output $\bot$.
\end{itemize}
}





==> com-ESTnew.tex <==
\section{Everlasting Security Transfer}
\subsection{Commitments with Everlasting Security Transfer}


We compile a statistically binding commitment with certified deletion(\cref{def:}) and non-interactive Reveal phase into one that satisfies \emph{everlasting security transfer} (\cref{def:com-EST}). %based only on the assumption that statistically binding computationally hiding commitments exist, which can either be based on the existence of one-way functions, or alternatively on the existence of pseudo-random quantum states. 

\protocol
{\proref{fig:com-EST}}
{Bit commitment with everlasting security transfer}
{fig:com-EST}
{
Parties: committer $\cC_\secp$ with input $b$, receiver $\cR_\secp$.\\
Parameters: polynomials $n(\cdot)$ and $k(\cdot)$, and function $\gamma(\cdot)$.\\
Ingredients: \\
(1) a statistically binding commitment $\mathsf{Com}$ with certified everlasting hiding, and\\ (2) a
secure two-party computation protocol $\Pi$ with one-sided statistical security.\\ \\
\noindent \textbf{Commit phase.}\\
\vspace{-8mm}
\begin{itemize}
    %\item $\cC_\secp$ samples $x_i,\theta_i \gets \{0,1\}^{n(\secp)}$ for each $i \in [k(\secp)]$, and sends $\{\ket{x_i}_{\theta_i}\}_{i \in [k(\secp)]}$ to $\cR_\secp$.
    \item %For $i \in [k(\secp)]$, 
    Let $b_1, \ldots, b_\secp$ denote a $2n/3$-out-of-$n$ secret sharing of the bit $b$.
    
    \item
    For every $i \in [\secp]$, execute the Commit phase of $\mathsf{Com}$, with committer input $b_i$.
    
    \item $\cR_\secp$ samples a random subset $T$ of $[n]$ of size $n/2$.
    %\vspace{-2mm}
    %\[\left(\theta_i,b \oplus \bigoplus_{j : \theta_{i,j} = 0} x_{i,j}\right).\]
    %\vspace{-8mm}
\end{itemize}
\noindent \textbf{Delete phase.}\\
\vspace{-8mm}
\begin{itemize}
    %\item 
    %For each $i \in [k(\secp)]$, $\cR_\secp$ samples $\theta_i' \gets \{0,1\}^{n(\secp)}$ and measures the $i$'th state received in the Commit phase in the $\theta_i'$ basis, obtaining $x_i' \in \{0,1\}^{n(\secp)}$.
    
    \item  Let $\cF$ denote a functionality that obtains input from $\cC_\secp$ $[n]$ verification keys
    $\{\vk_i\}_{i \in [n]}$;
    and input from $\cR_\secp$ a set $S \subset [n]$ of size $n/2$ and 
    deletion certificates corresponding to commitments in $S$, i.e., $\{\cert_i\}_{i \in S}$. 
    
    The functionality outputs 1 to $\cC_\secp$ if and only if $\mathsf{Ver}(\vk_i,\cert_i) = 1$ for all $i \in S$.

    
    \item $\cR_\secp$ runs the Delete phase for commitments in the subset $T$.
    
    \item
    $\cC_\secp$ and $\cR_\secp$ engage in $\Pi$ with statistical security against $\cR_\secp$ to compute $\cF$, where $\cC_\secp$ inputs  $\{\vk_i\}_{i \in [n]}$
    and $\cR_\secp$ inputs $T, \{\cert_i\}_{i \in T}$.
    $\cC_\secp$ returns the output of $\Pi$.
    %the following conditions hold.
    %\begin{itemize}
    %    \item For every $i \in [k(\secp)]$, the fraction of $\theta'_{i,j}$ such that $\theta'_{i,j} = 1$ is at least $1/2 - \gamma(\secp)$.
    %    \item For every $i \in [k(\secp)]$ and $j \in [n(\secp)]$ such that $\theta_{i,j} = \theta'_{i,j} = 1$, it holds that $x_{i,j} = x'_{i,j}$.
    %\end{itemize}
    %\item $\cC_\secp$ sets $d_\cC$ equal to the output of $\Pi$.
 \end{itemize}
\noindent \textbf{Reveal phase.}
\begin{itemize}
    \item $\cC_\secp$ sends $\cR_\secp$ all values $b, b_1, \ldots, b_\secp$.
   \item $\cC_\secp$ and $\cR_\secp$ execute the Reveal phase of $\mathsf{Com}$ for all $i \in [n]$.
   For any $i \in [n] \setminus T$, if $b_i \neq \mu_i$ where $\mu_i \leftarrow \mathsf{Rev}\langle \cC_\secp, \cR_\secp, \rho \rangle$, then $\cR_\secp$ outputs $\bot$.
   \item  $\cR_\secp$ outputs $b$ iff $b_1, \ldots, b_\secp$ is a $2n/3$-out-of-$n$ secret sharing of $b$, otherwise $\bot$.
    %\begin{itemize}
        %\item For each $i \in [k(\secp)]$, the fraction of $\theta_{i,j}$ such that $\theta_{i,j} = 0$ is at least $1/2 - \gamma(\secp)$.
        %\item For each $i \in [k(\secp)]$ and $j \in [n(\secp)]$ such that $\theta_{i,j} = \theta'_{i,j} = 0$, it holds that $x_{i,j} = x'_{i,j}$.
        %\item There exists a $b$ such that for all $i \in [k(\secp)]$, \[c_i \oplus \bigoplus_{j:\theta_{i,j} = 0}x_{i,j} = b.\]
    %\end{itemize}
    %If all conditions hold then output $b$, and otherwise output $\bot$.
\end{itemize}
}





==> definitions.tex <==
\section{Definitions}



\paragraph{Statistical-computational binding.} \james{placeholder name} Next, observe that the notion of statistical binding defined above does not guarantee anything in the case the Delete phase is executed. Thus, we formulate a definition of binding that remains meaningful even after a Delete phase is executed.

\begin{definition}[Statistical-computational binding.]\label{def:SCB}
A commitment scheme satisfies \emph{statistical-computational binding} if it satisfies statistical binding (\cref{def:SB}) and in addition satisfies the following property. For any unbounded adversary $\{\cC^*_{\Com,\secp}\}_{\secp \in \bbN}$ in the Commit phase, there exists an unbounded extractor $\cE = \{\cE_\secp\}_{\secp \in \bbN}$ such that for every QPT adversary $\{\cC^*_{\Del,\secp},\cC^*_{\Rev,\secp}\}_{\secp \in \bbN}$ in the Delete and Reveal phases, and every QPT distinguisher $\cD^* = \{\cD^*_{\secp}\}_{\secp \in \bbN}$, \[\bigg|\Pr\left[\cD^*_\secp\left(\Real_\secp^{\cC^*}\right) = 1\right] - \Pr\left[\cD^*_\secp\left(\Ideal_\secp^{\cC^*,\cE}\right) = 1\right]\bigg| = \negl(\secp),\] where $\Real_\secp^{\cC^*}$ and $\Ideal_\secp^{\cC^*,\cE}$ are defined as follows.
\begin{itemize}
    \item $\Real_\secp^{\cC^*}$: Execute the Commit phase $\rho_c^{\sC^*,\sR} \gets \Com\langle\cC^*_{\Com,\secp},\cR_{\Com,\secp}\rangle$. Execute the Delete phase $(d_\cC,\rho_d^{\sC^*,\sR}) \gets \Del\langle\cC^*_{\Del,\secp},\cR^*_{\Del,\secp},\rho_c^{\sC^*,\sR}\rangle$. Execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle\cC^*_{\Rev,\secp},\cR_{\Rev,\secp},\rho_d^{\sC^*,\sR}\rangle$ along with the committer's final state $\rho_r^{\sC^*}$. Output $(\mu,\rho_r^{\sC^*})$.
    \item $\Ideal_{\secp}^{\cC^*,\cE}$: Run the extractor $(\rho_c^{\sC^*,\sR},b^*) \gets \cE_\secp$, which outputs a joint state $\rho_c^{\sC^*,\sR}$ along with a bit $b^*$. Execute the Delete phase $(d_\cC,\rho_d^{\sC^*,\sR}) \gets \Del\langle\cC^*_{\Del,\secp},\cR^*_{\Del,\secp},\rho_c^{\sC^*,\sR}\rangle$. Execute the Reveal phase to obtain a trit $\mu \gets \Rev\langle\cC^*_{\Rev,\secp},\cR_{\Rev,\secp},\rho_d^{\sC^*,\sR}\rangle$ along with the committer's final state $\rho_r^{\sC^*}$. If $\mu \in \{\bot,b^*\}$ output $(\mu,\rho_r^{\sC^*})$, and otherwise output a special symbol $\Fail$. 
\end{itemize}
\end{definition}

\paragraph{Commitment with everlasting security transfer.} We define the notion of a bit commitment with \emph{everlasting security transfer}.

\begin{definition}[Commitment with everlasting security transfer]\label{def:com-EST}
A commitment scheme satisfies \emph{everlasting security transfer} if it is correct (satisfies \cref{def:correctness-decommitment} and \cref{def:correctness-deletion}), satisfies certified everlasting hiding (\cref{def:CEH}), and satisfies statistical-computational binding (\cref{def:SCB}).
\end{definition}



\subsection{Secure computation}

\paragraph{Functionalities and protocols.}
Let $\cF$ denote a \emph{functionality}, which is a classical interactive machine specifying some (potentially reactive) distributed classical computation. An $n$-party protocol $\Pi_\cF$ for $\cF$ consists of $n$ quantum interactive machines $P_1,\dots,P_n$.\footnote{Technically, $P_i$ are infinite families of interactive machines, parameterized by the security parameter $\secp$.} An adversary intending to attack the protocol can be described by a family $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$, where $\cA_\secp$ is a quantum interactive machine that corrupts a subset of parties $M \subset \{P_i\}_{i \in [n]}$, $\cD_\secp$ is a quantum machine, and $\ket{\psi}_\secp^{\sA,\sD}$ is an advice state on two registers $\sA,\sD$, where $\cA$ is initialized with register $\sA$. 

Given such an adversary, and a set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$ where $H = [n] \setminus M$, define the random variable $\Pi_\cF[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ as follows. $\cA_\secp(\sA)$ interacts with $\{P_i(x_{i,\secp})\}_{i \in H}$ during the execution of $\Pi_\cF$. $\cA_\secp$ outputs a quantum state on register $\sA'$, and $\{P_i(x_{i,\secp})\}_{i \in H}$ output classical strings $\{y_i\}_{i \in H}$. The output of the random variable then consists of the quantum state on registers $\sD$ and $\sA'$, along with $\{y_i\}_{i \in H}$. We will also define the random variable $\Pi_\cF^{\mathsf{Hon}}[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ to just consist of $\{y_i\}_{i \in H}$.

An \emph{ideal-world} protocol $\widetilde{\Pi}_\cF$ for functionality $\cF$ consists of ``dummy'' parties $\widetilde{P}_1,\dots,\widetilde{P}_n$ that have access to an additional ``trusted'' party that implements $\cF$. That is, $\widetilde{P}_1,\dots,\widetilde{P}_n$ each interact directly with $\cF$, which eventually returns outputs to them. We consider the execution of ideal-world protocols in the presence of a simulator, described by a family $\{\cS_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$. 

Given such a simulator, and a set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, define the random variable $\widetilde{\Pi}_\cF[\cS_\secp,\allowbreak\cD_\secp,\allowbreak\ket{\psi}^{\sA,\sD},\allowbreak\{x_{i,\secp}\}_{i \in H}]$ as follows. $\cS_\secp(\sA)$ interacts with $\{\widetilde{P}_i(x_{i,\secp})\}_{i \in H}$ during the execution of $\widetilde{\Pi}_\cF$. $\cS_\secp$ outputs a quantum state on register $\sA'$, and $\{\widetilde{P}_i(x_{i,\secp})\}_{i \in H}$ output classical strings $\{y_i\}_{i \in H}$. The output of the random variable then consists of the quantum state on registers $\sD$ and $\sA'$, along with $\{y_i\}_{i \in H}$. We will also define the random variable $\widetilde{\Pi}_\cF^{\mathsf{Hon}}[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}]$ to just consist of $\{y_i\}_{i \in H}$.

\paragraph{Security with abort.} We will by default consider the notion of \emph{security with abort}, where the ideal functionality $\cF$ is modified to (1) know the identities of corrupted parties and (2) be slightly reactive: after all parties have provided input, the functionality computes outputs and delivers the outputs to the corrupt parties only. Then the functionality awaits either a ``deliver'' or ``abort'' command from the corrupted parties. Upon receiving ``deliver'', the functionality delivers the outputs to all the honest parties. Upon receiving ``abort'', the functionality delivers $\abort$ to all the honest parties.


%\begin{definition}[Secure computation with abort]\label{def:MPC}
%A protocol $\Pi_\cF$ securely realizes a functionality $\cF$ with abort if for any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any subset of parties $M \subset [n]$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, it holds that for any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_\cF\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_\cF\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

%Moreover, we say that a protocol $\Pi_\cF$ realizes a functionality with \emph{statistical} security against some subset of parties $P \subseteq [n]$, if for any \emph{unbounded} adversary $\{\cA_{\secp},\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any set of parties $M \subseteq P$, there exists a simulator $\{\cS_{\secp},\}_{\secp \in \bbN}$ whose run-time is at most polynomially larger than $\cA_\secp$'s run-time, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, and any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,
%\begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_\cF\left[\cA_{\secp},\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_\cF\left[\cS_{\secp},\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

%\end{definition}


\paragraph{Certified everlasting security.} We will also consider the notion of \emph{certified everlasting security}. Here, $\cF$ is further modified to include a ``deletion'' phase after the abort phase described above, and we refer to the resulting ideal functionality as $\cF_{\Del}$. In this phase, $\cF_\Del$ takes as input a set of bits from each party $P_i$. For each honest party $P_i$, $\cF_\Del$ receives a set $\{d_{i,j}\}_{j \in [n] \setminus \{i\}}$, where each $d_{i,j}$ indicates whether $P_i$ deleted $P_j$'s input data. For each malicious party $P_i$, $\cF_\Del$ receives a set $\{d_{i,j}\}_{j \in H}$, where again each $d_{i,j}$ indicates whether $P_i$ deleted $P_j$'s input data. Then, $\cF_\Del$ returns to each party a set of bits. For each honest party $P_i$, $\cF_\Del$ returns a set of bits $\{d^*_{i,j}\}_{j \in [n] \setminus \{i\}}$, where $d^*_{i,j} \coloneqq d_{j,i}$ indicates whether party $P_j$ deleted $P_i$'s input data. For each malicious party $P_i$, $\cF_\Del$ returns a set of bits $\{d^*_{i,j}\}_{j \in H}$, where $d^*_{j,i} \coloneqq d_{j,i}$ indicates whether party $P_j$ deleted $P_i$'s data. 

Note that now each honest party $P_i$ is initialized with an additional input $\{d_{i,j}\}_{j \in [n] \setminus \{i\}}$, and obtains an additional output $\{d^*_{i,j}\}_{j \in [n] \setminus \{i\}}$. Given a set of malicious parties $M \subset [n]$, the honest party inputs $\{\{d_{i,j}\}_j\}_{i \in H}$, and the $\{\{d^*_{i,j}\}_j\}_{i \in H}$ included in each honest party output, define a flag $\mathsf{DEL}$ to be equal to $\top$ if $d_{i,j} = 0$ for all  $i \in H, j \in M$ and $d^*_{i,j} = 1$ for all $i \in H,j \in M$, and equal to $\bot$ otherwise. That is $\mathsf{DEL} = \top$ when (i) none of the honest parties deleted the malicious party input data and (ii) all of the malicious parties deleted the honest party input data. Note that $\mathsf{DEL}$ can be computed as a predicate on the outcome of random variables $\Pi_\cF$ or $\widetilde{\Pi}_\cF$, so below we will consider conditioning the output of these random variables on the outcome of $\mathsf{DEL}$. 

%\paragraph{Two-phase adversaries.} To realize our definitions of secure computation with certified everlasting security, we will construct protocols with two separate phases: an \emph{online} phase in which the ``original'' functionality is computed, and a \emph{deletion} phase in which parties exchange messages with the purpose of realizing the deletion phase of the ideal functionality described above. It will sometimes be convenient to explicitly consider two-phase adversaries $\{\cA_{1,\secp},\cA_{2,\secp}\}_{\secp \in \bbN}$, where $\cA_{1,\secp}$ interacts in the online phases, and then passes on a state to $\cA_{2,\secp}$, who interacts in the deletion phase. The reason for this is that we will sometimes want to consider adversaries that are \emph{unbounded} in the online phase but \emph{QPT} as soon as they receive honest party messages in the deletion phase.



\begin{definition}[Secure multi-party computation with certified everlasting security]\label{def:MPC-everlasting} A protocol $\Pi_{\cF_\Del}$ \emph{securely realizes} a functionality $\cF_\Del$ with abort and with certified everlasting security if for any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting any subset of parties $M \subset [n]$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$, such that for any set of honest party inputs $\{x_{i,\secp}\}_{i \in H}$, it holds that
\begin{itemize}
    \item For any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
    \item For any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,
    \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1 \ | \ \mathsf{DEL} = \top\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},\{x_{i,\secp}\}_{i \in H}\right]\right) = 1 \ | \ \mathsf{DEL} = \top\right]\bigg| = \negl(\secp).\end{align*}
\end{itemize}

\end{definition}

%We will also consider a special case of (potentially randomized) \emph{two-party} functionalities $\cF_\Del$ where only one party $P_1$ has an input and only the other party $P_2$ obtains output. We refer to such functionalities as \emph{uni-directional}, and we present a specialized definition of certified everlasting security for such protocols.

%\begin{definition}[Statistically secure computation of uni-directional functionalities with certified everlasting security]\label{def:uni-directional}
%For a uni-directional two-party functionality $\cF_\Del$, a protocol $\Pi_{\cF_\Del}$ statistically securely realizes $\cF_\Del$ with certified everlasting security if the following two properties hold.
%\begin{itemize}
    %\item \cref{def:MPC-everlasting} holds for any adversary that corrupts party $P_2$.
    %\item For any \emph{unbounded} adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA}\}_{\secp \in \bbN}$ that corrupts party $P_1$, it holds that for any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF_\Del}^{\mathsf{Hon}}\left[\cA_\secp,\ket{\psi}_\secp^{\sA}\right]\right) = 1\right] - \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF_\Del}^{\mathsf{Hon}}\left[\cS_\secp,\ket{\psi}_\secp^{\sA}\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
%\end{itemize}
%\end{definition}

\paragraph{Oblivious transfer}

In this work, our building block will be the \emph{oblivious transfer} (OT) functionality. $\cF[\OT]$ is a two-party functionality between a sender $\cS$ with input $m_0,m_1 \in \{0,1\}^\ell$ and a receiver $\cR$ with input $b \in \{0,1\}$. The functionality delivers $m_b$ as output to the receiver. 

We will consider the following ideal functionality $\cF[\OT]_\Del$ where only the receiver $\cR$ has the ability to delete data. That is, in the ``deletion'' phase, $\cF[\OT]_\Del$ will take as input a bit $d_\cR$ from the receiver and deliver it to the sender $\cS$. 

\begin{definition}[Statistically sender private (SSP) OT with everlasting security transfer]\label{def:SSP-transfer}
An SSP OT with everlasting security transfer is a protocol $\Pi_{\cF[\OT]_\Del}$ such that the following two properties hold.
\begin{itemize}
    \item For any QPT adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the receiver $\cR$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$ such that for any sender inputs $\{(m_{0,\secp},m_{1,\secp})\}_{\secp \in \bbN}$, it holds that 
    \begin{itemize}
        \item For any QPT distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
        \item For any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$,\begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1 \ | \ d_\cR = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(m_{0,\secp},m_{1,\secp})\right]\right) = 1 \ | \ d_\cR = 1\right]\bigg| = \negl(\secp).\end{align*}
    \end{itemize}
    \item For any \emph{unbounded} adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the sender $\cS$, there exists a simulator $\{\cS_\secp\}_{\secp \in \bbN}$ with run-time at most polynomially larger than $\cA_\secp$, such that for any receiver inputs $\{b_\secp,d_\cR \coloneqq 0\}_{\secp \in \bbN}$, it holds that for any \emph{unbounded} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,0)\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,0)\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}
    \item For any \emph{QPT} adversary $\{\cA_\secp,\ket{\psi}_\secp^{\sA,\sD}\}_{\secp \in \bbN}$ corrupting the sender $\cS$, there exists a QPT simulator $\{\cS_\secp\}_{\secp \in \bbN}$ such that for any receiver inputs $\{b_\secp,d_\cR \coloneqq 1\}_{\secp \in \bbN}$, it holds that for any \emph{QPT} distinguisher $\{\cD_\secp\}_{\secp \in \bbN}$, \begin{align*}&\bigg|\Pr\left[\cD_\secp\left(\Pi_{\cF[\OT]_\Del}\left[\cA_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,1)\right]\right) = 1\right]\\ &- \Pr\left[\cD_\secp\left(\widetilde{\Pi}_{\cF[\OT]_\Del}\left[\cS_\secp,\ket{\psi}_\secp^{\sA,\sD},(b_\secp,1)\right]\right) = 1\right]\bigg| = \negl(\secp).\end{align*}

    
\end{itemize}
\end{definition}


%\paragraph{Outline} 
%\begin{itemize}
    %\item Build OT satisfying \cref{def:SSP-transfer}
    %\item Show such an OT implies \cref{def:uni-directional} via Kil88, which then implies zero-knowledge proofs with certified everlasting zero-knowledge
    %\item Show such an OT implies \cref{def:MPC-everlasting} via IPS08
%\end{itemize}




%We will also show that our OT protocol satisfies an alternative definition that will be useful for building protocols that satisfy \cref{def:uni-directional}. Our protocols $\Pi$ for OT will come in two phases: an OT phase and a deletion phase. We will refer to $\Pi_{\cF[\OT]_\Del}$ as the protocol that includes both phases and $\Pi_{\cF[\OT]}$ as the protocol that only includes the OT phase.

%\begin{definition}[Statistically sender private (SSP) OT with everlasting security transfer]
%An SSP OT with everlasting security transfer is a protocol $\Pi$ such that $\Pi_{\cF[\OT]}$ satisfies \cref{def:MPC} with statistical security against any adversary that corrupts the sender $\cS$, and such that $\Pi_{\cF[\OT]_\Del}$ satisfies \cref{def:MPC-everlasting} against any adversary that corrupts the receiver $\cR$.
%\end{definition}

==> everlasting-security.tex <==
\subsection{Everlasting Security}

\cite{cryptoeprint:2021:1315} showed how to construct statistically binding commitment schemes where hiding is computational during the protocol execution, but holds unconditionally and everlasting against a verifier that provides a ``proof of deletion'' after the protocol completes. This can be used to build a proof system with a similar certified deletion property for zero-knowledge.

Such a commitment can be built in the plain model as follows.

\begin{itemize}
    \item Instantiate the BCKM quantum commitments with a statistically hiding commitment for the measurement check (which must be either collapse-binding or extractable).
    \item The proof of deletion is the openings of all of the measurement check commitments.
\end{itemize}

Now consider two-party computation. We want to do 2PC in a way that allows either party at any point after the protocol to ask the other party to delete their information, so that the protocol is now everlasting secure against them. This can be accomplished (at least for NC1 circuits) using an OT that is statistically secure against the sender, but also allows the sender to ask for a proof of deletion from the receiver that erases all information about $m_{1-b}$, but at the same time does not reveal $b$ (at least, against a computationally bounded sender). 

\begin{itemize}
    \item Instantiate the BCKM quantum OT with a statistically hiding (extractable) commitment that is used to commit to statistically binding commitments to the measurement results.
    \item During measurement check, the receiver will open the double commitments at all checked positions.
    \item The proof of deletion is the openings of the outer (statistically hiding) commitments at the non-checked positions, to reveal the statistically binding commitments. 
\end{itemize}

Questions:

\begin{itemize}
    \item Can we extend the 2PC with either-sided everlasting security to all polynomial size circuits?
    (probably with Kilian, yes)
    \item Can we extend to MPC with everlasting against all but one?
    \item Look at combiner approach to the above that doesn't require double commitments.
\end{itemize}  

More ambitious questions:
\begin{itemize}
    \item Is it possible to have a protocol that is statistically secure against honest majority during the protocol, and then everlasting secure against arbitrary collusion given deletion certificates?
    \item Call the process of transferring everlasting security from one player to the other by issuing a certificate -- everlasting security transfer. Can we design protocols that allow this to be done more than once? Unbounded number of times?
    
    \item Can we combine this with FHE?
    \item Can we make the server be quantum and the client be classical?
\end{itemize}

==> implication-deprecated.tex <==
\section{Relation with~\cite{10.1007/978-3-030-92062-3_21}'s definitions}
\label{sec:implication}
In this section, we prove that our definitions of certified deletion security for PKE and ABE imply prior definitions~\cite{10.1007/978-3-030-92062-3_21}. First, we reproduce the definitions in~\cite{10.1007/978-3-030-92062-3_21}, albeit following our notational conventions, for the settings of public-key encryption and attribute-based encryption below.

\begin{definition}[Certified deletion security for PKE in~\cite{10.1007/978-3-030-92062-3_21}]
\label{def:CD-security-prior}
$\CD$-$\PKE = (\Gen,\Enc,\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, it holds that 
\[\bigg|\Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\]
where the experiment $\mathsf{C}'\text{-}\EXP_\secp^{\cA}(b)$ is defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$ and $(\ct,\vk) \gets \Enc(\pk,b)$.
    \item Initialize $\cA_\secp(\ket{\psi_\secp})$ with $\pk$ and $\ct$.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$, set $\mathsf{ret} = \sk$, otherwise set $\mathsf{ret} = \bot$.
    \item Output $\cA_\secp \left(\rho, \mathsf{ret} \right)$.
    %\item If $\Ver(\vk,\cert) = \top$ then output $\rho$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

\begin{definition}[Certified deletion security for ABE in~\cite{10.1007/978-3-030-92062-3_21}]
\label{def:CD-sec-ABE-prior}
$\CD$-$\ABE = (\Gen,\KG,\Enc,\allowbreak\Dec,\Del,\Ver)$ satisfies \emph{certified deletion security} if for any non-uniform QPT adversary $\cA = \{\cA_\secp,\ket{\psi}_\secp\}_{\secp \in \bbN}$, it holds that 
\[\bigg|\Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(1) = 1\right]\bigg| = \negl(\secp),\] 
where the experiment $\mathsf{C}'\text{-}\EXP_\secp^{\cA}(b)$ is defined as follows.
%Both experiments take an input $b$, and interact with $\cA$ as follows.
\begin{itemize}
    \item Sample $(\pk,\msk) \gets \Gen(1^\secp)$
    and %send $\pk$ to $\cA$.
    %and $(\ct,\vk) \gets \Enc(\pk,b)$.
    %\item Initialize 
    initialize
    $\cA_\secp(\ket{\psi_\secp})$ with $\pk$.
    %and $\ct$.
    \item Set $i = 1$.
    \item If $\cA_\secp$ outputs a key query $P_i$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ and set $i = i + 1$. This process can be repeated polynomially many times.
    \item If $\cA_\secp$ outputs an attribute $X^*$ and a pair of messages $(m_0, m_1)$ where $P_i(X^*) = 0$ for all predicates $P_i$ queried so far, then compute $(\vk,\ct) = \Enc(\pk, X^*, m_b)$ and return $\ct$ to $\cA_\secp$, else exit and output $\bot$.
    \item If $\cA_\secp$ outputs a key query $P_i$ such that $P_i(X^*) = 0$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ (otherwise return $\bot$) and set $i = i + 1$. This process can be repeated polynomially many times.
    \item Parse $\cA_\secp$'s output as a deletion certificate $\cert$ and a left-over quantum state $\rho$.
    \item If $\Ver(\vk,\cert) = \top$ set $\mathsf{ret} = \msk$, and otherwise set $\mathsf{ret} = \bot$. Send $\mathsf{ret}$ to $\cA_\secp$.
    \item Again, upto polynomially many times, $\cA_\secp$ sends key queries $P_i$. For each $i$, if $P_i(X^*) = 0$, return $\sk_{P_i} \leftarrow \KG(\msk, P_i)$ to $\cA_\secp$ (otherwise return $\bot$) and set $i = i + 1$.
    Finally, $\cA_\secp$ generates an output bit, which is set to be the output of $\mathsf{C}'\text{-}\EXP_\secp^{\cA}(b)$.
    %$\CEXP_\secp^{\cA}(b)$ outputs $(\rho, \Ver(\vk,\cert))$.
\end{itemize}
\end{definition}

\begin{claim}
Any PKE scheme satisfying Definition \ref{def:CD-security} also satisfies Definition \ref{def:CD-security-prior}.
\end{claim}
\begin{proof}
Suppose the claim is not true. Then there exists an adversary $\cA$ and polynomial $p(\cdot)$ such that with respect to the notation in Definition \ref{def:CD-security-prior},
\[\bigg|\Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(1) = 1\right]\bigg| = \frac{1}{p(\secp)},\] 
and yet for every adversary $\cB$, with respect to the notation in Definition \ref{def:CD-security},
\begin{equation}
\label{eq:everlasting}
\TD\left(\EVEXP_\secp^{\cB}(0),\EVEXP_\secp^{\cB}(1)\right) = \negl(\secp),
\end{equation}
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cB}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cB}(1) = 1\right]\bigg| = \negl(\secp),\] 
Now we consider the following (efficient) reduction $\cR = \{\cR_\secp\}_{\secp \in \bbN}$ that acts as an adversary in the experiment $\CEXP$.
$\cR_\secp$ passes $\pk$ and $\ct$ to $\cA_\secp$, then passes the deletion certificate output by $\cA_\secp$ to its challenger and saves its residual state $\rho$. $\cR_\secp$ then obtains a verification outcome in $\{ \bot, \top \}$ from the challenger. 
If the outcome is $\top$, $\cR$ aborts, and otherwise $\cR_\secp$ outputs $\cA_\secp(\rho,\bot)$. 

By equation~(\ref{eq:everlasting}), when the outcome is $\top$, the resulting state $\rho$ in $\mathsf{C}'\text{-}\EXP_\secp^{\cA}(b)$ is statistically independent of $b$ (and in particular, since the distribution over $\sk$ is fixed by $\pk$ and is otherwise independent of $\ct$, the state is also statistically independent given $\sk$). Thus, except for a negligible loss, any advantage of $\cA_\secp$ can only manifest in the case when the output is $\bot$, which implies that
\[\bigg|\Pr\left[\CEXP_\secp^{\cR}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cR}(1) = 1\right]\bigg| = \frac{1}{p(\secp)} - \negl(\secp) > \frac{1}{2p(\secp)},\]
a contradiction.
\end{proof}


\begin{claim}
Any ABE scheme satisfying Definition \ref{def:CD-sec-ABE} also satisfies Definition \ref{def:CD-sec-ABE-prior}.
\end{claim}
\begin{proof}
Suppose the claim is not true. Then there exists an adversary $\cA$ and polynomial $p(\cdot)$ such that with respect to the notation in Definition \ref{def:CD-sec-ABE-prior},
\[\bigg|\Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(0) = 1\right] - \Pr\left[\mathsf{C}'\text{-}\EXP_\secp^{\cA}(1) = 1\right]\bigg| = \frac{1}{p(\secp)},\] 
and yet for every adversary $\cB$,with respect to the notation in Definition \ref{def:CD-sec-ABE},
\begin{equation}
\label{eq:everlasting2}
\TD\left(\EVEXP_\secp^{\cB}(0),\EVEXP_\secp^{\cB}(1)\right) = \negl(\secp),
\end{equation}
and
\[\bigg|\Pr\left[\CEXP_\secp^{\cB}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cB}(1) = 1\right]\bigg| = \negl(\secp),\] 
Now we consider the following (efficient) reduction $\cR = \{\cR_\secp\}_{\secp \in \bbN}$ that acts as an adversary in the experiment $\CEXP$.
$\cR_\secp$ passes $\pk$ to $\cA_\secp$, then forwards all key queries of $\cA_\secp$ to its challenger, and forwards challenger responses back to $\cA_\secp$. Furthermore, it forwards any attribute $X^*$ and pair of messages $(m_0, m_1)$ output by $\cA_\secp$ to its challenger.
Finally, it passes the deletion certificate output by $\cA_\secp$ to its challenger and saves its residual state $\rho$. $\cR_\secp$ then obtains a verification outcome in $\{ \bot, \top \}$ from the challenger. 
If the outcome is $\top$, $\cR$ aborts, and otherwise $\cR_\secp$ outputs $\cA_\secp(\rho,\bot)$. 

By equation~(\ref{eq:everlasting2}), when the outcome is $\top$, the resulting state $\rho$ in $\mathsf{C}'\text{-}\EXP_\secp^{\cA}(b)$ is statistically independent of $b$ (and in particular, since the distribution over $\msk$ is fixed by $\pk$ and is otherwise independent of $\ct$, the state is also statistically independent given $\msk$). Thus, except for a negligible loss, any advantage of $\cA_\secp$ can only manifest in the case when the output is $\bot$, which implies that
\[\bigg|\Pr\left[\CEXP_\secp^{\cR}(0) = 1\right] - \Pr\left[\CEXP_\secp^{\cR}(1) = 1\right]\bigg| = \frac{1}{p(\secp)} - \negl(\secp) > \frac{1}{2p(\secp)},\]
a contradiction.
\end{proof}

==> notes.tex <==
\section{Notes}

\input{everlasting-security}
\input{zero-knowledge}
\input{ot}

==> ot.tex <==
\subsection{Quantum OT with Unbounded Everlasting Security Transfer}
Maybe this is the right way to go about it. writing a very informal sketch below mostly so that I dont forget.
\begin{itemize}
    \item Instantiate the BCKM quantum OT with a statistically hiding (extractable) commitment that is used to commit to the measurement results.
    \item The measurement check and all subsequent steps will happen under the hood of a regular OT. During measurement check, the receiver will open the statistically hiding commitments at all checked positions, but a (PPT) receiver won't know the set T of checked positions.
    \item The proof of deletion from receiver Bob to sender Alice is a set of statistically binding extractable commitments to openings of their statistically hiding commitments, along with a proof (of knowledge?) that the committed openings are valid openings of the shcoms. 
    Each statistically binding extractable commitment is implemented via the same OT template, but where the commitment receiver, i.e. Alice performs measurements and commits to them via shcoms.
    
    This PoK can be implemented via 2PC with statistical security against Bob -- into the 2PC, Alice inputs the state she will use to verify Bob's decommitments, and Bob inputs his decommitments. The 2PC returns 1 to Alice if these all verify against Bob's original shcoms.
    
    Proof sketch: By soundness of the proof (of knowledge?), for any PPT receiver: whether we verify the measurement outcomes extracted from the OT, or once the certificate is produced we brute-force extract from the statistically binding commitments and verify what we extracted; the outcome should be the same. 
    By security of the regular OT, the probability, for any PPT receiver, that the check verifies on a randomly sampled subset of positions does not depend on the set T that was checked.
    \item Now the reason each statistically binding commitment used in the certificate actually involves the CK template itself - is to enable the next round of security transfer from sender to receiver. Namely the sender will send shcoms to their measurement results, and for the next round the process will repeat.
\end{itemize}

-- can we delete secret keys

==> zero-knowledge.tex <==
\subsection{Quantum Zero Knowledge}

Can we show that the following protocol is zero-knowledge with strict polynomial-time simulation? Would that contradict \cite{cryptoeprint:2021:376}?

\begin{itemize}
    \item The verifier samples BB84 states and sends them along with commitments to the bases $\Theta$.
    \item The prover samples $\Theta'$, measures in $\Theta'$, and sends $\Theta'$ along with the measurement results.
    \item The verifier checks that the appropriate measurements match, then sends $\Theta$.
    \item The prover proves a WI that either $x \in \cL$ or they know the bits encoded in the original BB84 states.
\end{itemize}

The simulation strategy would be to commit to the results of measuring the BB84 states in superposition, and then run the verifier sending $\Theta$ in superposition. If the verifier never aborts, this would allow to measure $\Theta$ and rewind without disturbing the initial BB84 states. What about a verifier that sometimes aborts?


